How common are extreme scattering events?: First large sample from the ASKAP VAST survey

Compact radio sources are occasionally observed to undergo extreme scattering events (ESEs): large, chromatic flux-density variations, often by more than a factor of two, over a few months. These were interpreted to be a smooth plasma lensing phenomenon due to AU-scale structures in the ISM. Although ESEs were discovered decades ago, observationally, only a few tens of ESEs have been reported, often from individual sources monitored at very high cadences. As such, the nature of the plasma lenses generating such events remains elusive. In this article, we present the most comprehensive sample of ESEs to date, using the ASKAP Variables and Slow Transients (VAST) survey. We report the discovery of a three-tier sample --- 72 sources that show promising ESE events (gold), 76 sources that are likely ESE-exhibiting (silver), and an additional 88 sources where ESE events are one plausible explanation (bronze). We show that the light curves demonstrate varied morphologies, which can be interpreted in terms of the source size and the strength of the lens in the paradigm of a simple one-dimensional Gaussian lens model. The spatial distribution of ESEs shows an appreciable excess in the direction of the Galactic center and along the Galactic loops. Using this sample, we infer an overall rate of 0.012 such events per year per deg^2 (or 0.006 events per source per year) for our (gold+silver) sample, for sources with mean flux density above 5 mJy at 888 MHz (0.01% of all isolated point sources detected in VAST).

==> ese_lcs.tex <==
\begin{figure*}
\label{fig:ese_lcs_1}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J00h23m42.9s-59d30m32.0s_lc_fit.pdf}{0.24\linewidth}{J00h23m42.9s$-$59d30m32.0s}
	\fig{lcs/J01h15m12.5s-29d41m45.3s_lc_fit.pdf}{0.24\linewidth}{J01h15m12.5s$-$29d41m45.3s}
	\fig{lcs/J01h50m09.8s-45d22m55.2s_lc_fit.pdf}{0.24\linewidth}{J01h50m09.8s$-$45d22m55.2s}
	\fig{lcs/J02h11m49.1s+06d00m14.5s_lc_fit.pdf}{0.24\linewidth}{J02h11m49.1s+06d00m14.5s}}
\gridline{\fig{lcs/J03h04m38.5s+00d12m41.7s_lc_fit.pdf}{0.24\linewidth}{J03h04m38.5s+00d12m41.7s}
	\fig{lcs/J03h11m05.9s-08d12m31.3s_lc_fit.pdf}{0.24\linewidth}{J03h11m05.9s$-$08d12m31.3s}
	\fig{lcs/J03h15m56.2s-06d25m01.6s_lc_fit.pdf}{0.24\linewidth}{J03h15m56.2s$-$06d25m01.6s}
	\fig{lcs/J03h58m55.3s+06d34m40.1s_lc_fit.pdf}{0.24\linewidth}{J03h58m55.3s+06d34m40.1s}}
\gridline{\fig{lcs/J04h02m42.0s+08d25m24.1s_lc_fit.pdf}{0.24\linewidth}{J04h02m42.0s+08d25m24.1s}
	\fig{lcs/J04h03m58.8s+06d45m38.9s_lc_fit.pdf}{0.24\linewidth}{J04h03m58.8s+06d45m38.9s}
	\fig{lcs/J04h08m00.2s-32d50m02.5s_lc_fit.pdf}{0.24\linewidth}{J04h08m00.2s$-$32d50m02.5s}
	\fig{lcs/J04h09m29.7s+00d11m36.5s_lc_fit.pdf}{0.24\linewidth}{J04h09m29.7s+00d11m36.5s}}
\gridline{\fig{lcs/J04h26m32.5s+02d22m59.1s_lc_fit.pdf}{0.24\linewidth}{J04h26m32.5s+02d22m59.1s}
	\fig{lcs/J04h27m22.4s-49d07m41.9s_lc_fit.pdf}{0.24\linewidth}{J04h27m22.4s$-$49d07m41.9s}
	\fig{lcs/J04h30m06.7s-39d06m22.2s_lc_fit.pdf}{0.24\linewidth}{J04h30m06.7s$-$39d06m22.2s}
	\fig{lcs/J04h31m24.7s+06d22m08.5s_lc_fit.pdf}{0.24\linewidth}{J04h31m24.7s+06d22m08.5s}}
\gridline{\fig{lcs/J04h31m36.0s-08d04m34.7s_lc_fit.pdf}{0.24\linewidth}{J04h31m36.0s$-$08d04m34.7s}
	\fig{lcs/J04h37m38.5s-44d54m26.6s_lc_fit.pdf}{0.24\linewidth}{J04h37m38.5s$-$44d54m26.6s}
	\fig{lcs/J04h45m04.7s-39d37m12.7s_lc_fit.pdf}{0.24\linewidth}{J04h45m04.7s$-$39d37m12.7s}
	\fig{lcs/J04h49m37.4s+08d11m33.9s_lc_fit.pdf}{0.24\linewidth}{J04h49m37.4s+08d11m33.9s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_2}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J04h51m27.2s+08d12m53.7s_lc_fit.pdf}{0.24\linewidth}{J04h51m27.2s+08d12m53.7s}
	\fig{lcs/J05h00m04.8s+00d14m20.8s_lc_fit.pdf}{0.24\linewidth}{J05h00m04.8s+00d14m20.8s}
	\fig{lcs/J05h02m37.9s-04d35m09.2s_lc_fit.pdf}{0.24\linewidth}{J05h02m37.9s$-$04d35m09.2s}
	\fig{lcs/J05h03m32.1s-04d57m56.0s_lc_fit.pdf}{0.24\linewidth}{J05h03m32.1s$-$04d57m56.0s}}
\gridline{\fig{lcs/J05h07m03.7s-08d40m08.8s_lc_fit.pdf}{0.24\linewidth}{J05h07m03.7s$-$08d40m08.8s}
	\fig{lcs/J05h08m31.9s+06d00m11.9s_lc_fit.pdf}{0.24\linewidth}{J05h08m31.9s+06d00m11.9s}
	\fig{lcs/J05h08m48.5s-45d09m20.6s_lc_fit.pdf}{0.24\linewidth}{J05h08m48.5s$-$45d09m20.6s}
	\fig{lcs/J05h09m12.5s-45d22m19.2s_lc_fit.pdf}{0.24\linewidth}{J05h09m12.5s$-$45d22m19.2s}}
\gridline{\fig{lcs/J05h09m17.4s-00d24m26.0s_lc_fit.pdf}{0.24\linewidth}{J05h09m17.4s$-$00d24m26.0s}
	\fig{lcs/J05h12m32.0s-02d58m29.1s_lc_fit.pdf}{0.24\linewidth}{J05h12m32.0s$-$02d58m29.1s}
	\fig{lcs/J05h13m41.0s-09d22m14.6s_lc_fit.pdf}{0.24\linewidth}{J05h13m41.0s$-$09d22m14.6s}
	\fig{lcs/J05h14m50.7s+02d48m29.1s_lc_fit.pdf}{0.24\linewidth}{J05h14m50.7s+02d48m29.1s}}
\gridline{\fig{lcs/J05h14m52.0s-00d54m15.6s_lc_fit.pdf}{0.24\linewidth}{J05h14m52.0s$-$00d54m15.6s}
	\fig{lcs/J05h16m45.1s+07d41m23.3s_lc_fit.pdf}{0.24\linewidth}{J05h16m45.1s+07d41m23.3s}
	\fig{lcs/J05h19m41.1s+00d34m30.3s_lc_fit.pdf}{0.24\linewidth}{J05h19m41.1s+00d34m30.3s}
	\fig{lcs/J05h23m25.7s+01d58m37.2s_lc_fit.pdf}{0.24\linewidth}{J05h23m25.7s+01d58m37.2s}}
\gridline{\fig{lcs/J05h28m03.1s-33d03m48.2s_lc_fit.pdf}{0.24\linewidth}{J05h28m03.1s$-$33d03m48.2s}
	\fig{lcs/J05h51m09.4s-04d06m55.1s_lc_fit.pdf}{0.24\linewidth}{J05h51m09.4s$-$04d06m55.1s}
	\fig{lcs/J05h52m02.1s-30d09m36.1s_lc_fit.pdf}{0.24\linewidth}{J05h52m02.1s$-$30d09m36.1s}
	\fig{lcs/J06h01m58.9s-05d27m50.8s_lc_fit.pdf}{0.24\linewidth}{J06h01m58.9s$-$05d27m50.8s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_3}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J06h11m39.7s-01d18m01.9s_lc_fit.pdf}{0.24\linewidth}{J06h11m39.7s$-$01d18m01.9s}
	\fig{lcs/J06h36m44.1s-05d30m01.9s_lc_fit.pdf}{0.24\linewidth}{J06h36m44.1s$-$05d30m01.9s}
	\fig{lcs/J07h13m28.3s+06d51m41.9s_lc_fit.pdf}{0.24\linewidth}{J07h13m28.3s+06d51m41.9s}
	\fig{lcs/J07h28m56.5s-06d11m40.1s_lc_fit.pdf}{0.24\linewidth}{J07h28m56.5s$-$06d11m40.1s}}
\gridline{\fig{lcs/J07h40m04.9s+04d15m28.6s_lc_fit.pdf}{0.24\linewidth}{J07h40m04.9s+04d15m28.6s}
	\fig{lcs/J07h46m13.8s-07d28m22.5s_lc_fit.pdf}{0.24\linewidth}{J07h46m13.8s$-$07d28m22.5s}
	\fig{lcs/J07h58m28.0s+08d27m08.3s_lc_fit.pdf}{0.24\linewidth}{J07h58m28.0s+08d27m08.3s}
	\fig{lcs/J08h54m39.5s+08d43m25.7s_lc_fit.pdf}{0.24\linewidth}{J08h54m39.5s+08d43m25.7s}}
\gridline{\fig{lcs/J08h56m34.8s-06d54m09.4s_lc_fit.pdf}{0.24\linewidth}{J08h56m34.8s$-$06d54m09.4s}
	\fig{lcs/J09h01m08.6s-00d33m34.0s_lc_fit.pdf}{0.24\linewidth}{J09h01m08.6s$-$00d33m34.0s}
	\fig{lcs/J09h09m43.2s+03d09m22.3s_lc_fit.pdf}{0.24\linewidth}{J09h09m43.2s+03d09m22.3s}
	\fig{lcs/J09h17m08.1s-03d06m18.0s_lc_fit.pdf}{0.24\linewidth}{J09h17m08.1s$-$03d06m18.0s}}
\gridline{\fig{lcs/J09h42m15.5s+04d36m22.1s_lc_fit.pdf}{0.24\linewidth}{J09h42m15.5s+04d36m22.1s}
	\fig{lcs/J10h12m19.1s-30d22m37.2s_lc_fit.pdf}{0.24\linewidth}{J10h12m19.1s$-$30d22m37.2s}
	\fig{lcs/J10h20m59.6s-36d14m26.7s_lc_fit.pdf}{0.24\linewidth}{J10h20m59.6s$-$36d14m26.7s}
	\fig{lcs/J10h24m43.5s-37d33m47.2s_lc_fit.pdf}{0.24\linewidth}{J10h24m43.5s$-$37d33m47.2s}}
\gridline{\fig{lcs/J10h26m45.9s-28d56m41.1s_lc_fit.pdf}{0.24\linewidth}{J10h26m45.9s$-$28d56m41.1s}
	\fig{lcs/J10h33m06.1s-30d54m39.9s_lc_fit.pdf}{0.24\linewidth}{J10h33m06.1s$-$30d54m39.9s}
	\fig{lcs/J10h44m24.0s-30d40m58.0s_lc_fit.pdf}{0.24\linewidth}{J10h44m24.0s$-$30d40m58.0s}
	\fig{lcs/J10h55m29.0s-30d11m03.2s_lc_fit.pdf}{0.24\linewidth}{J10h55m29.0s$-$30d11m03.2s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_4}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J10h56m13.1s-35d27m35.5s_lc_fit.pdf}{0.24\linewidth}{J10h56m13.1s$-$35d27m35.5s}
	\fig{lcs/J10h58m34.4s-42d15m13.3s_lc_fit.pdf}{0.24\linewidth}{J10h58m34.4s$-$42d15m13.3s}
	\fig{lcs/J11h02m20.7s+01d42m05.5s_lc_fit.pdf}{0.24\linewidth}{J11h02m20.7s+01d42m05.5s}
	\fig{lcs/J11h32m48.9s-50d48m58.8s_lc_fit.pdf}{0.24\linewidth}{J11h32m48.9s$-$50d48m58.8s}}
\gridline{\fig{lcs/J11h32m59.3s-48d42m35.1s_lc_fit.pdf}{0.24\linewidth}{J11h32m59.3s$-$48d42m35.1s}
	\fig{lcs/J11h33m47.6s-35d38m59.4s_lc_fit.pdf}{0.24\linewidth}{J11h33m47.6s$-$35d38m59.4s}
	\fig{lcs/J11h37m00.5s-45d05m12.6s_lc_fit.pdf}{0.24\linewidth}{J11h37m00.5s$-$45d05m12.6s}
	\fig{lcs/J11h43m39.8s+07d00m12.6s_lc_fit.pdf}{0.24\linewidth}{J11h43m39.8s+07d00m12.6s}}
\gridline{\fig{lcs/J11h45m28.5s-37d39m31.5s_lc_fit.pdf}{0.24\linewidth}{J11h45m28.5s$-$37d39m31.5s}
	\fig{lcs/J11h46m46.0s-46d05m30.8s_lc_fit.pdf}{0.24\linewidth}{J11h46m46.0s$-$46d05m30.8s}
	\fig{lcs/J11h49m36.2s-34d25m04.6s_lc_fit.pdf}{0.24\linewidth}{J11h49m36.2s$-$34d25m04.6s}
	\fig{lcs/J11h49m40.0s-37d54m34.2s_lc_fit.pdf}{0.24\linewidth}{J11h49m40.0s$-$37d54m34.2s}}
\gridline{\fig{lcs/J11h50m29.4s-33d57m16.2s_lc_fit.pdf}{0.24\linewidth}{J11h50m29.4s$-$33d57m16.2s}
	\fig{lcs/J11h54m58.5s-51d44m03.6s_lc_fit.pdf}{0.24\linewidth}{J11h54m58.5s$-$51d44m03.6s}
	\fig{lcs/J12h08m37.3s-41d05m14.1s_lc_fit.pdf}{0.24\linewidth}{J12h08m37.3s$-$41d05m14.1s}
	\fig{lcs/J12h13m11.9s+03d50m44.9s_lc_fit.pdf}{0.24\linewidth}{J12h13m11.9s+03d50m44.9s}}
\gridline{\fig{lcs/J12h13m35.5s-50d31m42.7s_lc_fit.pdf}{0.24\linewidth}{J12h13m35.5s$-$50d31m42.7s}
	\fig{lcs/J12h17m01.5s-51d01m01.6s_lc_fit.pdf}{0.24\linewidth}{J12h17m01.5s$-$51d01m01.6s}
	\fig{lcs/J12h17m58.4s-36d34m17.6s_lc_fit.pdf}{0.24\linewidth}{J12h17m58.4s$-$36d34m17.6s}
	\fig{lcs/J12h18m35.0s-01d19m53.2s_lc_fit.pdf}{0.24\linewidth}{J12h18m35.0s$-$01d19m53.2s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_5}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J12h50m02.7s-50d41m48.7s_lc_fit.pdf}{0.24\linewidth}{J12h50m02.7s$-$50d41m48.7s}
	\fig{lcs/J12h50m22.8s-44d32m03.2s_lc_fit.pdf}{0.24\linewidth}{J12h50m22.8s$-$44d32m03.2s}
	\fig{lcs/J12h50m51.8s-49d47m32.9s_lc_fit.pdf}{0.24\linewidth}{J12h50m51.8s$-$49d47m32.9s}
	\fig{lcs/J12h57m10.4s-46d37m40.8s_lc_fit.pdf}{0.24\linewidth}{J12h57m10.4s$-$46d37m40.8s}}
\gridline{\fig{lcs/J13h00m13.3s-50d11m53.0s_lc_fit.pdf}{0.24\linewidth}{J13h00m13.3s$-$50d11m53.0s}
	\fig{lcs/J13h00m23.0s-42d08m39.3s_lc_fit.pdf}{0.24\linewidth}{J13h00m23.0s$-$42d08m39.3s}
	\fig{lcs/J13h02m45.2s-43d08m55.9s_lc_fit.pdf}{0.24\linewidth}{J13h02m45.2s$-$43d08m55.9s}
	\fig{lcs/J13h08m26.8s-35d45m57.2s_lc_fit.pdf}{0.24\linewidth}{J13h08m26.8s$-$35d45m57.2s}}
\gridline{\fig{lcs/J13h11m26.9s-31d00m36.2s_lc_fit.pdf}{0.24\linewidth}{J13h11m26.9s$-$31d00m36.2s}
	\fig{lcs/J13h15m37.8s-47d34m57.5s_lc_fit.pdf}{0.24\linewidth}{J13h15m37.8s$-$47d34m57.5s}
	\fig{lcs/J13h23m43.8s-51d42m22.7s_lc_fit.pdf}{0.24\linewidth}{J13h23m43.8s$-$51d42m22.7s}
	\fig{lcs/J13h24m42.8s-50d20m37.8s_lc_fit.pdf}{0.24\linewidth}{J13h24m42.8s$-$50d20m37.8s}}
\gridline{\fig{lcs/J13h24m50.9s-06d39m40.8s_lc_fit.pdf}{0.24\linewidth}{J13h24m50.9s$-$06d39m40.8s}
	\fig{lcs/J13h31m00.3s-38d09m28.0s_lc_fit.pdf}{0.24\linewidth}{J13h31m00.3s$-$38d09m28.0s}
	\fig{lcs/J13h31m07.7s-53d09m57.4s_lc_fit.pdf}{0.24\linewidth}{J13h31m07.7s$-$53d09m57.4s}
	\fig{lcs/J13h32m22.0s-52d16m39.0s_lc_fit.pdf}{0.24\linewidth}{J13h32m22.0s$-$52d16m39.0s}}
\gridline{\fig{lcs/J13h32m32.8s-47d28m30.0s_lc_fit.pdf}{0.24\linewidth}{J13h32m32.8s$-$47d28m30.0s}
	\fig{lcs/J13h36m03.2s-51d36m00.0s_lc_fit.pdf}{0.24\linewidth}{J13h36m03.2s$-$51d36m00.0s}
	\fig{lcs/J13h37m56.4s-50d55m40.7s_lc_fit.pdf}{0.24\linewidth}{J13h37m56.4s$-$50d55m40.7s}
	\fig{lcs/J13h41m17.8s-49d03m36.8s_lc_fit.pdf}{0.24\linewidth}{J13h41m17.8s$-$49d03m36.8s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_6}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J13h42m36.4s-50d39m12.9s_lc_fit.pdf}{0.24\linewidth}{J13h42m36.4s$-$50d39m12.9s}
	\fig{lcs/J13h48m31.0s-30d35m36.2s_lc_fit.pdf}{0.24\linewidth}{J13h48m31.0s$-$30d35m36.2s}
	\fig{lcs/J13h49m22.2s+07d12m17.6s_lc_fit.pdf}{0.24\linewidth}{J13h49m22.2s+07d12m17.6s}
	\fig{lcs/J13h49m46.1s+09d08m16.3s_lc_fit.pdf}{0.24\linewidth}{J13h49m46.1s+09d08m16.3s}}
\gridline{\fig{lcs/J13h57m39.4s-45d20m29.1s_lc_fit.pdf}{0.24\linewidth}{J13h57m39.4s$-$45d20m29.1s}
	\fig{lcs/J14h06m02.1s-43d48m23.3s_lc_fit.pdf}{0.24\linewidth}{J14h06m02.1s$-$43d48m23.3s}
	\fig{lcs/J14h15m24.4s-42d49m12.2s_lc_fit.pdf}{0.24\linewidth}{J14h15m24.4s$-$42d49m12.2s}
	\fig{lcs/J14h19m04.9s-09d00m45.5s_lc_fit.pdf}{0.24\linewidth}{J14h19m04.9s$-$09d00m45.5s}}
\gridline{\fig{lcs/J14h19m45.9s-08d27m06.4s_lc_fit.pdf}{0.24\linewidth}{J14h19m45.9s$-$08d27m06.4s}
	\fig{lcs/J14h22m25.1s+07d01m58.1s_lc_fit.pdf}{0.24\linewidth}{J14h22m25.1s+07d01m58.1s}
	\fig{lcs/J14h34m52.7s-00d28m28.4s_lc_fit.pdf}{0.24\linewidth}{J14h34m52.7s$-$00d28m28.4s}
	\fig{lcs/J15h06m37.4s+00d25m40.4s_lc_fit.pdf}{0.24\linewidth}{J15h06m37.4s+00d25m40.4s}}
\gridline{\fig{lcs/J15h13m31.7s-09d19m19.6s_lc_fit.pdf}{0.24\linewidth}{J15h13m31.7s$-$09d19m19.6s}
	\fig{lcs/J15h14m46.8s+01d51m27.8s_lc_fit.pdf}{0.24\linewidth}{J15h14m46.8s+01d51m27.8s}
	\fig{lcs/J15h17m38.6s+03d45m28.3s_lc_fit.pdf}{0.24\linewidth}{J15h17m38.6s+03d45m28.3s}
	\fig{lcs/J15h19m51.3s-09d18m48.8s_lc_fit.pdf}{0.24\linewidth}{J15h19m51.3s$-$09d18m48.8s}}
\gridline{\fig{lcs/J15h24m45.4s-01d37m40.3s_lc_fit.pdf}{0.24\linewidth}{J15h24m45.4s$-$01d37m40.3s}
	\fig{lcs/J15h26m59.3s+06d33m48.5s_lc_fit.pdf}{0.24\linewidth}{J15h26m59.3s+06d33m48.5s}
	\fig{lcs/J15h29m14.4s-04d14m07.6s_lc_fit.pdf}{0.24\linewidth}{J15h29m14.4s$-$04d14m07.6s}
	\fig{lcs/J15h42m36.1s-05d47m55.4s_lc_fit.pdf}{0.24\linewidth}{J15h42m36.1s$-$05d47m55.4s}}
\end{figure*}
\begin{figure*}
\gridline{\fig{lcs/J15h42m44.0s+01d14m57.6s_lc_fit.pdf}{0.24\linewidth}{J15h42m44.0s+01d14m57.6s}
	\fig{lcs/J15h43m39.8s+08d06m12.8s_lc_fit.pdf}{0.24\linewidth}{J15h43m39.8s+08d06m12.8s}
	\fig{lcs/J15h49m08.8s-01d16m27.9s_lc_fit.pdf}{0.24\linewidth}{J15h49m08.8s$-$01d16m27.9s}
	\fig{lcs/J15h49m40.2s+01d06m01.6s_lc_fit.pdf}{0.24\linewidth}{J15h49m40.2s+01d06m01.6s}}
\gridline{\fig{lcs/J16h02m20.5s-04d25m36.5s_lc_fit.pdf}{0.24\linewidth}{J16h02m20.5s$-$04d25m36.5s}
	\fig{lcs/J16h03m14.9s+08d10m20.3s_lc_fit.pdf}{0.24\linewidth}{J16h03m14.9s+08d10m20.3s}
	\fig{lcs/J16h05m56.9s-01d09m49.3s_lc_fit.pdf}{0.24\linewidth}{J16h05m56.9s$-$01d09m49.3s}
	\fig{lcs/J16h06m06.9s+06d19m48.8s_lc_fit.pdf}{0.24\linewidth}{J16h06m06.9s+06d19m48.8s}}
\gridline{\fig{lcs/J16h08m56.1s+09d10m38.5s_lc_fit.pdf}{0.24\linewidth}{J16h08m56.1s+09d10m38.5s}
	\fig{lcs/J16h10m11.9s-03d49m17.1s_lc_fit.pdf}{0.24\linewidth}{J16h10m11.9s$-$03d49m17.1s}
	\fig{lcs/J16h10m12.4s-00d11m41.6s_lc_fit.pdf}{0.24\linewidth}{J16h10m12.4s$-$00d11m41.6s}
	\fig{lcs/J16h11m31.8s-03d40m58.3s_lc_fit.pdf}{0.24\linewidth}{J16h11m31.8s$-$03d40m58.3s}}
\gridline{\fig{lcs/J16h17m26.3s+06d32m32.5s_lc_fit.pdf}{0.24\linewidth}{J16h17m26.3s+06d32m32.5s}
	\fig{lcs/J16h17m52.7s-06d05m11.5s_lc_fit.pdf}{0.24\linewidth}{J16h17m52.7s$-$06d05m11.5s}
	\fig{lcs/J16h18m23.7s-06d03m26.3s_lc_fit.pdf}{0.24\linewidth}{J16h18m23.7s$-$06d03m26.3s}
	\fig{lcs/J16h18m46.7s+04d40m06.7s_lc_fit.pdf}{0.24\linewidth}{J16h18m46.7s+04d40m06.7s}}
\gridline{\fig{lcs/J16h22m23.7s+00d13m28.7s_lc_fit.pdf}{0.24\linewidth}{J16h22m23.7s+00d13m28.7s}
	\fig{lcs/J16h23m46.0s-08d35m38.4s_lc_fit.pdf}{0.24\linewidth}{J16h23m46.0s$-$08d35m38.4s}
	\fig{lcs/J16h25m20.4s+05d56m40.9s_lc_fit.pdf}{0.24\linewidth}{J16h25m20.4s+05d56m40.9s}
	\fig{lcs/J16h27m12.9s+04d18m34.6s_lc_fit.pdf}{0.24\linewidth}{J16h27m12.9s+04d18m34.6s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_7}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J16h27m47.9s-09d01m06.4s_lc_fit.pdf}{0.24\linewidth}{J16h27m47.9s$-$09d01m06.4s}
	\fig{lcs/J16h30m07.9s-04d51m35.9s_lc_fit.pdf}{0.24\linewidth}{J16h30m07.9s$-$04d51m35.9s}
	\fig{lcs/J16h30m51.5s-08d10m09.0s_lc_fit.pdf}{0.24\linewidth}{J16h30m51.5s$-$08d10m09.0s}
	\fig{lcs/J16h31m55.3s-08d30m08.2s_lc_fit.pdf}{0.24\linewidth}{J16h31m55.3s$-$08d30m08.2s}}
\gridline{\fig{lcs/J16h36m41.6s+09d24m58.0s_lc_fit.pdf}{0.24\linewidth}{J16h36m41.6s+09d24m58.0s}
	\fig{lcs/J16h37m50.2s+02d11m44.0s_lc_fit.pdf}{0.24\linewidth}{J16h37m50.2s+02d11m44.0s}
	\fig{lcs/J16h39m39.0s+09d07m36.5s_lc_fit.pdf}{0.24\linewidth}{J16h39m39.0s+09d07m36.5s}
	\fig{lcs/J16h39m51.1s+01d16m50.4s_lc_fit.pdf}{0.24\linewidth}{J16h39m51.1s+01d16m50.4s}}
\gridline{\fig{lcs/J16h40m43.3s-01d33m41.5s_lc_fit.pdf}{0.24\linewidth}{J16h40m43.3s$-$01d33m41.5s}
	\fig{lcs/J16h41m00.2s+05d58m10.6s_lc_fit.pdf}{0.24\linewidth}{J16h41m00.2s+05d58m10.6s}
	\fig{lcs/J16h43m51.8s+08d55m05.9s_lc_fit.pdf}{0.24\linewidth}{J16h43m51.8s+08d55m05.9s}
	\fig{lcs/J16h44m05.3s+02d14m08.8s_lc_fit.pdf}{0.24\linewidth}{J16h44m05.3s+02d14m08.8s}}
\gridline{\fig{lcs/J16h46m13.0s+05d17m50.1s_lc_fit.pdf}{0.24\linewidth}{J16h46m13.0s+05d17m50.1s}
	\fig{lcs/J16h49m18.4s+09d21m43.7s_lc_fit.pdf}{0.24\linewidth}{J16h49m18.4s+09d21m43.7s}
	\fig{lcs/J16h49m58.4s-04d48m47.2s_lc_fit.pdf}{0.24\linewidth}{J16h49m58.4s$-$04d48m47.2s}
	\fig{lcs/J16h51m07.1s+01d24m06.2s_lc_fit.pdf}{0.24\linewidth}{J16h51m07.1s+01d24m06.2s}}
\gridline{\fig{lcs/J16h52m06.0s+05d22m24.1s_lc_fit.pdf}{0.24\linewidth}{J16h52m06.0s+05d22m24.1s}
	\fig{lcs/J16h52m37.3s+01d00m16.3s_lc_fit.pdf}{0.24\linewidth}{J16h52m37.3s+01d00m16.3s}
	\fig{lcs/J16h56m00.0s-00d30m29.2s_lc_fit.pdf}{0.24\linewidth}{J16h56m00.0s$-$00d30m29.2s}
	\fig{lcs/J16h57m14.4s+02d30m55.7s_lc_fit.pdf}{0.24\linewidth}{J16h57m14.4s+02d30m55.7s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_8}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J16h58m44.7s+08d19m05.6s_lc_fit.pdf}{0.24\linewidth}{J16h58m44.7s+08d19m05.6s}
	\fig{lcs/J16h59m10.9s-07d37m10.2s_lc_fit.pdf}{0.24\linewidth}{J16h59m10.9s$-$07d37m10.2s}
	\fig{lcs/J16h59m22.1s-00d39m58.5s_lc_fit.pdf}{0.24\linewidth}{J16h59m22.1s$-$00d39m58.5s}
	\fig{lcs/J17h00m23.9s+05d22m43.9s_lc_fit.pdf}{0.24\linewidth}{J17h00m23.9s+05d22m43.9s}}
\gridline{\fig{lcs/J17h01m24.9s-06d31m33.5s_lc_fit.pdf}{0.24\linewidth}{J17h01m24.9s$-$06d31m33.5s}
	\fig{lcs/J17h02m07.7s-07d46m45.8s_lc_fit.pdf}{0.24\linewidth}{J17h02m07.7s$-$07d46m45.8s}
	\fig{lcs/J17h02m19.4s-03d38m58.1s_lc_fit.pdf}{0.24\linewidth}{J17h02m19.4s$-$03d38m58.1s}
	\fig{lcs/J17h02m33.2s-03d28m03.5s_lc_fit.pdf}{0.24\linewidth}{J17h02m33.2s$-$03d28m03.5s}}
\gridline{\fig{lcs/J17h04m29.0s+04d20m34.7s_lc_fit.pdf}{0.24\linewidth}{J17h04m29.0s+04d20m34.7s}
	\fig{lcs/J17h04m33.6s-08d55m52.2s_lc_fit.pdf}{0.24\linewidth}{J17h04m33.6s$-$08d55m52.2s}
	\fig{lcs/J17h05m43.5s+08d27m27.5s_lc_fit.pdf}{0.24\linewidth}{J17h05m43.5s+08d27m27.5s}
	\fig{lcs/J17h06m45.8s+00d51m56.1s_lc_fit.pdf}{0.24\linewidth}{J17h06m45.8s+00d51m56.1s}}
\gridline{\fig{lcs/J17h06m46.5s+06d17m14.2s_lc_fit.pdf}{0.24\linewidth}{J17h06m46.5s+06d17m14.2s}
	\fig{lcs/J17h07m15.7s-01d35m02.6s_lc_fit.pdf}{0.24\linewidth}{J17h07m15.7s$-$01d35m02.6s}
	\fig{lcs/J17h07m24.3s-02d17m51.5s_lc_fit.pdf}{0.24\linewidth}{J17h07m24.3s$-$02d17m51.5s}
	\fig{lcs/J17h07m51.3s-05d12m37.9s_lc_fit.pdf}{0.24\linewidth}{J17h07m51.3s$-$05d12m37.9s}}
\gridline{\fig{lcs/J17h09m31.9s-01d49m16.9s_lc_fit.pdf}{0.24\linewidth}{J17h09m31.9s$-$01d49m16.9s}
	\fig{lcs/J17h11m11.6s+08d23m17.5s_lc_fit.pdf}{0.24\linewidth}{J17h11m11.6s+08d23m17.5s}
	\fig{lcs/J17h11m30.9s+09d21m27.7s_lc_fit.pdf}{0.24\linewidth}{J17h11m30.9s+09d21m27.7s}
	\fig{lcs/J17h12m08.0s+05d39m32.2s_lc_fit.pdf}{0.24\linewidth}{J17h12m08.0s+05d39m32.2s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_9}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J17h12m44.0s+05d23m59.7s_lc_fit.pdf}{0.24\linewidth}{J17h12m44.0s+05d23m59.7s}
	\fig{lcs/J17h12m58.3s+01d01m59.8s_lc_fit.pdf}{0.24\linewidth}{J17h12m58.3s+01d01m59.8s}
	\fig{lcs/J17h14m09.6s+03d33m20.7s_lc_fit.pdf}{0.24\linewidth}{J17h14m09.6s+03d33m20.7s}
	\fig{lcs/J17h14m40.6s+05d12m38.1s_lc_fit.pdf}{0.24\linewidth}{J17h14m40.6s+05d12m38.1s}}
\gridline{\fig{lcs/J17h16m06.7s+07d08m47.2s_lc_fit.pdf}{0.24\linewidth}{J17h16m06.7s+07d08m47.2s}
	\fig{lcs/J17h16m19.2s+01d33m06.6s_lc_fit.pdf}{0.24\linewidth}{J17h16m19.2s+01d33m06.6s}
	\fig{lcs/J17h16m40.5s-07d11m21.7s_lc_fit.pdf}{0.24\linewidth}{J17h16m40.5s$-$07d11m21.7s}
	\fig{lcs/J17h19m14.2s+02d15m56.3s_lc_fit.pdf}{0.24\linewidth}{J17h19m14.2s+02d15m56.3s}}
\gridline{\fig{lcs/J17h21m35.0s+05d49m09.3s_lc_fit.pdf}{0.24\linewidth}{J17h21m35.0s+05d49m09.3s}
	\fig{lcs/J17h24m17.6s+08d33m46.1s_lc_fit.pdf}{0.24\linewidth}{J17h24m17.6s+08d33m46.1s}
	\fig{lcs/J17h25m56.5s+00d30m47.0s_lc_fit.pdf}{0.24\linewidth}{J17h25m56.5s+00d30m47.0s}
	\fig{lcs/J17h26m23.7s+04d23m57.5s_lc_fit.pdf}{0.24\linewidth}{J17h26m23.7s+04d23m57.5s}}
\gridline{\fig{lcs/J17h29m45.4s+04d16m12.5s_lc_fit.pdf}{0.24\linewidth}{J17h29m45.4s+04d16m12.5s}
	\fig{lcs/J17h31m49.6s+02d21m35.3s_lc_fit.pdf}{0.24\linewidth}{J17h31m49.6s+02d21m35.3s}
	\fig{lcs/J17h32m53.0s+08d58m29.8s_lc_fit.pdf}{0.24\linewidth}{J17h32m53.0s+08d58m29.8s}
	\fig{lcs/J17h33m24.4s+09d21m41.7s_lc_fit.pdf}{0.24\linewidth}{J17h33m24.4s+09d21m41.7s}}
\gridline{\fig{lcs/J17h34m00.5s-03d38m11.0s_lc_fit.pdf}{0.24\linewidth}{J17h34m00.5s$-$03d38m11.0s}
	\fig{lcs/J17h34m45.7s+02d01m46.0s_lc_fit.pdf}{0.24\linewidth}{J17h34m45.7s+02d01m46.0s}
	\fig{lcs/J17h35m00.8s-07d33m20.7s_lc_fit.pdf}{0.24\linewidth}{J17h35m00.8s$-$07d33m20.7s}
	\fig{lcs/J17h36m54.7s-07d31m33.0s_lc_fit.pdf}{0.24\linewidth}{J17h36m54.7s$-$07d31m33.0s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_10}
\caption{Light curves of the ESE candidates in the VAST sample.}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J17h37m09.8s+09d28m03.9s_lc_fit.pdf}{0.24\linewidth}{J17h37m09.8s+09d28m03.9s}
	\fig{lcs/J17h38m16.0s+01d25m39.1s_lc_fit.pdf}{0.24\linewidth}{J17h38m16.0s+01d25m39.1s}
	\fig{lcs/J17h39m33.1s-03d47m55.5s_lc_fit.pdf}{0.24\linewidth}{J17h39m33.1s$-$03d47m55.5s}
	\fig{lcs/J17h39m42.2s+00d10m18.2s_lc_fit.pdf}{0.24\linewidth}{J17h39m42.2s+00d10m18.2s}}
\gridline{\fig{lcs/J17h39m50.6s+03d18m09.8s_lc_fit.pdf}{0.24\linewidth}{J17h39m50.6s+03d18m09.8s}
	\fig{lcs/J17h40m54.7s+07d51m01.9s_lc_fit.pdf}{0.24\linewidth}{J17h40m54.7s+07d51m01.9s}
	\fig{lcs/J17h41m47.8s+01d33m00.1s_lc_fit.pdf}{0.24\linewidth}{J17h41m47.8s+01d33m00.1s}
	\fig{lcs/J17h43m49.3s+06d10m31.1s_lc_fit.pdf}{0.24\linewidth}{J17h43m49.3s+06d10m31.1s}}
\gridline{\fig{lcs/J17h44m30.9s+01d43m21.0s_lc_fit.pdf}{0.24\linewidth}{J17h44m30.9s+01d43m21.0s}
	\fig{lcs/J17h45m31.1s+03d48m03.7s_lc_fit.pdf}{0.24\linewidth}{J17h45m31.1s+03d48m03.7s}
	\fig{lcs/J17h51m48.9s+08d05m25.3s_lc_fit.pdf}{0.24\linewidth}{J17h51m48.9s+08d05m25.3s}
	\fig{lcs/J17h51m57.0s+00d22m19.8s_lc_fit.pdf}{0.24\linewidth}{J17h51m57.0s+00d22m19.8s}}
\gridline{\fig{lcs/J17h54m43.5s+06d46m43.2s_lc_fit.pdf}{0.24\linewidth}{J17h54m43.5s+06d46m43.2s}
	\fig{lcs/J17h55m56.8s+00d34m41.1s_lc_fit.pdf}{0.24\linewidth}{J17h55m56.8s+00d34m41.1s}
	\fig{lcs/J17h57m09.8s+08d56m28.5s_lc_fit.pdf}{0.24\linewidth}{J17h57m09.8s+08d56m28.5s}
	\fig{lcs/J17h57m13.1s+01d02m42.2s_lc_fit.pdf}{0.24\linewidth}{J17h57m13.1s+01d02m42.2s}}
\gridline{\fig{lcs/J17h57m36.1s+03d19m38.8s_lc_fit.pdf}{0.24\linewidth}{J17h57m36.1s+03d19m38.8s}
	\fig{lcs/J17h57m42.7s-01d35m51.9s_lc_fit.pdf}{0.24\linewidth}{J17h57m42.7s$-$01d35m51.9s}
	\fig{lcs/J18h00m06.4s+01d49m41.2s_lc_fit.pdf}{0.24\linewidth}{J18h00m06.4s+01d49m41.2s}
	\fig{lcs/J18h00m44.3s+04d31m59.0s_lc_fit.pdf}{0.24\linewidth}{J18h00m44.3s+04d31m59.0s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_11}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J18h00m51.8s+08d31m29.8s_lc_fit.pdf}{0.24\linewidth}{J18h00m51.8s+08d31m29.8s}
	\fig{lcs/J18h03m47.2s-01d16m26.4s_lc_fit.pdf}{0.24\linewidth}{J18h03m47.2s$-$01d16m26.4s}
	\fig{lcs/J18h04m02.3s-00d35m51.0s_lc_fit.pdf}{0.24\linewidth}{J18h04m02.3s$-$00d35m51.0s}
	\fig{lcs/J18h04m30.7s+08d58m57.3s_lc_fit.pdf}{0.24\linewidth}{J18h04m30.7s+08d58m57.3s}}
\gridline{\fig{lcs/J18h09m28.5s+01d14m04.5s_lc_fit.pdf}{0.24\linewidth}{J18h09m28.5s+01d14m04.5s}
	\fig{lcs/J18h15m23.7s+04d49m21.1s_lc_fit.pdf}{0.24\linewidth}{J18h15m23.7s+04d49m21.1s}
	\fig{lcs/J18h26m44.5s+09d04m06.0s_lc_fit.pdf}{0.24\linewidth}{J18h26m44.5s+09d04m06.0s}
	\fig{lcs/J18h29m41.0s+03d55m32.7s_lc_fit.pdf}{0.24\linewidth}{J18h29m41.0s+03d55m32.7s}}
\gridline{\fig{lcs/J18h32m20.5s+05d36m48.2s_lc_fit.pdf}{0.24\linewidth}{J18h32m20.5s+05d36m48.2s}
	\fig{lcs/J18h37m04.1s+09d09m24.1s_lc_fit.pdf}{0.24\linewidth}{J18h37m04.1s+09d09m24.1s}
	\fig{lcs/J19h07m10.6s-03d46m43.0s_lc_fit.pdf}{0.24\linewidth}{J19h07m10.6s$-$03d46m43.0s}
	\fig{lcs/J19h08m55.9s-05d05m27.6s_lc_fit.pdf}{0.24\linewidth}{J19h08m55.9s$-$05d05m27.6s}}
\gridline{\fig{lcs/J19h15m33.4s-05d11m09.1s_lc_fit.pdf}{0.24\linewidth}{J19h15m33.4s$-$05d11m09.1s}
	\fig{lcs/J19h17m57.7s-08d26m51.1s_lc_fit.pdf}{0.24\linewidth}{J19h17m57.7s$-$08d26m51.1s}
	\fig{lcs/J19h19m34.4s-07d40m43.2s_lc_fit.pdf}{0.24\linewidth}{J19h19m34.4s$-$07d40m43.2s}
	\fig{lcs/J19h19m59.0s-07d57m25.7s_lc_fit.pdf}{0.24\linewidth}{J19h19m59.0s$-$07d57m25.7s}}
\gridline{\fig{lcs/J19h20m25.0s-05d19m43.2s_lc_fit.pdf}{0.24\linewidth}{J19h20m25.0s$-$05d19m43.2s}
	\fig{lcs/J19h21m20.0s-05d34m32.1s_lc_fit.pdf}{0.24\linewidth}{J19h21m20.0s$-$05d34m32.1s}
	\fig{lcs/J19h27m55.8s+06d42m49.0s_lc_fit.pdf}{0.24\linewidth}{J19h27m55.8s+06d42m49.0s}
	\fig{lcs/J19h28m33.2s-01d10m46.7s_lc_fit.pdf}{0.24\linewidth}{J19h28m33.2s$-$01d10m46.7s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_12}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J19h28m34.3s+06d49m06.8s_lc_fit.pdf}{0.24\linewidth}{J19h28m34.3s+06d49m06.8s}
	\fig{lcs/J19h31m55.5s-00d45m37.0s_lc_fit.pdf}{0.24\linewidth}{J19h31m55.5s$-$00d45m37.0s}
	\fig{lcs/J19h33m16.7s-08d22m39.7s_lc_fit.pdf}{0.24\linewidth}{J19h33m16.7s$-$08d22m39.7s}
	\fig{lcs/J19h34m46.2s-05d29m02.8s_lc_fit.pdf}{0.24\linewidth}{J19h34m46.2s$-$05d29m02.8s}}
\gridline{\fig{lcs/J19h35m03.6s-01d11m06.2s_lc_fit.pdf}{0.24\linewidth}{J19h35m03.6s$-$01d11m06.2s}
	\fig{lcs/J19h35m45.2s+04d14m19.8s_lc_fit.pdf}{0.24\linewidth}{J19h35m45.2s+04d14m19.8s}
	\fig{lcs/J19h36m37.5s-06d17m34.0s_lc_fit.pdf}{0.24\linewidth}{J19h36m37.5s$-$06d17m34.0s}
	\fig{lcs/J19h39m07.0s-04d11m46.1s_lc_fit.pdf}{0.24\linewidth}{J19h39m07.0s$-$04d11m46.1s}}
\gridline{\fig{lcs/J19h41m32.9s-08d16m54.5s_lc_fit.pdf}{0.24\linewidth}{J19h41m32.9s$-$08d16m54.5s}
	\fig{lcs/J19h44m44.6s+07d43m02.5s_lc_fit.pdf}{0.24\linewidth}{J19h44m44.6s+07d43m02.5s}
	\fig{lcs/J19h46m52.3s-05d09m41.2s_lc_fit.pdf}{0.24\linewidth}{J19h46m52.3s$-$05d09m41.2s}
	\fig{lcs/J19h47m51.6s+04d22m15.8s_lc_fit.pdf}{0.24\linewidth}{J19h47m51.6s+04d22m15.8s}}
\gridline{\fig{lcs/J19h49m34.5s+07d08m33.6s_lc_fit.pdf}{0.24\linewidth}{J19h49m34.5s+07d08m33.6s}
	\fig{lcs/J19h50m06.8s-07d16m42.7s_lc_fit.pdf}{0.24\linewidth}{J19h50m06.8s$-$07d16m42.7s}
	\fig{lcs/J19h50m55.8s+02d00m43.2s_lc_fit.pdf}{0.24\linewidth}{J19h50m55.8s+02d00m43.2s}
	\fig{lcs/J19h51m11.1s+06d03m18.5s_lc_fit.pdf}{0.24\linewidth}{J19h51m11.1s+06d03m18.5s}}
\gridline{\fig{lcs/J19h52m17.6s-45d28m19.3s_lc_fit.pdf}{0.24\linewidth}{J19h52m17.6s$-$45d28m19.3s}
	\fig{lcs/J19h52m35.6s-06d57m06.7s_lc_fit.pdf}{0.24\linewidth}{J19h52m35.6s$-$06d57m06.7s}
	\fig{lcs/J19h53m41.4s+09d17m39.1s_lc_fit.pdf}{0.24\linewidth}{J19h53m41.4s+09d17m39.1s}
	\fig{lcs/J19h53m44.9s-55d56m10.7s_lc_fit.pdf}{0.24\linewidth}{J19h53m44.9s$-$55d56m10.7s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_13}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J19h54m57.9s-08d40m28.6s_lc_fit.pdf}{0.24\linewidth}{J19h54m57.9s$-$08d40m28.6s}
	\fig{lcs/J19h56m06.7s+07d36m33.3s_lc_fit.pdf}{0.24\linewidth}{J19h56m06.7s+07d36m33.3s}
	\fig{lcs/J19h58m18.1s+06d30m13.6s_lc_fit.pdf}{0.24\linewidth}{J19h58m18.1s+06d30m13.6s}
	\fig{lcs/J19h59m09.1s-08d16m23.2s_lc_fit.pdf}{0.24\linewidth}{J19h59m09.1s$-$08d16m23.2s}}
\gridline{\fig{lcs/J20h01m50.2s-06d19m43.4s_lc_fit.pdf}{0.24\linewidth}{J20h01m50.2s$-$06d19m43.4s}
	\fig{lcs/J20h02m42.9s-08d25m38.1s_lc_fit.pdf}{0.24\linewidth}{J20h02m42.9s$-$08d25m38.1s}
	\fig{lcs/J20h03m41.5s-31d29m52.2s_lc_fit.pdf}{0.24\linewidth}{J20h03m41.5s$-$31d29m52.2s}
	\fig{lcs/J20h04m56.5s-31d09m50.8s_lc_fit.pdf}{0.24\linewidth}{J20h04m56.5s$-$31d09m50.8s}}
\gridline{\fig{lcs/J20h05m44.9s-34d15m15.7s_lc_fit.pdf}{0.24\linewidth}{J20h05m44.9s$-$34d15m15.7s}
	\fig{lcs/J20h10m56.9s-00d34m26.6s_lc_fit.pdf}{0.24\linewidth}{J20h10m56.9s$-$00d34m26.6s}
	\fig{lcs/J20h11m12.8s+07d13m32.4s_lc_fit.pdf}{0.24\linewidth}{J20h11m12.8s+07d13m32.4s}
	\fig{lcs/J20h11m33.7s-33d58m57.3s_lc_fit.pdf}{0.24\linewidth}{J20h11m33.7s$-$33d58m57.3s}}
\gridline{\fig{lcs/J20h12m26.5s-30d39m46.4s_lc_fit.pdf}{0.24\linewidth}{J20h12m26.5s$-$30d39m46.4s}
	\fig{lcs/J20h13m26.5s-04d50m58.4s_lc_fit.pdf}{0.24\linewidth}{J20h13m26.5s$-$04d50m58.4s}
	\fig{lcs/J20h14m22.1s-07d57m01.6s_lc_fit.pdf}{0.24\linewidth}{J20h14m22.1s$-$07d57m01.6s}
	\fig{lcs/J20h19m31.1s+05d41m40.9s_lc_fit.pdf}{0.24\linewidth}{J20h19m31.1s+05d41m40.9s}}
\gridline{\fig{lcs/J20h20m49.5s-28d48m22.5s_lc_fit.pdf}{0.24\linewidth}{J20h20m49.5s$-$28d48m22.5s}
	\fig{lcs/J20h21m08.8s-35d55m27.3s_lc_fit.pdf}{0.24\linewidth}{J20h21m08.8s$-$35d55m27.3s}
	\fig{lcs/J20h26m49.5s+04d59m56.8s_lc_fit.pdf}{0.24\linewidth}{J20h26m49.5s+04d59m56.8s}
	\fig{lcs/J20h28m40.7s-30d56m10.4s_lc_fit.pdf}{0.24\linewidth}{J20h28m40.7s$-$30d56m10.4s}}
\end{figure*}
\begin{figure*}
\label{fig:ese_lcs_14}
\caption{Light curves of the ESE candidates in the VAST sample.}
\gridline{\fig{lcs/J20h33m10.5s-44d44m52.8s_lc_fit.pdf}{0.24\linewidth}{J20h33m10.5s$-$44d44m52.8s}
	\fig{lcs/J20h33m13.7s-44d23m23.8s_lc_fit.pdf}{0.24\linewidth}{J20h33m13.7s$-$44d23m23.8s}
	\fig{lcs/J20h35m05.4s-07d11m30.8s_lc_fit.pdf}{0.24\linewidth}{J20h35m05.4s$-$07d11m30.8s}
	\fig{lcs/J20h35m15.8s-29d03m40.0s_lc_fit.pdf}{0.24\linewidth}{J20h35m15.8s$-$29d03m40.0s}}
\gridline{\fig{lcs/J20h36m29.2s-05d13m03.6s_lc_fit.pdf}{0.24\linewidth}{J20h36m29.2s$-$05d13m03.6s}
	\fig{lcs/J20h39m09.1s-30d45m20.7s_lc_fit.pdf}{0.24\linewidth}{J20h39m09.1s$-$30d45m20.7s}
	\fig{lcs/J20h48m47.1s-43d59m33.1s_lc_fit.pdf}{0.24\linewidth}{J20h48m47.1s$-$43d59m33.1s}
	\fig{lcs/J20h51m55.8s-36d55m22.5s_lc_fit.pdf}{0.24\linewidth}{J20h51m55.8s$-$36d55m22.5s}}
\gridline{\fig{lcs/J20h56m55.7s+00d20m31.9s_lc_fit.pdf}{0.24\linewidth}{J20h56m55.7s+00d20m31.9s}
	\fig{lcs/J21h02m49.3s-48d38m04.3s_lc_fit.pdf}{0.24\linewidth}{J21h02m49.3s$-$48d38m04.3s}
	\fig{lcs/J21h14m29.8s-00d52m17.6s_lc_fit.pdf}{0.24\linewidth}{J21h14m29.8s$-$00d52m17.6s}
	\fig{lcs/J21h16m03.2s-07d53m23.0s_lc_fit.pdf}{0.24\linewidth}{J21h16m03.2s$-$07d53m23.0s}}
\gridline{\fig{lcs/J21h16m11.4s+01d18m12.9s_lc_fit.pdf}{0.24\linewidth}{J21h16m11.4s+01d18m12.9s}
	\fig{lcs/J21h17m25.0s-00d34m52.9s_lc_fit.pdf}{0.24\linewidth}{J21h17m25.0s$-$00d34m52.9s}
	\fig{lcs/J21h17m51.1s-09d19m08.8s_lc_fit.pdf}{0.24\linewidth}{J21h17m51.1s$-$09d19m08.8s}
	\fig{lcs/J21h19m14.3s-35d52m38.9s_lc_fit.pdf}{0.24\linewidth}{J21h19m14.3s$-$35d52m38.9s}}
\gridline{\fig{lcs/J21h25m06.8s-05d36m39.2s_lc_fit.pdf}{0.24\linewidth}{J21h25m06.8s$-$05d36m39.2s}
	\fig{lcs/J21h41m47.3s+06d11m16.0s_lc_fit.pdf}{0.24\linewidth}{J21h41m47.3s+06d11m16.0s}
	\fig{lcs/J21h41m48.2s+04d38m19.7s_lc_fit.pdf}{0.24\linewidth}{J21h41m48.2s+04d38m19.7s}
	\fig{lcs/J22h02m42.1s+04d36m37.8s_lc_fit.pdf}{0.24\linewidth}{J22h02m42.1s+04d36m37.8s}}
\end{figure*}


==> ese_prop_data_old.tex <==
% J02342.9$-$593032 & 5.9288 & $-$59.5089 & $-$0.02$\pm$0.28 & 57.8$\pm$6.0 & 7.7$\pm$3.7 & 0.377$\pm$0.031 & 42.26$\pm$0.66 & 60818.0$\pm$3.8 \\
% J11512.5$-$294145 & 18.8021 & $-$29.6959 & 0.016$\pm$0.047 & 2.48$\pm$0.46 & 19.429$\pm$0.049 & 0.614$\pm$0.016 & 12.15$\pm$0.14 & 60167.59$\pm$0.38 \\
% J15009.8$-$452255 & 27.5408 & $-$45.382 & 0.21$\pm$0.51 & 26.5$\pm$2.3 & 12.43$\pm$0.74 & 0.290$\pm$0.025 & 6.01$\pm$0.24 & 60455.7$\pm$5.4 \\
% J21149.1+60015 & 32.9546 & 6.004 & $-$0.32$\pm$0.26 & 64$\pm$17 & 17.0$\pm$5.1 & 0.33$\pm$0.14 & 5.920$\pm$0.067 & 60150$\pm$10 \\
% J30438.5+01242 & 46.1604 & 0.2116 & $-$0.144$\pm$0.025 & 8.7$\pm$4.3 & 17.1$\pm$1.4 & 0.637$\pm$0.093 & 4.562$\pm$0.045 & 60445.0$\pm$5.3 \\
% J31105.9$-$81231 & 47.7746 & $-$8.2087 & $-$0.4475$\pm$0.0032 & 38.6$\pm$1.1 & 16.121$\pm$0.091 & 0.4684$\pm$0.0092 & 24.190$\pm$0.058 & 60304.6$\pm$1.1 \\
% J31556.2$-$62502 & 48.9842 & $-$6.4171 & 0.41$\pm$0.14 & 26.96$\pm$0.34 & 11.36$\pm$0.12 & 0.472$\pm$0.016 & 5.232$\pm$0.033 & 60771.3$\pm$4.2 \\
% J35855.3+63440 & 59.7304 & 6.5778 & 0.47$\pm$0.17 & 7.8$\pm$3.0 & 7.50$\pm$0.18 & 0.408$\pm$0.024 & 2.891$\pm$0.050 & 61014.9$\pm$8.5 \\
% J40242.0+82524 & 60.675 & 8.4234 & $-$0.526$\pm$0.066 & 32.1$\pm$6.7 & 4.57$\pm$0.22 & 0.578$\pm$0.041 & 6.68$\pm$0.10 & 60673.6$\pm$9.8 \\
% J40358.8+64539 & 60.995 & 6.7608 & $-$0.233$\pm$0.093 & 67$\pm$12 & 6.8$\pm$1.0 & 0.33$\pm$0.12 & 4.30$\pm$0.16 & 59969$\pm$17 \\
% J40800.2$-$325002 & 62.0008 & $-$32.834 & $-$0.251$\pm$0.012 & 4.21$\pm$0.78 & 11.406$\pm$0.075 & 0.675$\pm$0.011 & 6.05$\pm$0.13 & 60648.6$\pm$1.4 \\
% J40929.7+01136 & 62.3738 & 0.1935 & $-$0.63$\pm$0.62 & 31$\pm$23 & 3$\pm$15 & 0.39$\pm$0.17 & 4.10$\pm$0.39 & 59648$\pm$36 \\
% J42632.5+22300 & 66.6354 & 2.3831 & $-$0.546$\pm$0.012 & 8.17$\pm$0.72 & 5.20$\pm$0.10 & 0.532$\pm$0.021 & 5.972$\pm$0.074 & 60112.8$\pm$2.6 \\
% J42722.4$-$490742 & 66.8433 & $-$49.1283 & $-$0.342$\pm$0.043 & 20.3$\pm$4.6 & 20.1$\pm$1.4 & 0.419$\pm$0.045 & 3.491$\pm$0.037 & 60781.3$\pm$4.0 \\
% J43006.7$-$390622 & 67.5279 & $-$39.1062 & $-$0.91$\pm$0.11 & 26.1$\pm$1.3 & 3.78$\pm$0.51 & 0.589$\pm$0.073 & 4.062$\pm$0.030 & 60800.1$\pm$8.7 \\
% J43124.7+62208 & 67.8529 & 6.369 & $-$0.37$\pm$0.23 & 79.5$\pm$7.2 & 9.9$\pm$1.4 & 0.10$\pm$0.10 & 8.160$\pm$0.077 & 60744.0$\pm$4.6 \\
% J43136.0$-$80435 & 67.9 & $-$8.0763 & 0.951$\pm$0.039 & 26.00$\pm$0.34 & 11.5091$\pm$0.0093 & 0.49218$\pm$0.00065 & 231.06$\pm$0.77 & 60438.27$\pm$0.52 \\
% J43738.5$-$445427 & 69.4104 & $-$44.9074 & $-$0.955$\pm$0.013 & 17.0$\pm$1.1 & 10.34$\pm$0.16 & 0.554$\pm$0.029 & 10.707$\pm$0.062 & 60600.6$\pm$2.9 \\
% J44504.7$-$393713 & 71.2696 & $-$39.6202 & $-$0.69$\pm$0.20 & 4$\pm$13 & 18.6$\pm$7.1 & 0.59$\pm$0.13 & 17.1$\pm$5.0 & 60648$\pm$12 \\
% J44937.4+81134 & 72.4058 & 8.1928 & $-$0.295$\pm$0.055 & 45$\pm$12 & 9.02$\pm$0.61 & 0.511$\pm$0.073 & 4.155$\pm$0.060 & 60816$\pm$11 \\
% J45127.2+81254 & 72.8633 & 8.2149 & $-$0.042$\pm$0.069 & 28.1$\pm$3.3 & 13.57$\pm$0.59 & 0.422$\pm$0.046 & 2.926$\pm$0.072 & 60710.8$\pm$5.8 \\
% J50004.8+01421 & 75.02 & 0.2391 & $-$0.616$\pm$0.023 & 20.02$\pm$0.28 & 10.70$\pm$0.25 & 0.657$\pm$0.018 & 7.589$\pm$0.045 & 60623.0$\pm$2.5 \\
% J050237.9$-$43509 & 75.6579 & $-$4.5859 & $-$0.21$\pm$0.47 & 9$\pm$25 & 2$\pm$16 & 0.64$\pm$0.21 & 15.58$\pm$0.23 & 5.8930$\pm$110 \\
% J050332.1$-$45756 & 75.8837 & $-$4.9656 & $-$0.52$\pm$0.17 & 21$\pm$16 & 5.3$\pm$9.3 & 0.68$\pm$0.16 & 8.621$\pm$0.075 & 61055$\pm$63 \\
% J050703.7$-$84009 & 76.7654 & $-$8.6691 & $-$0.51$\pm$0.23 & 27.9$\pm$4.5 & 5.7$\pm$8.2 & 0.636$\pm$0.047 & 24.4$\pm$5.8 & 60355$\pm$28 \\
% J050831.9+60012 & 77.1329 & 6.0033 & $-$0.145$\pm$0.037 & 29.00$\pm$0.75 & 15.43$\pm$0.98 & 0.530$\pm$0.031 & 5.062$\pm$0.054 & 60496.5$\pm$4.7 \\
% J050848.5$-$450921 & 77.2021 & $-$45.1557 & $-$0.020$\pm$0.024 & 19.1$\pm$2.3 & 9.99$\pm$0.24 & 0.580$\pm$0.035 & 4.331$\pm$0.071 & 60269$\pm$18 \\
% J050912.5$-$452219 & 77.3021 & $-$45.372 & $-$0.42$\pm$0.13 & 71$\pm$13 & 12.7$\pm$3.0 & 0.498$\pm$0.056 & 6.847$\pm$0.046 & 60268.4$\pm$8.1 \\
% J050917.4$-$02426 & 77.3225 & $-$0.4072 & $-$0.134$\pm$0.022 & 29.05$\pm$0.27 & 17.34$\pm$0.64 & 0.638$\pm$0.026 & 5.250$\pm$0.085 & 60550.7$\pm$6.0 \\
% J051232.0$-$25829 & 78.1333 & $-$2.9748 & $-$0.222$\pm$0.031 & 20.5$\pm$3.2 & 9.68$\pm$0.26 & 0.477$\pm$0.033 & 4.233$\pm$0.067 & 60484.9$\pm$6.5 \\
% J051341.0$-$92215 & 78.4208 & $-$9.3707 & $-$0.271$\pm$0.020 & 24.26$\pm$0.55 & 7.55$\pm$0.19 & 0.584$\pm$0.028 & 6.165$\pm$0.049 & 59967.6$\pm$6.8 \\
% J051450.7+24829 & 78.7112 & 2.8081 & $-$0.354$\pm$0.043 & 32.5$\pm$6.5 & 7.4$\pm$1.1 & 0.619$\pm$0.031 & 5.836$\pm$0.079 & 60206$\pm$33 \\
% J051452.0$-$05416 & 78.7167 & $-$0.9043 & $-$0.947$\pm$0.020 & 9.7$\pm$2.4 & 3.56$\pm$0.20 & 0.666$\pm$0.052 & 4.56$\pm$0.10 & 60746$\pm$23 \\
% J051645.1+74123 & 79.1879 & 7.6898 & $-$0.3610$\pm$0.0091 & 96.0$\pm$2.5 & 7.517$\pm$0.097 & 0.058$\pm$0.029 & 33.501$\pm$0.073 & 60780.0$\pm$2.7 \\
% J051941.1+03430 & 79.9212 & 0.5751 & $-$0.5148$\pm$0.0056 & 27.93$\pm$0.49 & 7.040$\pm$0.061 & 0.5813$\pm$0.0099 & 9.461$\pm$0.069 & 60419.0$\pm$4.5 \\
% J052325.7+15837 & 80.8571 & 1.977 & $-$1.00$\pm$0.41 & 12$\pm$12 & 3.7$\pm$8.9 & 0.543$\pm$0.093 & 9.61$\pm$0.20 & 60813$\pm$13 \\
% J052803.1$-$330348 & 82.0129 & $-$33.0634 & $-$0.027$\pm$0.019 & 30.4$\pm$1.0 & 23.45$\pm$0.12 & 0.156$\pm$0.017 & 20.01$\pm$0.11 & 60163.2$\pm$4.2 \\
% J055109.4$-$40655 & 87.7892 & $-$4.1153 & $-$0.96$\pm$0.32 & 16$\pm$14 & 3$\pm$12 & 0.67$\pm$0.15 & 3.377$\pm$0.080 & 61060$\pm$110 \\
% J055202.1$-$300936 & 88.0087 & $-$30.16 & $-$0.570$\pm$0.010 & 9.9$\pm$2.1 & 5.289$\pm$0.077 & 0.823$\pm$0.011 & 6.261$\pm$0.038 & 60735.4$\pm$3.9 \\
% J060158.9$-$52751 & 90.4954 & $-$5.4641 & $-$0.314$\pm$0.021 & 24.28$\pm$0.66 & 10.72$\pm$0.39 & 0.632$\pm$0.019 & 5.678$\pm$0.041 & 60311.0$\pm$6.5 \\
% J061139.7$-$11802 & 92.9154 & $-$1.3005 & $-$0.83$\pm$0.11 & 22.4$\pm$5.7 & 2.40$\pm$0.16 & 0.465$\pm$0.035 & 6.42$\pm$0.47 & 6.0190$\pm$120 \\
% J063644.1$-$53002 & 99.1837 & $-$5.5005 & 0.0049$\pm$0.0069 & 22.8$\pm$3.3 & 16.0$\pm$1.1 & 0.272$\pm$0.052 & 3.127$\pm$0.086 & 60791.4$\pm$9.2 \\
% J071328.3+65142 & 108.3679 & 6.8616 & 0.223$\pm$0.023 & 2.44$\pm$0.49 & 24.81$\pm$0.25 & 0.457$\pm$0.031 & 5.228$\pm$0.042 & 60753.5$\pm$8.6 \\
% J072856.5$-$61140 & 112.2354 & $-$6.1945 & $-$0.186$\pm$0.028 & 28.0$\pm$4.8 & 17.4$\pm$1.0 & 0.608$\pm$0.021 & 10.647$\pm$0.087 & 60614.4$\pm$8.0 \\
% J074004.9+41529 & 115.0204 & 4.2579 & $-$0.34$\pm$0.11 & 27.6$\pm$9.7 & 12.2$\pm$2.8 & 0.571$\pm$0.077 & 4.282$\pm$0.049 & 60168$\pm$13 \\
% J074613.8$-$72822 & 116.5575 & $-$7.4729 & $-$0.271$\pm$0.023 & 18.9$\pm$8.8 & 14.3$\pm$1.1 & 0.749$\pm$0.028 & 8.335$\pm$0.073 & 60225.7$\pm$3.6 \\
% J075828.0+82708 & 119.6167 & 8.4523 & $-$0.4379$\pm$0.0093 & 49.94$\pm$0.49 & 4.611$\pm$0.015 & 0.5526$\pm$0.0039 & 80.998$\pm$0.059 & 59996.2$\pm$2.8 \\
% J085439.5+84326 & 133.6646 & 8.7238 & $-$0.344$\pm$0.060 & 17.5$\pm$2.1 & 11.8$\pm$1.1 & 0.299$\pm$0.064 & 3.084$\pm$0.081 & 60486.3$\pm$2.7 \\
% J085634.8$-$65409 & 134.145 & $-$6.9026 & 0.027$\pm$0.060 & 11.0$\pm$3.5 & 14.80$\pm$0.54 & 0.585$\pm$0.011 & 10.64$\pm$0.11 & 60255.2$\pm$9.0 \\
% J090108.6$-$03334 & 135.2858 & $-$0.5594 & $-$0.95$\pm$0.39 & 33$\pm$16 & 10.4$\pm$7.6 & 0.03$\pm$0.19 & 10.017$\pm$0.096 & 60636$\pm$17 \\
% J090943.2+30922 & 137.43 & 3.1562 & $-$0.43$\pm$0.67 & 15.4$\pm$3.7 & 6.9$\pm$1.8 & 0.498$\pm$0.099 & 6.93$\pm$0.22 & 60632.7$\pm$7.3 \\
% J091708.1$-$30618 & 139.2837 & $-$3.105 & $-$0.61$\pm$0.26 & 20.3$\pm$4.5 & 23.0$\pm$4.3 & 0.093$\pm$0.051 & 9.469$\pm$0.047 & 60715$\pm$11 \\
% J094215.5+43622 & 145.5646 & 4.6061 & $-$0.2033$\pm$0.0064 & 91.4$\pm$2.8 & 8.32$\pm$0.26 & 0.625$\pm$0.029 & 70.893$\pm$0.099 & 60815.6$\pm$2.2 \\
% J101219.1$-$302237 & 153.0796 & $-$30.377 & $-$0.437$\pm$0.091 & 4.1$\pm$1.5 & 5.50$\pm$0.71 & 0.6860$\pm$0.0070 & 3.31$\pm$0.10 & 60810$\pm$29 \\
% J102059.6$-$361427 & 155.2483 & $-$36.2408 & $-$0.5324$\pm$0.0099 & 26.19$\pm$0.17 & 13.701$\pm$0.064 & 0.401$\pm$0.021 & 13.186$\pm$0.063 & 60635.49$\pm$0.80 \\
% J102443.5$-$373347 & 156.1812 & $-$37.5631 & $-$0.101$\pm$0.014 & 16.7$\pm$1.3 & 5.609$\pm$0.061 & 0.538$\pm$0.037 & 3.569$\pm$0.040 & 60031.4$\pm$6.3 \\
% J102645.9$-$285641 & 156.6912 & $-$28.9448 & $-$0.74$\pm$0.26 & 24.4$\pm$6.8 & 8.7$\pm$7.5 & 0.499$\pm$0.033 & 18.6$\pm$3.0 & 60498$\pm$27 \\
% J103306.1$-$305440 & 158.2754 & $-$30.9111 & $-$0.07$\pm$0.47 & 2$\pm$20 & 8.3$\pm$6.9 & 0.72$\pm$0.17 & 4.01$\pm$0.48 & 60724$\pm$78 \\
% J104424.0$-$304058 & 161.1 & $-$30.6828 & $-$1.04$\pm$0.25 & 41.6$\pm$7.9 & 6.7$\pm$8.4 & 0.440$\pm$0.063 & 49.80$\pm$0.53 & 60575$\pm$12 \\
% J105529.0$-$301103 & 163.8708 & $-$30.1842 & $-$0.30$\pm$0.11 & 27.07$\pm$0.44 & 14.4$\pm$1.9 & 0.655$\pm$0.045 & 3.159$\pm$0.042 & 60486$\pm$22 \\
% J105613.1$-$352736 & 164.0546 & $-$35.4599 & 0.055$\pm$0.038 & 20.4$\pm$4.8 & 13.16$\pm$0.47 & 0.540$\pm$0.025 & 5.211$\pm$0.093 & 60302.1$\pm$3.8 \\
% J105834.4$-$421513 & 164.6433 & $-$42.2537 & $-$0.317$\pm$0.021 & 18.1$\pm$4.5 & 13.71$\pm$0.38 & 0.646$\pm$0.018 & 5.468$\pm$0.085 & 60519.8$\pm$2.8 \\
% J110220.7+14206 & 165.5862 & 1.7015 & $-$0.251$\pm$0.033 & 28.8$\pm$1.5 & 19.5$\pm$1.7 & 0.451$\pm$0.028 & 8.217$\pm$0.062 & 60224.9$\pm$2.7 \\
% J113248.9$-$504859 & 173.2037 & $-$50.8163 & 0.113$\pm$0.022 & 27.12$\pm$0.57 & 23.19$\pm$0.60 & 0.572$\pm$0.018 & 17.72$\pm$0.19 & 60638.8$\pm$2.7 \\
% J113259.3$-$484235 & 173.2471 & $-$48.7098 & $-$0.361$\pm$0.011 & 85.0$\pm$7.7 & 19.7$\pm$1.3 & 0.106$\pm$0.088 & 7.222$\pm$0.047 & 60470.2$\pm$3.1 \\
% J113347.6$-$353900 & 173.4483 & $-$35.6498 & $-$0.14$\pm$0.38 & 4$\pm$20 & 1$\pm$14 & 0.83$\pm$0.10 & 30.13$\pm$0.17 & 58330$\pm$140 \\
% J113700.5$-$450513 & 174.2521 & $-$45.0868 & 0.089$\pm$0.045 & 27.87$\pm$0.29 & 7.29$\pm$0.12 & 0.405$\pm$0.019 & 12.93$\pm$0.17 & 60539.3$\pm$8.4 \\
% J114339.8+70013 & 175.9158 & 7.0035 & $-$0.94$\pm$0.54 & 29$\pm$20 & 6.0$\pm$2.6 & 0.49$\pm$0.12 & 17.0$\pm$2.0 & 60404.5$\pm$8.6 \\
% J114528.5$-$373931 & 176.3687 & $-$37.6588 & $-$0.960$\pm$0.017 & 26.96$\pm$0.91 & 15.62$\pm$0.73 & 0.687$\pm$0.034 & 3.426$\pm$0.043 & 60337.3$\pm$9.0 \\
% J114646.0$-$460531 & 176.6917 & $-$46.0919 & $-$0.82$\pm$0.16 & 6$\pm$25 & 4$\pm$13 & 0.88$\pm$0.25 & 8.18$\pm$0.12 & 60765$\pm$73 \\
% J114936.2$-$342505 & 177.4008 & $-$34.4179 & $-$0.43$\pm$0.39 & 30$\pm$19 & 31.7$\pm$6.9 & 0.647$\pm$0.059 & 3.849$\pm$0.060 & 60905.1$\pm$9.5 \\
% J114940.0$-$375434 & 177.4167 & $-$37.9095 & $-$0.16$\pm$0.37 & 27.2$\pm$7.3 & 28$\pm$12 & 0.29$\pm$0.13 & 10.6$\pm$2.6 & 60470.0$\pm$6.5 \\
% J115029.4$-$335716 & 177.6225 & $-$33.9545 & $-$0.87$\pm$0.11 & 27.55$\pm$0.84 & 8.5$\pm$1.9 & 0.448$\pm$0.059 & 7.890$\pm$0.090 & 60703.5$\pm$8.9 \\
% J115458.5$-$514404 & 178.7437 & $-$51.7343 & $-$0.156$\pm$0.063 & 21.3$\pm$3.9 & 9.3$\pm$1.5 & 0.435$\pm$0.018 & 5.97$\pm$0.14 & 60154$\pm$43 \\
% J120837.3$-$410514 & 182.1554 & $-$41.0873 & $-$0.801$\pm$0.073 & 19.2$\pm$2.1 & 8.90$\pm$0.93 & 0.267$\pm$0.052 & 6.042$\pm$0.055 & 60242.9$\pm$4.6 \\
% J121311.9+35045 & 183.2996 & 3.8458 & $-$0.37$\pm$0.23 & 7$\pm$23 & 29.1$\pm$7.7 & 0.65$\pm$0.10 & 12.4$\pm$2.0 & 60438$\pm$25 \\
% J121335.5$-$503143 & 183.3979 & $-$50.5285 & $-$0.287$\pm$0.014 & 24.01$\pm$0.53 & 12.82$\pm$0.40 & 0.591$\pm$0.031 & 3.168$\pm$0.038 & 60263.6$\pm$6.5 \\
% J121701.5$-$510102 & 184.2562 & $-$51.0171 & 0.02$\pm$0.30 & 29.4$\pm$2.6 & 12.66$\pm$0.15 & 0.6211$\pm$0.0086 & 14.67$\pm$0.15 & 60347.7$\pm$2.1 \\
% J121758.4$-$363418 & 184.4933 & $-$36.5716 & $-$0.0980$\pm$0.0056 & 18.83$\pm$0.30 & 11.315$\pm$0.060 & 0.60124$\pm$0.00091 & 330.86$\pm$0.31 & 60292.48$\pm$0.72 \\
% % J121835.0$-$11953 & 184.6458 & $-$1.3314 & $-$1.06$\pm$0.18 & 12.14$\pm$0.33 & 39.61$\pm$0.32 & \mathrm{nan}$\pm$\mathrm{nan} & 209.469$\pm$0.064 & 59416.4$\pm$6.8 \\
% J125002.7$-$504149 & 192.5112 & $-$50.6969 & 0.1202$\pm$0.0074 & 23.04$\pm$0.32 & 18.75$\pm$0.17 & 0.395$\pm$0.022 & 3.713$\pm$0.040 & 60538.3$\pm$7.7 \\
% J125022.8$-$443203 & 192.595 & $-$44.5342 & $-$0.3716$\pm$0.0040 & 98.50$\pm$0.37 & 14.828$\pm$0.051 & 0.1200$\pm$0.0059 & 45.944$\pm$0.040 & 60427.77$\pm$0.88 \\
% J125051.8$-$494733 & 192.7158 & $-$49.7925 & $-$0.334$\pm$0.016 & 17.27$\pm$0.54 & 9.077$\pm$0.088 & 0.7443$\pm$0.0063 & 10.531$\pm$0.044 & 60411.4$\pm$4.0 \\
% J125710.4$-$463741 & 194.2933 & $-$46.628 & $-$0.734$\pm$0.011 & 26.31$\pm$0.11 & 8.786$\pm$0.063 & 0.7162$\pm$0.0053 & 16.850$\pm$0.024 & 60453.1$\pm$1.9 \\
% J130013.3$-$501153 & 195.0554 & $-$50.1981 & $-$0.057$\pm$0.081 & 33.9$\pm$1.7 & 5.43$\pm$0.18 & 0.6465$\pm$0.0088 & 16.50$\pm$0.11 & 60100.0$\pm$4.5 \\
% J130023.0$-$420839 & 195.0958 & $-$42.1442 & $-$0.52$\pm$0.26 & 31.9$\pm$7.0 & 7.4$\pm$1.7 & 0.580$\pm$0.073 & 4.200$\pm$0.093 & 60213$\pm$25 \\
% J130245.2$-$430856 & 195.6883 & $-$43.1489 & $-$0.43$\pm$0.39 & 43$\pm$24 & 13.3$\pm$6.6 & 0.56$\pm$0.14 & 10.98$\pm$0.12 & 60172.4$\pm$7.1 \\
% J130826.8$-$354557 & 197.1117 & $-$35.7659 & $-$1.21$\pm$0.65 & 4$\pm$26 & 7.7$\pm$2.6 & 0.620$\pm$0.096 & 10.8$\pm$3.1 & 60396$\pm$29 \\
% J131126.9$-$310036 & 197.8621 & $-$31.0101 & $-$0.452$\pm$0.089 & 39.3$\pm$7.9 & 12.4$\pm$1.3 & 0.607$\pm$0.047 & 7.664$\pm$0.036 & 60218.2$\pm$5.4 \\
% J131537.8$-$473458 & 198.9075 & $-$47.5826 & $-$0.5059$\pm$0.0087 & 28.06$\pm$0.30 & 10.19$\pm$0.28 & 0.662$\pm$0.015 & 8.874$\pm$0.062 & 60220.0$\pm$7.2 \\
% J132343.8$-$514223 & 200.9325 & $-$51.7063 & 0.54$\pm$0.22 & 41.7$\pm$5.4 & 15.02$\pm$0.40 & 0.542$\pm$0.032 & 4.233$\pm$0.043 & 60674.4$\pm$6.4 \\
% J132442.8$-$502038 & 201.1783 & $-$50.3438 & $-$0.364$\pm$0.037 & 28.0$\pm$3.8 & 5.47$\pm$0.25 & 0.733$\pm$0.021 & 7.672$\pm$0.067 & 60808$\pm$12 \\
% J132450.9$-$63941 & 201.2121 & $-$6.6613 & $-$0.273$\pm$0.038 & 57.6$\pm$2.4 & 24.6$\pm$1.3 & 0.031$\pm$0.025 & 18.030$\pm$0.056 & 60424.56$\pm$0.86 \\
% J133100.3$-$380928 & 202.7512 & $-$38.1578 & $-$0.5854$\pm$0.0056 & 36.77$\pm$0.76 & 14.652$\pm$0.037 & 0.5654$\pm$0.0072 & 40.076$\pm$0.049 & 60616.7$\pm$1.3 \\
% % J133107.7$-$530957 & 202.7821 & $-$53.1659 & $-$0.45$\pm$0.42 & \mathrm{nan}$\pm$\mathrm{nan} & 12.1$\pm$2.4 & 0.636$\pm$0.057 & 2.403$\pm$0.069 & 60610$\pm$22 \\
% J133222.0$-$521639 & 203.0917 & $-$52.2775 & $-$0.578$\pm$0.028 & 5.05$\pm$0.73 & 4.33$\pm$0.20 & 0.778$\pm$0.016 & 4.966$\pm$0.074 & 60981$\pm$24 \\
% J133232.8$-$472830 & 203.1367 & $-$47.475 & $-$0.732$\pm$0.016 & 26.23$\pm$0.53 & 8.79$\pm$0.48 & 0.635$\pm$0.032 & 3.994$\pm$0.052 & 60490.6$\pm$6.2 \\
% J133603.2$-$513600 & 204.0133 & $-$51.6 & $-$0.45$\pm$0.37 & 23$\pm$20 & 5$\pm$16 & 0.77$\pm$0.17 & 11.743$\pm$0.084 & 60968$\pm$97 \\
% J133756.4$-$505541 & 204.485 & $-$50.928 & $-$0.578$\pm$0.075 & 25.4$\pm$2.0 & 5.60$\pm$0.47 & 0.680$\pm$0.029 & 3.070$\pm$0.050 & 60799.5$\pm$5.7 \\
% J134117.8$-$490337 & 205.3242 & $-$49.0602 & $-$0.497$\pm$0.034 & 28.4$\pm$3.8 & 10.45$\pm$0.66 & 0.505$\pm$0.048 & 3.362$\pm$0.045 & 60516.2$\pm$5.8 \\
% J134236.4$-$503913 & 205.6517 & $-$50.6536 & $-$0.949$\pm$0.037 & 14.4$\pm$3.3 & 8.468$\pm$0.052 & 0.682$\pm$0.071 & 3.047$\pm$0.054 & 60443$\pm$10 \\
% J134831.0$-$303536 & 207.1292 & $-$30.5934 & $-$0.164$\pm$0.030 & 4.2$\pm$1.6 & 16.10$\pm$0.73 & 0.655$\pm$0.038 & 3.147$\pm$0.063 & 60559.7$\pm$5.4 \\
% J134922.2+71218 & 207.3425 & 7.2049 & $-$0.379$\pm$0.035 & 28.1$\pm$5.9 & 4.70$\pm$0.60 & 0.504$\pm$0.036 & 3.484$\pm$0.070 & 60002$\pm$17 \\
% J134946.1+90816 & 207.4421 & 9.1379 & $-$0.55$\pm$0.14 & 22.7$\pm$4.3 & 25.3$\pm$5.1 & 0.378$\pm$0.039 & 26.1$\pm$5.9 & 60612$\pm$20 \\
% J135739.4$-$452029 & 209.4142 & $-$45.3414 & $-$0.541$\pm$0.034 & 10.4$\pm$4.2 & 6.1$\pm$1.0 & 0.647$\pm$0.038 & 3.468$\pm$0.058 & 60900$\pm$12 \\
% J140602.1$-$434823 & 211.5087 & $-$43.8065 & $-$0.9539$\pm$0.0090 & 29.00$\pm$0.33 & 13.15$\pm$0.23 & 0.062$\pm$0.020 & 5.957$\pm$0.073 & 60814.2$\pm$2.5 \\
% J141524.4$-$424912 & 213.8517 & $-$42.8201 & $-$0.45$\pm$0.58 & 8$\pm$45 & 35$\pm$15 & 0.005$\pm$0.019 & 21.4$\pm$1.5 & 60299$\pm$63 \\
% J141904.9$-$90045 & 214.7704 & $-$9.0126 & $-$0.725$\pm$0.095 & 10.2$\pm$3.7 & 5.12$\pm$0.90 & 0.56$\pm$0.14 & 2.746$\pm$0.075 & 60553.4$\pm$7.0 \\
% J141945.9$-$82706 & 214.9412 & $-$8.4518 & $-$0.3562$\pm$0.0090 & 64.1$\pm$7.6 & 7.78$\pm$0.75 & 0.157$\pm$0.078 & 2.778$\pm$0.048 & 60661.4$\pm$9.6 \\
% J142225.1+70158 & 215.6046 & 7.0328 & 0.211$\pm$0.023 & 71.0$\pm$4.6 & 15.01$\pm$0.69 & 0.163$\pm$0.064 & 5.880$\pm$0.082 & 61097$\pm$25 \\
% J143452.7$-$02828 & 218.7196 & $-$0.4746 & 0.65$\pm$0.25 & 30.5$\pm$3.6 & 23.4$\pm$3.9 & 0.351$\pm$0.013 & 34.1$\pm$5.7 & 60658.6$\pm$6.8 \\
% J150637.4+02540 & 226.6558 & 0.4279 & 0.38$\pm$0.26 & 7.3$\pm$2.8 & 12.92$\pm$0.25 & 0.701$\pm$0.022 & 5.306$\pm$0.061 & 60710.8$\pm$4.1 \\
% J151331.7$-$91920 & 228.3821 & $-$9.3221 & $-$0.423$\pm$0.028 & 4.23$\pm$0.53 & 10.80$\pm$0.55 & 0.459$\pm$0.047 & 9.44$\pm$0.14 & 60141$\pm$15 \\
% J151446.8+15128 & 228.695 & 1.8577 & $-$0.635$\pm$0.094 & 14.0$\pm$2.8 & 7.67$\pm$0.82 & 0.582$\pm$0.031 & 6.448$\pm$0.080 & 60924$\pm$13 \\
% J151738.6+34528 & 229.4108 & 3.7579 & $-$0.233$\pm$0.026 & 41.1$\pm$4.4 & 9.69$\pm$0.46 & 0.533$\pm$0.020 & 14.93$\pm$0.14 & 60830.4$\pm$4.0 \\
% J151951.3$-$91849 & 229.9637 & $-$9.3136 & $-$0.0159$\pm$0.0068 & 46.4$\pm$7.0 & 22.01$\pm$0.82 & 0.463$\pm$0.045 & 8.192$\pm$0.076 & 60641.3$\pm$4.7 \\
% J152445.4$-$13740 & 231.1892 & $-$1.6279 & $-$0.950$\pm$0.018 & 27.9$\pm$2.2 & 9.67$\pm$0.56 & 0.354$\pm$0.055 & 5.611$\pm$0.063 & 60477.9$\pm$7.2 \\
% J152659.3+63348 & 231.7471 & 6.5635 & $-$0.15$\pm$0.73 & 33$\pm$14 & 39$\pm$16 & 0.17$\pm$0.11 & 5.538$\pm$0.061 & 59639$\pm$17 \\
% J152914.4$-$41408 & 232.31 & $-$4.2354 & $-$0.024$\pm$0.012 & 82.6$\pm$8.0 & 43.4$\pm$2.0 & 0.220$\pm$0.084 & 6.841$\pm$0.041 & 60678.2$\pm$2.5 \\
% J154236.1$-$54755 & 235.6504 & $-$5.7987 & $-$0.7593$\pm$0.0071 & 27.0$\pm$8.5 & 12.5$\pm$1.1 & 0.488$\pm$0.052 & 3.916$\pm$0.058 & 60628.7$\pm$7.1 \\
% J154244.0+11458 & 235.6833 & 1.2493 & $-$0.300$\pm$0.037 & 18.22$\pm$0.26 & 9.27$\pm$0.57 & 0.644$\pm$0.016 & 8.459$\pm$0.097 & 60827$\pm$11 \\
% J154339.8+80613 & 235.9158 & 8.1036 & $-$1.15$\pm$0.52 & 7$\pm$21 & 2$\pm$12 & 0.64$\pm$0.13 & 4.88$\pm$0.57 & 59563$\pm$68 \\
% J154908.8$-$11628 & 237.2867 & $-$1.2744 & $-$0.439$\pm$0.047 & 19.3$\pm$3.3 & 4.24$\pm$0.37 & 0.672$\pm$0.018 & 6.40$\pm$0.14 & 60796$\pm$21 \\
% J154940.2+10602 & 237.4175 & 1.1004 & $-$0.364$\pm$0.028 & 56$\pm$17 & 19.5$\pm$2.4 & 0.557$\pm$0.027 & 5.567$\pm$0.073 & 60550.4$\pm$4.5 \\
% J160220.5$-$42537 & 240.5854 & $-$4.4268 & $-$0.48$\pm$0.11 & 40.0$\pm$9.1 & 5.27$\pm$0.54 & 0.474$\pm$0.090 & 4.585$\pm$0.081 & 60098$\pm$14 \\
% J160314.9+81020 & 240.8121 & 8.1723 & $-$0.397$\pm$0.021 & 25.1$\pm$1.8 & 10.17$\pm$0.35 & 0.436$\pm$0.022 & 6.589$\pm$0.062 & 60854.7$\pm$5.9 \\
% J160556.9$-$10949 & 241.4871 & $-$1.1637 & $-$0.023$\pm$0.023 & 38.0$\pm$3.1 & 3.10$\pm$0.21 & 0.260$\pm$0.025 & 9.13$\pm$0.26 & 61185$\pm$35 \\
% J160606.9+61949 & 241.5287 & 6.3302 & $-$0.36$\pm$0.10 & 38.3$\pm$6.0 & 16.2$\pm$4.8 & 0.00$\pm$0.10 & 49$\pm$15 & 60048$\pm$13 \\
% J160856.1+91038 & 242.2337 & 9.1774 & $-$0.41$\pm$0.20 & 8$\pm$24 & 6$\pm$11 & 0.59$\pm$0.16 & 18.83$\pm$0.26 & 60913.0$\pm$7.3 \\
% J161011.9$-$34917 & 242.5496 & $-$3.8214 & $-$0.433$\pm$0.012 & 23.8$\pm$2.0 & 4.871$\pm$0.016 & 0.443$\pm$0.042 & 12.02$\pm$0.14 & 59665$\pm$19 \\
% J161012.4$-$01142 & 242.5517 & $-$0.1949 & $-$1.003$\pm$0.077 & 5.97$\pm$0.89 & 2.02$\pm$0.26 & 0.770$\pm$0.072 & 4.18$\pm$0.17 & 58840$\pm$120 \\
% J161131.8$-$34058 & 242.8825 & $-$3.6829 & $-$0.112$\pm$0.046 & 27.27$\pm$0.36 & 12.1$\pm$1.5 & 0.559$\pm$0.067 & 11.57$\pm$0.14 & 60539$\pm$13 \\
% J161726.3+63232 & 244.3596 & 6.5424 & $-$0.272$\pm$0.020 & 12.1$\pm$6.2 & 11.69$\pm$0.43 & 0.161$\pm$0.026 & 2.086$\pm$0.063 & 60297.7$\pm$3.6 \\
% J161752.7$-$60511 & 244.4696 & $-$6.0865 & $-$0.659$\pm$0.066 & 29.3$\pm$4.8 & 3.49$\pm$0.56 & 0.618$\pm$0.020 & 17.13$\pm$0.37 & 59909$\pm$27 \\
% J161823.7$-$60326 & 244.5987 & $-$6.0573 & $-$0.437$\pm$0.015 & 10.00$\pm$0.99 & 6.49$\pm$0.35 & 0.596$\pm$0.015 & 5.125$\pm$0.073 & 60857.2$\pm$7.8 \\
% J161846.7+44007 & 244.6946 & 4.6685 & $-$0.52$\pm$0.20 & 34$\pm$15 & 13.3$\pm$6.7 & 0.539$\pm$0.047 & 25.7$\pm$3.2 & 60273.9$\pm$7.3 \\
% J162223.7+01329 & 245.5987 & 0.2246 & $-$0.360$\pm$0.030 & 61.6$\pm$3.6 & 8.57$\pm$0.32 & 0.044$\pm$0.044 & 4.902$\pm$0.047 & 60805.2$\pm$5.3 \\
% J162346.0$-$83538 & 245.9417 & $-$8.594 & 0.34$\pm$0.62 & 21.8$\pm$8.7 & 5$\pm$18 & 0.24$\pm$0.10 & 19.0$\pm$6.5 & 60639$\pm$35 \\
% J162520.4+55641 & 246.335 & 5.9447 & $-$0.597$\pm$0.037 & 37.7$\pm$1.2 & 5.949$\pm$0.021 & 0.6123$\pm$0.0096 & 38.056$\pm$0.041 & 60392.9$\pm$3.7 \\
% J162712.9+41835 & 246.8038 & 4.3096 & $-$0.57$\pm$0.17 & 42$\pm$19 & 6.8$\pm$6.6 & 0.514$\pm$0.095 & 5.00$\pm$0.14 & 60141$\pm$19 \\
% J162747.9$-$90106 & 246.9496 & $-$9.0184 & $-$0.480$\pm$0.080 & 59$\pm$12 & 9.6$\pm$1.4 & 0.492$\pm$0.093 & 4.41$\pm$0.17 & 60771$\pm$13 \\
% J163007.9$-$45136 & 247.5329 & $-$4.86 & $-$0.496$\pm$0.074 & 22.3$\pm$3.2 & 8.18$\pm$0.67 & 0.637$\pm$0.034 & 3.57$\pm$0.15 & 60453$\pm$10 \\
% J163051.5$-$81009 & 247.7146 & $-$8.1692 & $-$0.4675$\pm$0.0028 & 33.92$\pm$0.71 & 9.183$\pm$0.050 & 0.6456$\pm$0.0025 & 124.502$\pm$0.095 & 60509.2$\pm$1.4 \\
% J163155.3$-$83008 & 247.9804 & $-$8.5023 & $-$0.572$\pm$0.073 & 27.5$\pm$1.9 & 2.85$\pm$0.33 & 0.631$\pm$0.026 & 8.39$\pm$0.14 & 61132$\pm$29 \\
% J163641.6+92458 & 249.1733 & 9.4161 & 0.59$\pm$0.24 & 98.7$\pm$1.7 & 14.05$\pm$0.44 & 0.166$\pm$0.020 & 54.54$\pm$0.11 & 60160.9$\pm$2.3 \\
% J163750.2+21144 & 249.4592 & 2.1956 & $-$0.57$\pm$0.33 & 41.0$\pm$5.2 & 9.7$\pm$7.8 & 0.632$\pm$0.051 & 63.05$\pm$0.45 & 60435$\pm$11 \\
% J163939.0+90737 & 249.9125 & 9.1268 & 0.010$\pm$0.062 & 72$\pm$21 & 10.7$\pm$2.1 & 0.529$\pm$0.091 & 3.462$\pm$0.079 & 60766$\pm$35 \\
% J163951.1+11650 & 249.9629 & 1.2807 & $-$0.493$\pm$0.077 & 23$\pm$17 & 5.3$\pm$1.6 & 0.557$\pm$0.057 & 2.780$\pm$0.047 & 60561$\pm$14 \\
% J164043.3$-$13342 & 250.1804 & $-$1.5615 & $-$0.505$\pm$0.035 & 23.6$\pm$3.1 & 6.38$\pm$0.37 & 0.621$\pm$0.025 & 3.987$\pm$0.051 & 60083$\pm$13 \\
% J164100.2+55811 & 250.2508 & 5.9696 & $-$0.375$\pm$0.043 & 71$\pm$12 & 8.94$\pm$0.90 & 0.31$\pm$0.15 & 7.289$\pm$0.069 & 60014$\pm$11 \\
% % J164351.8+85506 & 250.9658 & 8.9183 & \mathrm{nan}$\pm$\mathrm{nan} & 27.72$\pm$0.53 & 10.61$\pm$0.15 & 0.6179$\pm$0.0025 & 44.60$\pm$0.12 & 60250.3$\pm$3.8 \\
% J164405.3+21409 & 251.0221 & 2.2358 & 0.1714$\pm$0.0061 & 32.0$\pm$1.7 & 16.62$\pm$0.23 & 0.5722$\pm$0.0086 & 23.382$\pm$0.095 & 60699.5$\pm$2.0 \\
% J164613.0+51750 & 251.5542 & 5.2972 & $-$0.7271$\pm$0.0069 & 26.36$\pm$0.23 & 6.10$\pm$0.38 & 0.736$\pm$0.013 & 15.05$\pm$0.13 & 60542.4$\pm$7.4 \\
% J164918.4+92144 & 252.3267 & 9.3621 & $-$0.021$\pm$0.036 & 18.8$\pm$1.8 & 7.7$\pm$1.5 & 0.663$\pm$0.022 & 6.61$\pm$0.13 & 60211$\pm$30 \\
% J164958.4$-$44847 & 252.4933 & $-$4.8131 & $-$0.75$\pm$0.70 & 74$\pm$11 & 4.4$\pm$1.1 & 0.13$\pm$0.25 & 14.53$\pm$0.18 & 60097.4$\pm$8.8 \\
% J165107.1+12406 & 252.7796 & 1.4017 & $-$0.472$\pm$0.084 & 33.8$\pm$5.7 & 4.77$\pm$0.55 & 0.519$\pm$0.054 & 12.12$\pm$0.24 & 60027$\pm$14 \\
% % J165206.0+52224 & 253.025 & 5.3734 & \mathrm{nan}$\pm$\mathrm{nan} & \mathrm{nan}$\pm$\mathrm{nan} & \mathrm{nan}$\pm$\mathrm{nan} & \mathrm{nan}$\pm$\mathrm{nan} & 7.67$\pm$0.78 & \mathrm{nan}$\pm$\mathrm{nan} \\
% J165237.3+10016 & 253.1554 & 1.0045 & $-$0.640$\pm$0.077 & 22.5$\pm$5.9 & 6.56$\pm$0.53 & 0.555$\pm$0.047 & 4.46$\pm$0.12 & 60360.0$\pm$9.2 \\
% J165600.0$-$03029 & 254.0 & $-$0.5081 & $-$0.699$\pm$0.067 & 12.6$\pm$3.1 & 7.45$\pm$0.37 & 0.752$\pm$0.045 & 5.448$\pm$0.056 & 60700.8$\pm$5.0 \\
% J165714.4+23056 & 254.31 & 2.5155 & $-$0.616$\pm$0.018 & 26.24$\pm$0.44 & 3.677$\pm$0.090 & 0.510$\pm$0.014 & 11.781$\pm$0.074 & 61182$\pm$20 \\
% J165844.7+81906 & 254.6862 & 8.3182 & $-$0.37$\pm$0.23 & 78.0$\pm$5.2 & 18.0$\pm$3.2 & 0.049$\pm$0.064 & 9.35$\pm$0.10 & 60811.8$\pm$3.6 \\
% J165910.9$-$73710 & 254.7954 & $-$7.6195 & $-$0.064$\pm$0.011 & 28.12$\pm$0.25 & 20.107$\pm$0.063 & 0.2540$\pm$0.0051 & 36.408$\pm$0.052 & 60666.95$\pm$0.98 \\
% J165922.1$-$03959 & 254.8421 & $-$0.6662 & $-$1.052$\pm$0.093 & 81$\pm$12 & 9.5$\pm$2.5 & 0.483$\pm$0.058 & 6.72$\pm$0.31 & 60661$\pm$11 \\
% J170023.9+52244 & 255.0996 & 5.3789 & $-$0.0593$\pm$0.0096 & 30.33$\pm$0.29 & 13.744$\pm$0.029 & 0.4614$\pm$0.0021 & 124.861$\pm$0.081 & 60312.44$\pm$0.23 \\
% J170124.9$-$63134 & 255.3537 & $-$6.526 & $-$0.62$\pm$0.43 & 16.0$\pm$3.4 & 4.0$\pm$5.3 & 0.543$\pm$0.035 & 36.5$\pm$2.1 & 59548$\pm$41 \\
% J170207.7$-$74646 & 255.5321 & $-$7.7794 & $-$0.058$\pm$0.058 & 24.4$\pm$2.6 & 4.79$\pm$0.13 & 0.599$\pm$0.017 & 5.71$\pm$0.10 & 60197$\pm$14 \\
% J170219.4$-$33858 & 255.5808 & $-$3.6495 & $-$0.37$\pm$0.28 & 72$\pm$29 & 5$\pm$11 & 0.22$\pm$0.19 & 4.79$\pm$0.11 & 60738$\pm$21 \\
% J170233.2$-$32804 & 255.6383 & $-$3.4676 & $-$0.39$\pm$0.62 & 9$\pm$28 & 2$\pm$15 & 0.48$\pm$0.16 & 5.81$\pm$0.51 & 58928$\pm$96 \\
% J170429.0+42035 & 256.1208 & 4.343 & $-$0.104$\pm$0.075 & 83$\pm$11 & 10.9$\pm$1.5 & 0.484$\pm$0.068 & 6.57$\pm$0.11 & 60738$\pm$12 \\
% J170433.6$-$85552 & 256.14 & $-$8.9312 & $-$0.054$\pm$0.087 & 84$\pm$13 & 10.4$\pm$1.5 & 0.446$\pm$0.081 & 5.66$\pm$0.11 & 60081$\pm$21 \\
% J170543.5+82728 & 256.4312 & 8.4576 & $-$0.106$\pm$0.057 & 24.8$\pm$2.2 & 10.49$\pm$0.98 & 0.35$\pm$0.11 & 6.332$\pm$0.066 & 60242$\pm$12 \\
% J170645.8+05156 & 256.6908 & 0.8656 & $-$0.03$\pm$0.50 & 69$\pm$16 & 19.3$\pm$8.3 & 0.25$\pm$0.16 & 7.056$\pm$0.067 & 60781$\pm$12 \\
% J170646.5+61714 & 256.6937 & 6.2873 & $-$0.10$\pm$0.59 & 18$\pm$24 & 5.9$\pm$8.9 & 0.45$\pm$0.20 & 1.461$\pm$0.084 & 5.8510$\pm$280 \\
% J170715.7$-$13503 & 256.8154 & $-$1.5841 & $-$0.59$\pm$0.18 & 25.4$\pm$4.9 & 6.9$\pm$1.3 & 0.434$\pm$0.059 & 4.43$\pm$0.13 & 60877.0$\pm$9.0 \\
% J170724.3$-$21751 & 256.8512 & $-$2.2976 & 0.004$\pm$0.020 & 22.5$\pm$2.0 & 17.5$\pm$1.2 & 0.612$\pm$0.023 & 7.19$\pm$0.10 & 60770.0$\pm$7.3 \\
% J170751.3$-$51238 & 256.9638 & $-$5.2105 & $-$0.149$\pm$0.045 & 43.8$\pm$4.7 & 5.33$\pm$0.23 & 0.558$\pm$0.015 & 12.52$\pm$0.14 & 60656.5$\pm$6.6 \\
% J170931.9$-$14917 & 257.3829 & $-$1.8214 & $-$0.105$\pm$0.094 & 26.3$\pm$4.0 & 12.3$\pm$2.1 & 0.726$\pm$0.031 & 5.91$\pm$0.18 & 60706$\pm$13 \\
% J171111.6+82317 & 257.7983 & 8.3882 & $-$0.584$\pm$0.010 & 27.02$\pm$0.25 & 17.03$\pm$0.17 & 0.602$\pm$0.021 & 12.048$\pm$0.059 & 60287.6$\pm$2.6 \\
% J171130.9+92128 & 257.8787 & 9.3577 & $-$0.756$\pm$0.081 & 14.4$\pm$1.8 & 3.14$\pm$0.28 & 0.697$\pm$0.035 & 4.513$\pm$0.093 & 60891$\pm$42 \\
% J171208.0+53932 & 258.0333 & 5.6589 & $-$0.795$\pm$0.020 & 25.65$\pm$0.86 & 8.63$\pm$0.69 & 0.642$\pm$0.030 & 7.23$\pm$0.11 & 60618.2$\pm$4.9 \\
% J171244.0+52400 & 258.1833 & 5.3999 & $-$0.326$\pm$0.085 & 32.7$\pm$8.9 & 13.7$\pm$1.8 & 0.674$\pm$0.038 & 5.521$\pm$0.048 & 60161.7$\pm$9.8 \\
% J171258.3+10200 & 258.2429 & 1.0333 & 0.25$\pm$0.65 & 43$\pm$15 & 14.6$\pm$4.2 & 0.60$\pm$0.12 & 13.7$\pm$1.2 & 60098$\pm$47 \\
% J171409.6+33321 & 258.54 & 3.5558 & $-$0.597$\pm$0.037 & 11.8$\pm$5.0 & 3.4$\pm$6.8 & 0.694$\pm$0.044 & 7.32$\pm$0.19 & 61086$\pm$99 \\
% J171440.6+51238 & 258.6692 & 5.2106 & $-$0.178$\pm$0.063 & 74.9$\pm$8.8 & 28.2$\pm$2.4 & 0.120$\pm$0.078 & 10.576$\pm$0.053 & 60732.7$\pm$1.9 \\
% J171606.7+70847 & 259.0279 & 7.1464 & $-$0.345$\pm$0.029 & 22.4$\pm$2.0 & 10.80$\pm$0.39 & 0.650$\pm$0.016 & 7.103$\pm$0.098 & 60744.8$\pm$5.5 \\
% J171619.2+13307 & 259.08 & 1.5518 & $-$0.588$\pm$0.038 & 14.3$\pm$3.6 & 4.79$\pm$0.44 & 0.775$\pm$0.021 & 6.406$\pm$0.097 & 60987$\pm$17 \\
% J171640.5$-$71122 & 259.1688 & $-$7.1894 & $-$0.434$\pm$0.010 & 25.6$\pm$1.9 & 10.83$\pm$0.48 & 0.691$\pm$0.011 & 8.653$\pm$0.046 & 60490.5$\pm$5.4 \\
% J171914.2+21556 & 259.8092 & 2.2656 & 0.12$\pm$0.55 & 77$\pm$30 & 4.1$\pm$5.7 & 0.30$\pm$0.14 & 5.4$\pm$1.1 & 60985$\pm$67 \\
% J172135.0+54909 & 260.3958 & 5.8192 & $-$0.822$\pm$0.069 & 25.6$\pm$3.1 & 6.5$\pm$2.1 & 0.36$\pm$0.11 & 3.491$\pm$0.098 & 60423.9$\pm$9.4 \\
% J172417.6+83346 & 261.0733 & 8.5628 & $-$0.17$\pm$0.33 & 2$\pm$19 & 40$\pm$14 & 0.08$\pm$0.23 & 9.709$\pm$0.096 & 58542$\pm$26 \\
% J172556.5+03047 & 261.4854 & 0.5131 & $-$0.4248$\pm$0.0047 & 57.7$\pm$2.4 & 13.29$\pm$0.13 & 0.490$\pm$0.022 & 51.317$\pm$0.062 & 60678.8$\pm$1.2 \\
% J172623.7+42358 & 261.5987 & 4.3993 & 0.42$\pm$0.59 & 28.3$\pm$6.8 & 15.5$\pm$7.4 & 0.01$\pm$0.23 & 9.49$\pm$0.26 & 5.9520$\pm$150 \\
% J172945.4+41613 & 262.4392 & 4.2701 & $-$0.738$\pm$0.073 & 16.0$\pm$3.5 & 5.41$\pm$0.71 & 0.594$\pm$0.070 & 4.932$\pm$0.058 & 61229$\pm$29 \\
% J173149.6+22135 & 262.9567 & 2.3598 & $-$0.444$\pm$0.089 & 32.5$\pm$9.2 & 8.74$\pm$0.20 & 0.547$\pm$0.084 & 6.745$\pm$0.068 & 60336$\pm$11 \\
% J173253.0+85830 & 263.2208 & 8.9749 & 0.09$\pm$0.58 & 53$\pm$10 & 12.9$\pm$4.7 & 0.56$\pm$0.20 & 67.8$\pm$1.2 & 60668.5$\pm$4.2 \\
% J173324.4+92142 & 263.3517 & 9.3616 & 0.253$\pm$0.030 & 22.26$\pm$0.57 & 18.32$\pm$0.27 & 0.463$\pm$0.013 & 11.551$\pm$0.056 & 60753.5$\pm$1.8 \\
% J173400.5$-$33811 & 263.5021 & $-$3.6364 & $-$1.12$\pm$0.50 & 4$\pm$15 & 1$\pm$11 & 0.60$\pm$0.13 & 3.35$\pm$0.17 & 59704$\pm$38 \\
% J173445.7+20146 & 263.6904 & 2.0294 & $-$0.759$\pm$0.061 & 18.2$\pm$1.6 & 2.49$\pm$0.13 & 0.660$\pm$0.061 & 4.438$\pm$0.062 & 61290$\pm$31 \\
% % J173500.8$-$73321 & 263.7533 & $-$7.5558 & \mathrm{nan}$\pm$\mathrm{nan} & 92.0$\pm$4.4 & 7.96$\pm$0.24 & 0.324$\pm$0.033 & 10.334$\pm$0.082 & 60804.2$\pm$7.8 \\
% J173654.7$-$73133 & 264.2279 & $-$7.5258 & $-$0.76$\pm$0.50 & 24$\pm$20 & 3$\pm$16 & 0.48$\pm$0.18 & 11.01$\pm$0.36 & 59680$\pm$140 \\
% J173709.8+92804 & 264.2908 & 9.4678 & $-$0.207$\pm$0.011 & 11.6$\pm$1.2 & 9.592$\pm$0.095 & 0.7054$\pm$0.0071 & 16.216$\pm$0.072 & 60770.2$\pm$2.3 \\
% J173816.0+12539 & 264.5667 & 1.4275 & $-$0.78$\pm$0.14 & 58.0$\pm$7.5 & 7.5$\pm$1.6 & 0.681$\pm$0.018 & 4.82$\pm$0.11 & 60737$\pm$15 \\
% J173933.1$-$34756 & 264.8879 & $-$3.7988 & $-$0.30$\pm$0.48 & 10.9$\pm$7.6 & 2$\pm$15 & 0.638$\pm$0.081 & 22.76$\pm$0.84 & 58110$\pm$430 \\
% J173942.2+01018 & 264.9258 & 0.1717 & $-$0.36$\pm$0.49 & 87$\pm$19 & 7.1$\pm$8.3 & 0.422$\pm$0.054 & 35.64$\pm$0.42 & 60566$\pm$43 \\
% J173950.6+31810 & 264.9608 & 3.3027 & $-$0.59$\pm$0.43 & 26$\pm$24 & 4.2$\pm$7.0 & 0.54$\pm$0.21 & 3.864$\pm$0.092 & 60739$\pm$54 \\
% J174054.7+75102 & 265.2279 & 7.8505 & $-$0.118$\pm$0.064 & 33$\pm$15 & 15.4$\pm$1.9 & 0.641$\pm$0.071 & 5.008$\pm$0.059 & 60707.9$\pm$8.3 \\
% J174147.8+13300 & 265.4492 & 1.55 & $-$0.32$\pm$0.29 & 27$\pm$24 & 6.0$\pm$4.7 & 0.672$\pm$0.082 & 8.30$\pm$0.13 & 59987$\pm$73 \\
% J174349.3+61031 & 265.9554 & 6.1753 & $-$0.221$\pm$0.026 & 28.21$\pm$0.91 & 7.46$\pm$0.11 & 0.6656$\pm$0.0064 & 14.418$\pm$0.093 & 60626.7$\pm$7.5 \\
% J174430.9+14321 & 266.1287 & 1.7225 & $-$0.742$\pm$0.031 & 25.97$\pm$0.50 & 4.49$\pm$0.26 & 0.667$\pm$0.019 & 6.390$\pm$0.068 & 60759.3$\pm$8.7 \\
% J174531.1+34804 & 266.3796 & 3.801 & $-$0.5832$\pm$0.0096 & 37.0$\pm$3.2 & 11.49$\pm$0.15 & 0.496$\pm$0.031 & 12.174$\pm$0.056 & 60662.8$\pm$3.1 \\
% J175148.9+80525 & 267.9538 & 8.0904 & $-$0.77$\pm$0.66 & 41$\pm$22 & 10.2$\pm$5.2 & 0.45$\pm$0.22 & 5.93$\pm$0.10 & 60155$\pm$25 \\
% J175157.0+02220 & 267.9875 & 0.3722 & $-$0.945$\pm$0.099 & 31$\pm$12 & 36.5$\pm$2.5 & 0.363$\pm$0.016 & 4.281$\pm$0.056 & 60308.3$\pm$5.9 \\
% J175443.5+64643 & 268.6812 & 6.7787 & $-$0.357$\pm$0.084 & 51$\pm$16 & 9.84$\pm$0.98 & 0.521$\pm$0.031 & 3.467$\pm$0.055 & 60288$\pm$11 \\
% J175556.8+03441 & 268.9867 & 0.5781 & 0.080$\pm$0.038 & 91.8$\pm$6.2 & 15.6$\pm$1.5 & 0.427$\pm$0.048 & 5.349$\pm$0.074 & 60462.5$\pm$8.2 \\
% J175709.8+85629 & 269.2908 & 8.9412 & 0.01$\pm$0.29 & 53.7$\pm$9.5 & 24.1$\pm$5.5 & 0.582$\pm$0.053 & 56.9$\pm$8.0 & 60444.0$\pm$1.4 \\
% J175713.1+10242 & 269.3046 & 1.0451 & $-$0.55$\pm$0.32 & 29.5$\pm$8.6 & 3.42$\pm$0.41 & 0.42$\pm$0.13 & 2.92$\pm$0.16 & 59648$\pm$24 \\
% J175736.1+31939 & 269.4004 & 3.3274 & $-$0.061$\pm$0.085 & 61$\pm$24 & 22.2$\pm$3.5 & 0.53$\pm$0.12 & 5.631$\pm$0.064 & 60208.4$\pm$6.4 \\
% J175742.7$-$13552 & 269.4279 & $-$1.5978 & $-$0.08$\pm$0.11 & 86.3$\pm$9.6 & 7.1$\pm$1.1 & 0.40$\pm$0.10 & 6.322$\pm$0.090 & 60603$\pm$10 \\
% J180006.4+14941 & 270.0267 & 1.8281 & 0.50$\pm$0.59 & 75$\pm$14 & 8.8$\pm$1.9 & 0.420$\pm$0.065 & 5.80$\pm$0.12 & 60629$\pm$11 \\
% J180044.3+43159 & 270.1846 & 4.5331 & $-$0.643$\pm$0.043 & 27.3$\pm$1.4 & 4.34$\pm$0.43 & 0.591$\pm$0.073 & 4.109$\pm$0.049 & 60241$\pm$38 \\
% J180051.8+83130 & 270.2158 & 8.5249 & $-$0.34$\pm$0.41 & 34$\pm$18 & 10$\pm$12 & 0.06$\pm$0.16 & 3.655$\pm$0.080 & 59420$\pm$210 \\
% J180347.2$-$11626 & 270.9467 & $-$1.274 & $-$0.193$\pm$0.038 & 26.92$\pm$0.98 & 6.88$\pm$0.21 & 0.698$\pm$0.011 & 7.366$\pm$0.072 & 60562.0$\pm$7.4 \\
% J180402.3$-$03551 & 271.0096 & $-$0.5975 & $-$0.132$\pm$0.085 & 78$\pm$16 & 6.35$\pm$0.57 & 0.30$\pm$0.15 & 9.619$\pm$0.085 & 60870.9$\pm$9.2 \\
% J180430.7+85857 & 271.1279 & 8.9826 & $-$0.60$\pm$0.51 & 40$\pm$19 & 8.0$\pm$7.5 & 0.04$\pm$0.26 & 4.46$\pm$0.62 & 59760$\pm$430 \\
% J180928.5+11405 & 272.3687 & 1.2346 & $-$0.58$\pm$0.40 & 81$\pm$29 & 32.1$\pm$3.7 & 0.00$\pm$0.27 & 104.5$\pm$1.3 & 60302$\pm$25 \\
% J181523.7+44921 & 273.8487 & 4.8225 & $-$0.1068$\pm$0.0062 & 97.87$\pm$0.36 & 12.198$\pm$0.062 & 0.352$\pm$0.011 & 44.46$\pm$0.15 & 60719.9$\pm$2.1 \\
% J182644.5+90406 & 276.6854 & 9.0683 & $-$0.435$\pm$0.011 & 36.6$\pm$4.4 & 5.80$\pm$0.46 & 0.450$\pm$0.068 & 5.219$\pm$0.082 & 60044.0$\pm$8.8 \\
% J182941.0+35533 & 277.4208 & 3.9258 & $-$0.01$\pm$0.77 & 28$\pm$15 & 14$\pm$10 & 0.15$\pm$0.26 & 2.971$\pm$0.081 & 59610$\pm$120 \\
% J183220.5+53648 & 278.0854 & 5.6134 & 0.51$\pm$0.82 & 23$\pm$14 & 24$\pm$13 & 0.21$\pm$0.19 & 14.83$\pm$0.33 & 59597$\pm$55 \\
% J183704.1+90924 & 279.2671 & 9.1567 & $-$0.530$\pm$0.033 & 14.2$\pm$1.1 & 17.2$\pm$1.0 & 0.558$\pm$0.015 & 17.17$\pm$0.17 & 61023.3$\pm$3.0 \\
% J190710.6$-$34643 & 286.7942 & $-$3.7786 & $-$0.582$\pm$0.011 & 28.2$\pm$2.3 & 3.207$\pm$0.061 & 0.629$\pm$0.027 & 7.914$\pm$0.092 & 61093$\pm$14 \\
% J190855.9$-$50528 & 287.2329 & $-$5.091 & $-$0.496$\pm$0.070 & 26.3$\pm$1.9 & 9.5$\pm$1.9 & 0.598$\pm$0.089 & 3.502$\pm$0.047 & 60485.1$\pm$8.5 \\
% J191533.4$-$51109 & 288.8892 & $-$5.1859 & 0.011$\pm$0.016 & 25.06$\pm$0.99 & 16.47$\pm$0.35 & 0.494$\pm$0.028 & 3.879$\pm$0.055 & 60510.6$\pm$7.9 \\
% J191757.7$-$82651 & 289.4904 & $-$8.4475 & $-$0.526$\pm$0.020 & 12.99$\pm$0.29 & 6.33$\pm$0.20 & 0.674$\pm$0.011 & 25.98$\pm$0.16 & 60877.9$\pm$6.1 \\
% J191934.4$-$74043 & 289.8933 & $-$7.6787 & $-$0.95$\pm$0.36 & 11$\pm$18 & 2$\pm$16 & 0.55$\pm$0.12 & 45.63$\pm$0.17 & 59623$\pm$23 \\
% J191959.0$-$75726 & 289.9958 & $-$7.9571 & $-$0.779$\pm$0.021 & 17.98$\pm$0.65 & 4.453$\pm$0.071 & 0.7799$\pm$0.0096 & 13.088$\pm$0.076 & 60784.5$\pm$7.8 \\
% J192025.0$-$51943 & 290.1042 & $-$5.3287 & $-$0.941$\pm$0.017 & 43.9$\pm$9.6 & 6.6$\pm$1.1 & 0.606$\pm$0.035 & 5.26$\pm$0.15 & 60033$\pm$13 \\
% J192120.0$-$53432 & 290.3333 & $-$5.5756 & $-$0.68$\pm$0.15 & 14.8$\pm$6.9 & 3$\pm$17 & 0.67$\pm$0.13 & 20.16$\pm$0.55 & 61185$\pm$78 \\
% J192755.8+64249 & 291.9825 & 6.7136 & 0.54$\pm$0.23 & 21.1$\pm$3.9 & 10.30$\pm$0.40 & 0.666$\pm$0.020 & 6.107$\pm$0.062 & 60618.7$\pm$7.1 \\
% J192833.2$-$11047 & 292.1383 & $-$1.1796 & $-$0.44$\pm$0.14 & 31.5$\pm$7.0 & 9.0$\pm$5.6 & 0.483$\pm$0.084 & 14.65$\pm$0.21 & 60268$\pm$19 \\
% J192834.3+64907 & 292.1429 & 6.8186 & $-$0.3509$\pm$0.0058 & 63.6$\pm$6.1 & 5.29$\pm$0.30 & 0.356$\pm$0.064 & 6.015$\pm$0.074 & 60571.4$\pm$9.7 \\
% J193155.5$-$04537 & 292.9812 & $-$0.7603 & $-$0.360$\pm$0.066 & 58.0$\pm$6.5 & 10.7$\pm$1.8 & 0.462$\pm$0.046 & 8.382$\pm$0.091 & 60530.7$\pm$6.3 \\
% J193316.7$-$82240 & 293.3196 & $-$8.3777 & $-$1.32$\pm$0.13 & 10.7$\pm$8.6 & 2.85$\pm$0.78 & 0.45$\pm$0.15 & 3.285$\pm$0.098 & 60703$\pm$20 \\
% J193446.2$-$52903 & 293.6925 & $-$5.4841 & $-$0.67$\pm$0.11 & 27.9$\pm$1.5 & 6.15$\pm$0.36 & 0.533$\pm$0.061 & 3.342$\pm$0.082 & 60418$\pm$11 \\
% J193503.6$-$11106 & 293.765 & $-$1.1851 & 0.1718$\pm$0.0056 & 37.4$\pm$1.0 & 5.336$\pm$0.019 & 0.4146$\pm$0.0050 & 31.258$\pm$0.064 & 60092.2$\pm$2.2 \\
% J193545.2+41420 & 293.9383 & 4.2388 & 0.20$\pm$0.56 & 25$\pm$14 & 4.1$\pm$8.1 & 0.55$\pm$0.12 & 4.20$\pm$0.28 & 60814$\pm$47 \\
% J193637.5$-$61734 & 294.1562 & $-$6.2928 & $-$0.4415$\pm$0.0067 & 33.7$\pm$1.2 & 10.717$\pm$0.072 & 0.476$\pm$0.010 & 17.474$\pm$0.047 & 60278.31$\pm$0.73 \\
% J193907.0$-$41146 & 294.7792 & $-$4.1961 & $-$0.7937$\pm$0.0023 & 26.39$\pm$0.74 & 10.68$\pm$0.23 & 0.598$\pm$0.013 & 6.564$\pm$0.053 & 60429.1$\pm$4.8 \\
% J194132.9$-$81655 & 295.3871 & $-$8.2818 & $-$0.446$\pm$0.041 & 22.6$\pm$3.3 & 12.25$\pm$0.73 & 0.699$\pm$0.027 & 4.126$\pm$0.058 & 60541.8$\pm$6.1 \\
% J194444.6+74302 & 296.1858 & 7.7174 & $-$0.15$\pm$0.33 & 48$\pm$13 & 10.7$\pm$5.0 & 0.088$\pm$0.083 & 4.099$\pm$0.096 & 59944$\pm$39 \\
% J194652.3$-$50941 & 296.7179 & $-$5.1614 & $-$0.689$\pm$0.089 & 18.08$\pm$0.25 & 5.23$\pm$0.39 & 0.768$\pm$0.021 & 5.948$\pm$0.077 & 60658$\pm$12 \\
% J194751.6+42216 & 296.965 & 4.3711 & $-$1.068$\pm$0.012 & 11.08$\pm$0.42 & 4.41$\pm$0.40 & 0.6711$\pm$0.0034 & 71.04$\pm$0.11 & 60215.7$\pm$1.0 \\
% J194934.5+70834 & 297.3937 & 7.1427 & $-$0.245$\pm$0.018 & 20.0$\pm$1.4 & 7.59$\pm$0.15 & 0.619$\pm$0.030 & 7.47$\pm$0.10 & 60533.4$\pm$5.4 \\
% J195006.8$-$71643 & 297.5283 & $-$7.2785 & 0.196$\pm$0.022 & 48.5$\pm$3.9 & 8.76$\pm$0.19 & 0.560$\pm$0.019 & 7.727$\pm$0.061 & 60560.5$\pm$6.2 \\
% J195055.8+20043 & 297.7325 & 2.012 & $-$0.546$\pm$0.011 & 29.13$\pm$0.21 & 9.590$\pm$0.054 & 0.379$\pm$0.014 & 17.08$\pm$0.14 & 60900.1$\pm$2.3 \\
% J195111.1+60319 & 297.7962 & 6.0551 & $-$0.37$\pm$0.22 & 91$\pm$25 & 11.7$\pm$4.6 & 0.08$\pm$0.18 & 8.812$\pm$0.053 & 60607.6$\pm$6.7 \\
% J195217.6$-$452819 & 298.0733 & $-$45.472 & $-$0.569$\pm$0.016 & 23.95$\pm$0.40 & 2.799$\pm$0.049 & 0.386$\pm$0.020 & 5.567$\pm$0.072 & 60107.6$\pm$6.5 \\
% J195235.6$-$65707 & 298.1483 & $-$6.9519 & $-$0.063$\pm$0.018 & 14.07$\pm$0.31 & 6.69$\pm$0.67 & 0.486$\pm$0.022 & 8.01$\pm$0.13 & 60161.1$\pm$2.3 \\
% J195341.4+91739 & 298.4225 & 9.2942 & $-$0.732$\pm$0.011 & 26.05$\pm$0.27 & 9.99$\pm$0.12 & 0.6484$\pm$0.0062 & 28.961$\pm$0.071 & 60765.4$\pm$1.1 \\
% J195344.9$-$555611 & 298.4371 & $-$55.9363 & $-$0.2139$\pm$0.0076 & 16.02$\pm$0.33 & 10.95$\pm$0.22 & 0.683$\pm$0.014 & 6.238$\pm$0.038 & 60693.8$\pm$4.4 \\
% J195457.9$-$84029 & 298.7412 & $-$8.6746 & $-$0.630$\pm$0.088 & 26.9$\pm$1.9 & 5.34$\pm$0.36 & 0.418$\pm$0.041 & 5.37$\pm$0.15 & 59779$\pm$16 \\
% J195606.7+73633 & 299.0279 & 7.6092 & $-$0.47$\pm$0.16 & 45$\pm$11 & 8.2$\pm$1.5 & 0.320$\pm$0.089 & 4.472$\pm$0.071 & 60040.0$\pm$9.1 \\
% J195818.1+63014 & 299.5754 & 6.5038 & $-$0.772$\pm$0.075 & 26.00$\pm$0.29 & 7.127$\pm$0.061 & 0.610$\pm$0.017 & 4.922$\pm$0.074 & 60779.7$\pm$8.1 \\
% J195909.1$-$81623 & 299.7879 & $-$8.2731 & $-$0.15$\pm$0.18 & 29$\pm$27 & 11.3$\pm$1.6 & 0.51$\pm$0.23 & 8.880$\pm$0.060 & 60840.5$\pm$5.7 \\
% J200150.2$-$61943 & 300.4592 & $-$6.3287 & 0.1544$\pm$0.0049 & 41.9$\pm$4.0 & 9.45$\pm$0.18 & 0.634$\pm$0.015 & 9.392$\pm$0.043 & 60643.7$\pm$4.4 \\
% J200242.9$-$82538 & 300.6788 & $-$8.4272 & $-$0.434$\pm$0.011 & 96.9$\pm$1.1 & 11.13$\pm$0.24 & 0.371$\pm$0.015 & 16.515$\pm$0.067 & 60257.0$\pm$3.7 \\
% J200341.5$-$312952 & 300.9229 & $-$31.4978 & $-$0.009$\pm$0.040 & 46.6$\pm$2.0 & 9.17$\pm$0.38 & 0.471$\pm$0.011 & 13.81$\pm$0.15 & 60436.3$\pm$2.8 \\
% J200456.5$-$310951 & 301.2354 & $-$31.1641 & $-$0.7687$\pm$0.0096 & 42$\pm$10 & 7.40$\pm$0.92 & 0.414$\pm$0.048 & 9.628$\pm$0.070 & 60147$\pm$14 \\
% J200544.9$-$341516 & 301.4371 & $-$34.2544 & $-$0.585$\pm$0.011 & 32.3$\pm$2.8 & 8.58$\pm$0.22 & 0.652$\pm$0.022 & 9.668$\pm$0.063 & 60584.9$\pm$3.5 \\
% J201056.9$-$03427 & 302.7371 & $-$0.5741 & $-$0.83$\pm$0.32 & 30.6$\pm$7.1 & 3.6$\pm$7.3 & 0.544$\pm$0.079 & 6.91$\pm$0.14 & 60839$\pm$41 \\
% J201112.8+71332 & 302.8033 & 7.2257 & $-$0.105$\pm$0.020 & 5.2$\pm$1.4 & 31.90$\pm$0.21 & 0.428$\pm$0.040 & 7.593$\pm$0.046 & 60165.1$\pm$2.4 \\
% J201133.7$-$335857 & 302.8904 & $-$33.9826 & $-$0.3730$\pm$0.0033 & 43.3$\pm$2.4 & 10.20$\pm$0.10 & 0.396$\pm$0.020 & 13.345$\pm$0.044 & 60561.8$\pm$1.8 \\
% J201226.5$-$303946 & 303.1104 & $-$30.6629 & $-$0.346$\pm$0.033 & 34$\pm$13 & 28.5$\pm$2.9 & 0.477$\pm$0.044 & 10.918$\pm$0.038 & 60098.7$\pm$8.2 \\
% J201326.5$-$45058 & 303.3604 & $-$4.8496 & 0.059$\pm$0.014 & 27.2$\pm$3.0 & 6.18$\pm$0.29 & 0.562$\pm$0.020 & 5.578$\pm$0.092 & 60642.0$\pm$9.4 \\
% J201422.1$-$75702 & 303.5921 & $-$7.9504 & $-$0.96$\pm$0.32 & 9$\pm$11 & 14.3$\pm$5.9 & 0.458$\pm$0.069 & 10.2$\pm$1.6 & 61081$\pm$21 \\
% J201931.1+54141 & 304.8796 & 5.6947 & $-$0.44$\pm$0.34 & 5$\pm$16 & 3$\pm$14 & 0.69$\pm$0.24 & 6.93$\pm$0.31 & 60915$\pm$85 \\
% J202049.5$-$284823 & 305.2062 & $-$28.8062 & $-$0.384$\pm$0.063 & 39$\pm$14 & 32.0$\pm$3.8 & 0.225$\pm$0.074 & 3.594$\pm$0.049 & 61045.4$\pm$4.9 \\
% J202108.8$-$355527 & 305.2867 & $-$35.9242 & $-$0.621$\pm$0.011 & 18.66$\pm$0.34 & 7.323$\pm$0.045 & 0.701$\pm$0.010 & 9.503$\pm$0.044 & 60565.7$\pm$2.3 \\
% J202649.5+45957 & 306.7062 & 4.9991 & $-$0.646$\pm$0.094 & 28.7$\pm$3.0 & 6.11$\pm$0.23 & 0.560$\pm$0.030 & 5.116$\pm$0.076 & 60199$\pm$15 \\
% J202840.7$-$305610 & 307.1696 & $-$30.9362 & $-$0.950$\pm$0.011 & 56.7$\pm$8.1 & 4.0$\pm$1.1 & 0.114$\pm$0.080 & 5.74$\pm$0.20 & 60064$\pm$16 \\
% J203310.5$-$444453 & 308.2938 & $-$44.748 & $-$0.679$\pm$0.048 & 32.4$\pm$5.1 & 10.1$\pm$1.5 & 0.417$\pm$0.046 & 9.935$\pm$0.033 & 60188.4$\pm$7.5 \\
% J203313.7$-$442324 & 308.3071 & $-$44.3899 & $-$0.395$\pm$0.010 & 59.0$\pm$6.5 & 15.5$\pm$1.7 & 0.330$\pm$0.042 & 14.998$\pm$0.033 & 60138.3$\pm$4.4 \\
% J203505.4$-$71131 & 308.7725 & $-$7.1919 & $-$0.651$\pm$0.036 & 26.01$\pm$0.31 & 7.20$\pm$0.17 & 0.622$\pm$0.018 & 13.598$\pm$0.076 & 60615.7$\pm$4.0 \\
% J203515.8$-$290340 & 308.8158 & $-$29.0611 & $-$0.206$\pm$0.054 & 92.3$\pm$5.3 & 22.8$\pm$1.5 & 0.224$\pm$0.041 & 18.09$\pm$0.11 & 60561.0$\pm$1.7 \\
% J203629.2$-$51304 & 309.1217 & $-$5.2177 & $-$0.92$\pm$0.37 & 25.7$\pm$6.4 & 9$\pm$12 & 0.54$\pm$0.16 & 24.86$\pm$0.32 & 60614$\pm$26 \\
% J203909.1$-$304521 & 309.7879 & $-$30.7558 & $-$0.81$\pm$0.17 & 14.8$\pm$8.5 & 2$\pm$11 & 0.342$\pm$0.081 & 6.34$\pm$0.59 & 61110$\pm$130 \\
% J204847.1$-$435933 & 312.1962 & $-$43.9925 & $-$0.571$\pm$0.026 & 29.5$\pm$1.5 & 6.25$\pm$0.17 & 0.362$\pm$0.021 & 5.370$\pm$0.041 & 60575.0$\pm$5.8 \\
% J205155.8$-$365522 & 312.9825 & $-$36.9229 & $-$0.5493$\pm$0.0059 & 27.23$\pm$0.16 & 14.86$\pm$0.12 & 0.5595$\pm$0.0028 & 51.343$\pm$0.032 & 60846.61$\pm$0.53 \\
% J205655.7+02032 & 314.2321 & 0.3422 & $-$0.7601$\pm$0.0050 & 84$\pm$12 & 2.94$\pm$0.41 & 0.416$\pm$0.089 & 10.96$\pm$0.47 & 60116$\pm$13 \\
% J210249.3$-$483804 & 315.7054 & $-$48.6345 & $-$0.80$\pm$0.43 & 14$\pm$23 & 2$\pm$17 & 0.51$\pm$0.18 & 2.249$\pm$0.076 & 59528$\pm$75 \\
% J211429.8$-$05218 & 318.6242 & $-$0.8716 & $-$0.65$\pm$0.22 & 17.9$\pm$5.4 & 30.3$\pm$5.4 & 0.052$\pm$0.073 & 13.404$\pm$0.089 & 60714.7$\pm$5.0 \\
% J211603.2$-$75323 & 319.0133 & $-$7.8897 & $-$0.26$\pm$0.41 & 45$\pm$18 & 10.9$\pm$5.2 & 0.616$\pm$0.092 & 20.8$\pm$2.9 & 60181.7$\pm$7.6 \\
% J211611.4+11813 & 319.0475 & 1.3036 & $-$0.63$\pm$0.34 & 3$\pm$21 & 3$\pm$13 & 0.77$\pm$0.20 & 4.874$\pm$0.077 & 59180$\pm$150 \\
% J211725.0$-$03453 & 319.3542 & $-$0.5814 & $-$0.24$\pm$0.54 & 4.8$\pm$4.5 & 8.1$\pm$2.0 & 0.686$\pm$0.074 & 3.442$\pm$0.050 & 60500$\pm$13 \\
% J211751.1$-$91909 & 319.4629 & $-$9.3191 & 0.050$\pm$0.020 & 31$\pm$12 & 16.60$\pm$0.58 & 0.641$\pm$0.025 & 6.941$\pm$0.054 & 60206.7$\pm$7.7 \\
% J211914.3$-$355239 & 319.8096 & $-$35.8775 & $-$0.772$\pm$0.019 & 89.5$\pm$5.4 & 3.55$\pm$0.17 & 0.155$\pm$0.038 & 8.24$\pm$0.43 & 59945$\pm$16 \\
% J212506.8$-$53639 & 321.2783 & $-$5.6109 & $-$0.446$\pm$0.030 & 32.0$\pm$1.9 & 4.226$\pm$0.078 & 0.4818$\pm$0.0099 & 12.558$\pm$0.060 & 61006$\pm$21 \\
% % J214147.3+61116 & 325.4471 & 6.1878 & \mathrm{nan}$\pm$\mathrm{nan} & 28.337$\pm$0.096 & 19.36$\pm$0.35 & 0.396$\pm$0.022 & 8.502$\pm$0.052 & 60203.8$\pm$4.1 \\
% J214148.2+43820 & 325.4508 & 4.6388 & $-$0.37$\pm$0.14 & 47.1$\pm$4.4 & 13.5$\pm$3.2 & 0.503$\pm$0.050 & 5.791$\pm$0.079 & 60538.3$\pm$6.5 \\
% J220242.1+43638 & 330.6754 & 4.6105 & $-$0.822$\pm$0.070 & 13.3$\pm$6.2 & 6.97$\pm$0.38 & 0.665$\pm$0.099 & 8.82$\pm$0.11 & 60516.9$\pm$2.4 \\
% J220651.7+64951 & 331.7154 & 6.8308 & $-$0.77$\pm$0.17 & 18$\pm$15 & 9.1$\pm$6.2 & 0.703$\pm$0.098 & 16.5$\pm$2.2 & 60394.9$\pm$6.7 \\
% J220717.4$-$80210 & 331.8225 & $-$8.0362 & $-$0.02$\pm$0.20 & 3.6$\pm$2.0 & 19.6$\pm$4.8 & 0.510$\pm$0.030 & 25.56$\pm$0.26 & 60801$\pm$14 \\
% J220755.3+93305 & 331.9804 & 9.5514 & $-$0.44$\pm$0.65 & 16.8$\pm$6.6 & 6.1$\pm$2.1 & 0.40$\pm$0.15 & 17.7$\pm$1.3 & 60915$\pm$35 \\
% J231919.0$-$445903 & 349.8292 & $-$44.9842 & $-$0.279$\pm$0.011 & 28.81$\pm$0.48 & 7.443$\pm$0.049 & 0.296$\pm$0.033 & 8.089$\pm$0.080 & 60045.0$\pm$4.2 \\

==> ese_prop_extended_lcs.tex <==

\begin{figure*}
\centering
\gridline{\fig{lcs/J01h50m09.8s-45d22m55.2s_lc_fit_full.pdf}{0.24\linewidth}{J01h50m09.8s$-$45d22m55.2s}
	\fig{lcs/J03h58m55.3s+06d34m40.1s_lc_fit_full.pdf}{0.24\linewidth}{J03h58m55.3s+06d34m40.1s}
	\fig{lcs/J04h03m58.8s+06d45m38.9s_lc_fit_full.pdf}{0.24\linewidth}{J04h03m58.8s+06d45m38.9s}
	\fig{lcs/J04h08m00.2s-32d50m02.5s_lc_fit_full.pdf}{0.24\linewidth}{J04h08m00.2s$-$32d50m02.5s}}
\gridline{\fig{lcs/J04h27m22.4s-49d07m41.9s_lc_fit_full.pdf}{0.24\linewidth}{J04h27m22.4s$-$49d07m41.9s}
	\fig{lcs/J04h51m27.2s+08d12m53.7s_lc_fit_full.pdf}{0.24\linewidth}{J04h51m27.2s+08d12m53.7s}
	\fig{lcs/J05h00m04.8s+00d14m20.8s_lc_fit_full.pdf}{0.24\linewidth}{J05h00m04.8s+00d14m20.8s}
	\fig{lcs/J05h09m12.5s-45d22m19.2s_lc_fit_full.pdf}{0.24\linewidth}{J05h09m12.5s$-$45d22m19.2s}}
\gridline{\fig{lcs/J05h12m32.0s-02d58m29.1s_lc_fit_full.pdf}{0.24\linewidth}{J05h12m32.0s$-$02d58m29.1s}
	\fig{lcs/J05h13m41.0s-09d22m14.6s_lc_fit_full.pdf}{0.24\linewidth}{J05h13m41.0s$-$09d22m14.6s}
	\fig{lcs/J05h23m25.7s+01d58m37.2s_lc_fit_full.pdf}{0.24\linewidth}{J05h23m25.7s+01d58m37.2s}
	\fig{lcs/J05h52m02.1s-30d09m36.1s_lc_fit_full.pdf}{0.24\linewidth}{J05h52m02.1s$-$30d09m36.1s}}
\gridline{\fig{lcs/J07h40m04.9s+04d15m28.6s_lc_fit_full.pdf}{0.24\linewidth}{J07h40m04.9s+04d15m28.6s}
	\fig{lcs/J08h54m39.5s+08d43m25.7s_lc_fit_full.pdf}{0.24\linewidth}{J08h54m39.5s+08d43m25.7s}
	\fig{lcs/J09h42m15.5s+04d36m22.1s_lc_fit_full.pdf}{0.24\linewidth}{J09h42m15.5s+04d36m22.1s}
	\fig{lcs/J10h24m43.5s-37d33m47.2s_lc_fit_full.pdf}{0.24\linewidth}{J10h24m43.5s$-$37d33m47.2s}}
\gridline{\fig{lcs/J10h44m24.0s-30d40m58.0s_lc_fit_full.pdf}{0.24\linewidth}{J10h44m24.0s$-$30d40m58.0s}
	\fig{lcs/J11h02m20.7s+01d42m05.5s_lc_fit_full.pdf}{0.24\linewidth}{J11h02m20.7s+01d42m05.5s}
	\fig{lcs/J11h32m59.3s-48d42m35.1s_lc_fit_full.pdf}{0.24\linewidth}{J11h32m59.3s$-$48d42m35.1s}
	\fig{lcs/J12h50m02.7s-50d41m48.7s_lc_fit_full.pdf}{0.24\linewidth}{J12h50m02.7s$-$50d41m48.7s}}
\caption{Light curves of the ESE candidates in the VAST silver sample. \label{fig:ese_ext_lcs_1}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J13h00m23.0s-42d08m39.3s_lc_fit_full.pdf}{0.24\linewidth}{J13h00m23.0s$-$42d08m39.3s}
	\fig{lcs/J13h24m42.8s-50d20m37.8s_lc_fit_full.pdf}{0.24\linewidth}{J13h24m42.8s$-$50d20m37.8s}
	\fig{lcs/J13h41m17.8s-49d03m36.8s_lc_fit_full.pdf}{0.24\linewidth}{J13h41m17.8s$-$49d03m36.8s}
	\fig{lcs/J13h48m31.0s-30d35m36.2s_lc_fit_full.pdf}{0.24\linewidth}{J13h48m31.0s$-$30d35m36.2s}}
\gridline{\fig{lcs/J13h49m22.2s+07d12m17.6s_lc_fit_full.pdf}{0.24\linewidth}{J13h49m22.2s+07d12m17.6s}
	\fig{lcs/J14h19m45.9s-08d27m06.4s_lc_fit_full.pdf}{0.24\linewidth}{J14h19m45.9s$-$08d27m06.4s}
	\fig{lcs/J15h06m37.4s+00d25m40.4s_lc_fit_full.pdf}{0.24\linewidth}{J15h06m37.4s+00d25m40.4s}
	\fig{lcs/J15h17m38.6s+03d45m28.3s_lc_fit_full.pdf}{0.24\linewidth}{J15h17m38.6s+03d45m28.3s}}
\gridline{\fig{lcs/J15h19m51.3s-09d18m48.8s_lc_fit_full.pdf}{0.24\linewidth}{J15h19m51.3s$-$09d18m48.8s}
	\fig{lcs/J15h29m14.4s-04d14m07.6s_lc_fit_full.pdf}{0.24\linewidth}{J15h29m14.4s$-$04d14m07.6s}
	\fig{lcs/J15h42m36.1s-05d47m55.4s_lc_fit_full.pdf}{0.24\linewidth}{J15h42m36.1s$-$05d47m55.4s}
	\fig{lcs/J16h02m20.5s-04d25m36.5s_lc_fit_full.pdf}{0.24\linewidth}{J16h02m20.5s$-$04d25m36.5s}}
\gridline{\fig{lcs/J16h05m56.9s-01d09m49.3s_lc_fit_full.pdf}{0.24\linewidth}{J16h05m56.9s$-$01d09m49.3s}
	\fig{lcs/J16h27m12.9s+04d18m34.6s_lc_fit_full.pdf}{0.24\linewidth}{J16h27m12.9s+04d18m34.6s}
	\fig{lcs/J16h27m47.9s-09d01m06.4s_lc_fit_full.pdf}{0.24\linewidth}{J16h27m47.9s$-$09d01m06.4s}
	\fig{lcs/J16h30m07.9s-04d51m35.9s_lc_fit_full.pdf}{0.24\linewidth}{J16h30m07.9s$-$04d51m35.9s}}
\gridline{\fig{lcs/J16h31m55.3s-08d30m08.2s_lc_fit_full.pdf}{0.24\linewidth}{J16h31m55.3s$-$08d30m08.2s}
	\fig{lcs/J16h39m39.0s+09d07m36.5s_lc_fit_full.pdf}{0.24\linewidth}{J16h39m39.0s+09d07m36.5s}
	\fig{lcs/J16h39m51.1s+01d16m50.4s_lc_fit_full.pdf}{0.24\linewidth}{J16h39m51.1s+01d16m50.4s}
	\fig{lcs/J16h40m43.3s-01d33m41.5s_lc_fit_full.pdf}{0.24\linewidth}{J16h40m43.3s$-$01d33m41.5s}}
\caption{Light curves of the ESE candidates in the VAST silver sample. \label{fig:ese_ext_lcs_2}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J16h41m00.2s+05d58m10.6s_lc_fit_full.pdf}{0.24\linewidth}{J16h41m00.2s+05d58m10.6s}
	\fig{lcs/J16h46m13.0s+05d17m50.1s_lc_fit_full.pdf}{0.24\linewidth}{J16h46m13.0s+05d17m50.1s}
	\fig{lcs/J16h49m18.4s+09d21m43.7s_lc_fit_full.pdf}{0.24\linewidth}{J16h49m18.4s+09d21m43.7s}
	\fig{lcs/J16h51m07.1s+01d24m06.2s_lc_fit_full.pdf}{0.24\linewidth}{J16h51m07.1s+01d24m06.2s}}
\gridline{\fig{lcs/J16h59m22.1s-00d39m58.5s_lc_fit_full.pdf}{0.24\linewidth}{J16h59m22.1s$-$00d39m58.5s}
	\fig{lcs/J17h02m07.7s-07d46m45.8s_lc_fit_full.pdf}{0.24\linewidth}{J17h02m07.7s$-$07d46m45.8s}
	\fig{lcs/J17h04m29.0s+04d20m34.7s_lc_fit_full.pdf}{0.24\linewidth}{J17h04m29.0s+04d20m34.7s}
	\fig{lcs/J17h11m30.9s+09d21m27.7s_lc_fit_full.pdf}{0.24\linewidth}{J17h11m30.9s+09d21m27.7s}}
\gridline{\fig{lcs/J17h12m58.3s+01d01m59.8s_lc_fit_full.pdf}{0.24\linewidth}{J17h12m58.3s+01d01m59.8s}
	\fig{lcs/J17h16m40.5s-07d11m21.7s_lc_fit_full.pdf}{0.24\linewidth}{J17h16m40.5s$-$07d11m21.7s}
	\fig{lcs/J17h21m35.0s+05d49m09.3s_lc_fit_full.pdf}{0.24\linewidth}{J17h21m35.0s+05d49m09.3s}
	\fig{lcs/J17h14m09.6s+03d33m20.7s_lc_fit_full.pdf}{0.24\linewidth}{J17h14m09.6s+03d33m20.7s}}
\gridline{\fig{lcs/J17h31m49.6s+02d21m35.3s_lc_fit_full.pdf}{0.24\linewidth}{J17h31m49.6s+02d21m35.3s}
	\fig{lcs/J17h38m16.0s+01d25m39.1s_lc_fit_full.pdf}{0.24\linewidth}{J17h38m16.0s+01d25m39.1s}
	\fig{lcs/J17h39m50.6s+03d18m09.8s_lc_fit_full.pdf}{0.24\linewidth}{J17h39m50.6s+03d18m09.8s}
	\fig{lcs/J17h40m54.7s+07d51m01.9s_lc_fit_full.pdf}{0.24\linewidth}{J17h40m54.7s+07d51m01.9s}}
\gridline{\fig{lcs/J17h44m30.9s+01d43m21.0s_lc_fit_full.pdf}{0.24\linewidth}{J17h44m30.9s+01d43m21.0s}
	\fig{lcs/J17h51m48.9s+08d05m25.3s_lc_fit_full.pdf}{0.24\linewidth}{J17h51m48.9s+08d05m25.3s}
	\fig{lcs/J17h55m56.8s+00d34m41.1s_lc_fit_full.pdf}{0.24\linewidth}{J17h55m56.8s+00d34m41.1s}
	\fig{lcs/J17h57m36.1s+03d19m38.8s_lc_fit_full.pdf}{0.24\linewidth}{J17h57m36.1s+03d19m38.8s}}
\caption{Light curves of the ESE candidates in the VAST silver sample. \label{fig:ese_ext_lcs_3}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J17h57m42.7s-01d35m51.9s_lc_fit_full.pdf}{0.24\linewidth}{J17h57m42.7s$-$01d35m51.9s}
	\fig{lcs/J18h03m47.2s-01d16m26.4s_lc_fit_full.pdf}{0.24\linewidth}{J18h03m47.2s$-$01d16m26.4s}
	\fig{lcs/J18h26m44.5s+09d04m06.0s_lc_fit_full.pdf}{0.24\linewidth}{J18h26m44.5s+09d04m06.0s}
	\fig{lcs/J18h29m41.0s+03d55m32.7s_lc_fit_full.pdf}{0.24\linewidth}{J18h29m41.0s+03d55m32.7s}}
\gridline{\fig{lcs/J19h08m55.9s-05d05m27.6s_lc_fit_full.pdf}{0.24\linewidth}{J19h08m55.9s$-$05d05m27.6s}
	\fig{lcs/J19h15m33.4s-05d11m09.1s_lc_fit_full.pdf}{0.24\linewidth}{J19h15m33.4s$-$05d11m09.1s}
	\fig{lcs/J19h19m34.4s-07d40m43.2s_lc_fit_full.pdf}{0.24\linewidth}{J19h19m34.4s$-$07d40m43.2s}
	\fig{lcs/J19h19m59.0s-07d57m25.7s_lc_fit_full.pdf}{0.24\linewidth}{J19h19m59.0s$-$07d57m25.7s}}
\gridline{\fig{lcs/J19h20m25.0s-05d19m43.2s_lc_fit_full.pdf}{0.24\linewidth}{J19h20m25.0s$-$05d19m43.2s}
	\fig{lcs/J19h27m55.8s+06d42m49.0s_lc_fit_full.pdf}{0.24\linewidth}{J19h27m55.8s+06d42m49.0s}
	\fig{lcs/J19h28m34.3s+06d49m06.8s_lc_fit_full.pdf}{0.24\linewidth}{J19h28m34.3s+06d49m06.8s}
	\fig{lcs/J19h33m16.7s-08d22m39.7s_lc_fit_full.pdf}{0.24\linewidth}{J19h33m16.7s$-$08d22m39.7s}}
\gridline{\fig{lcs/J19h34m46.2s-05d29m02.8s_lc_fit_full.pdf}{0.24\linewidth}{J19h34m46.2s$-$05d29m02.8s}
	\fig{lcs/J19h39m07.0s-04d11m46.1s_lc_fit_full.pdf}{0.24\linewidth}{J19h39m07.0s$-$04d11m46.1s}
	\fig{lcs/J19h41m32.9s-08d16m54.5s_lc_fit_full.pdf}{0.24\linewidth}{J19h41m32.9s$-$08d16m54.5s}
	\fig{lcs/J19h46m52.3s-05d09m41.2s_lc_fit_full.pdf}{0.24\linewidth}{J19h46m52.3s$-$05d09m41.2s}}
\gridline{\fig{lcs/J19h51m11.1s+06d03m18.5s_lc_fit_full.pdf}{0.24\linewidth}{J19h51m11.1s+06d03m18.5s}
	\fig{lcs/J19h52m17.6s-45d28m19.3s_lc_fit_full.pdf}{0.24\linewidth}{J19h52m17.6s$-$45d28m19.3s}
	\fig{lcs/J19h53m44.9s-55d56m10.7s_lc_fit_full.pdf}{0.24\linewidth}{J19h53m44.9s$-$55d56m10.7s}
	\fig{lcs/J19h54m57.9s-08d40m28.6s_lc_fit_full.pdf}{0.24\linewidth}{J19h54m57.9s$-$08d40m28.6s}}
\caption{Light curves of the ESE candidates in the VAST silver sample. \label{fig:ese_ext_lcs_4}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J20h13m26.5s-04d50m58.4s_lc_fit_full.pdf}{0.24\linewidth}{J20h13m26.5s$-$04d50m58.4s}
	\fig{lcs/J20h19m31.1s+05d41m40.9s_lc_fit_full.pdf}{0.24\linewidth}{J20h19m31.1s+05d41m40.9s}
	\fig{lcs/J20h28m40.7s-30d56m10.4s_lc_fit_full.pdf}{0.24\linewidth}{J20h28m40.7s$-$30d56m10.4s}
	\fig{lcs/J21h17m25.0s-00d34m52.9s_lc_fit_full.pdf}{0.24\linewidth}{J21h17m25.0s$-$00d34m52.9s}}
\gridline{\fig{lcs/J21h17m51.1s-09d19m08.8s_lc_fit_full.pdf}{0.24\linewidth}{J21h17m51.1s$-$09d19m08.8s}
	\fig{lcs/J21h41m48.2s+04d38m19.7s_lc_fit_full.pdf}{0.24\linewidth}{J21h41m48.2s+04d38m19.7s}
	\fig{lcs/J23h19m19.0s-44d59m03.0s_lc_fit_full.pdf}{0.24\linewidth}{J23h19m19.0s$-$44d59m03.0s}}
\caption{Light curves of the ESE candidates in the VAST silver sample. \label{fig:ese_ext_lcs_5}}
\end{figure*}


==> ese_prop_qual_lcs.tex <==

\begin{figure*}
\centering
\gridline{\fig{lcs/J00h23m42.9s-59d30m32.0s_lc_fit_full.pdf}{0.24\linewidth}{J00h23m42.9s$-$59d30m32.0s}
	\fig{lcs/J04h02m42.0s+08d25m24.1s_lc_fit_full.pdf}{0.24\linewidth}{J04h02m42.0s+08d25m24.1s}
	\fig{lcs/J04h49m37.4s+08d11m33.9s_lc_fit_full.pdf}{0.24\linewidth}{J04h49m37.4s+08d11m33.9s}
	\fig{lcs/J05h08m48.5s-45d09m20.6s_lc_fit_full.pdf}{0.24\linewidth}{J05h08m48.5s$-$45d09m20.6s}}
\gridline{\fig{lcs/J05h28m03.1s-33d03m48.2s_lc_fit_full.pdf}{0.24\linewidth}{J05h28m03.1s$-$33d03m48.2s}
	\fig{lcs/J07h58m28.0s+08d27m08.3s_lc_fit_full.pdf}{0.24\linewidth}{J07h58m28.0s+08d27m08.3s}
	\fig{lcs/J09h09m43.2s+03d09m22.3s_lc_fit_full.pdf}{0.24\linewidth}{J09h09m43.2s+03d09m22.3s}
	\fig{lcs/J09h17m08.1s-03d06m18.0s_lc_fit_full.pdf}{0.24\linewidth}{J09h17m08.1s$-$03d06m18.0s}}
\gridline{\fig{lcs/J10h26m45.9s-28d56m41.1s_lc_fit_full.pdf}{0.24\linewidth}{J10h26m45.9s$-$28d56m41.1s}
	\fig{lcs/J11h37m00.5s-45d05m12.6s_lc_fit_full.pdf}{0.24\linewidth}{J11h37m00.5s$-$45d05m12.6s}
	\fig{lcs/J11h50m29.4s-33d57m16.2s_lc_fit_full.pdf}{0.24\linewidth}{J11h50m29.4s$-$33d57m16.2s}
	\fig{lcs/J12h17m01.5s-51d01m01.6s_lc_fit_full.pdf}{0.24\linewidth}{J12h17m01.5s$-$51d01m01.6s}}
\gridline{\fig{lcs/J12h17m58.4s-36d34m17.6s_lc_fit_full.pdf}{0.24\linewidth}{J12h17m58.4s$-$36d34m17.6s}
	\fig{lcs/J13h23m43.8s-51d42m22.7s_lc_fit_full.pdf}{0.24\linewidth}{J13h23m43.8s$-$51d42m22.7s}
	\fig{lcs/J13h24m50.9s-06d39m40.8s_lc_fit_full.pdf}{0.24\linewidth}{J13h24m50.9s$-$06d39m40.8s}
	\fig{lcs/J13h31m00.3s-38d09m28.0s_lc_fit_full.pdf}{0.24\linewidth}{J13h31m00.3s$-$38d09m28.0s}}
\gridline{\fig{lcs/J13h49m46.1s+09d08m16.3s_lc_fit_full.pdf}{0.24\linewidth}{J13h49m46.1s+09d08m16.3s}
	\fig{lcs/J14h34m52.7s-00d28m28.4s_lc_fit_full.pdf}{0.24\linewidth}{J14h34m52.7s$-$00d28m28.4s}
	\fig{lcs/J15h13m31.7s-09d19m19.6s_lc_fit_full.pdf}{0.24\linewidth}{J15h13m31.7s$-$09d19m19.6s}
	\fig{lcs/J16h06m06.9s+06d19m48.8s_lc_fit_full.pdf}{0.24\linewidth}{J16h06m06.9s+06d19m48.8s}}
\caption{Light curves of the ESE candidates in the VAST qualitative sample. \label{fig:ese_qual_lcs_1}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J16h08m56.1s+09d10m38.5s_lc_fit_full.pdf}{0.24\linewidth}{J16h08m56.1s+09d10m38.5s}
	\fig{lcs/J16h10m11.9s-03d49m17.1s_lc_fit_full.pdf}{0.24\linewidth}{J16h10m11.9s$-$03d49m17.1s}
	\fig{lcs/J16h11m31.8s-03d40m58.3s_lc_fit_full.pdf}{0.24\linewidth}{J16h11m31.8s$-$03d40m58.3s}
	\fig{lcs/J16h22m23.7s+00d13m28.7s_lc_fit_full.pdf}{0.24\linewidth}{J16h22m23.7s+00d13m28.7s}}
\gridline{\fig{lcs/J16h23m46.0s-08d35m38.4s_lc_fit_full.pdf}{0.24\linewidth}{J16h23m46.0s$-$08d35m38.4s}
	\fig{lcs/J16h30m51.5s-08d10m09.0s_lc_fit_full.pdf}{0.24\linewidth}{J16h30m51.5s$-$08d10m09.0s}
	\fig{lcs/J16h43m51.8s+08d55m05.9s_lc_fit_full.pdf}{0.24\linewidth}{J16h43m51.8s+08d55m05.9s}
	\fig{lcs/J16h57m14.4s+02d30m55.7s_lc_fit_full.pdf}{0.24\linewidth}{J16h57m14.4s+02d30m55.7s}}
\gridline{\fig{lcs/J17h00m23.9s+05d22m43.9s_lc_fit_full.pdf}{0.24\linewidth}{J17h00m23.9s+05d22m43.9s}
	\fig{lcs/J17h07m24.3s-02d17m51.5s_lc_fit_full.pdf}{0.24\linewidth}{J17h07m24.3s$-$02d17m51.5s}
	\fig{lcs/J17h07m51.3s-05d12m37.9s_lc_fit_full.pdf}{0.24\linewidth}{J17h07m51.3s$-$05d12m37.9s}
	\fig{lcs/J17h14m40.6s+05d12m38.1s_lc_fit_full.pdf}{0.24\linewidth}{J17h14m40.6s+05d12m38.1s}}
\gridline{\fig{lcs/J17h16m06.7s+07d08m47.2s_lc_fit_full.pdf}{0.24\linewidth}{J17h16m06.7s+07d08m47.2s}
	\fig{lcs/J17h37m09.8s+09d28m03.9s_lc_fit_full.pdf}{0.24\linewidth}{J17h37m09.8s+09d28m03.9s}
	\fig{lcs/J17h39m33.1s-03d47m55.5s_lc_fit_full.pdf}{0.24\linewidth}{J17h39m33.1s$-$03d47m55.5s}
	\fig{lcs/J17h39m42.2s+00d10m18.2s_lc_fit_full.pdf}{0.24\linewidth}{J17h39m42.2s+00d10m18.2s}}
\gridline{\fig{lcs/J18h00m06.4s+01d49m41.2s_lc_fit_full.pdf}{0.24\linewidth}{J18h00m06.4s+01d49m41.2s}
	\fig{lcs/J18h04m02.3s-00d35m51.0s_lc_fit_full.pdf}{0.24\linewidth}{J18h04m02.3s$-$00d35m51.0s}
	\fig{lcs/J18h09m28.5s+01d14m04.5s_lc_fit_full.pdf}{0.24\linewidth}{J18h09m28.5s+01d14m04.5s}
	\fig{lcs/J18h15m23.7s+04d49m21.1s_lc_fit_full.pdf}{0.24\linewidth}{J18h15m23.7s+04d49m21.1s}}
\caption{Light curves of the ESE candidates in the VAST qualitative sample. \label{fig:ese_qual_lcs_2}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J19h35m45.2s+04d14m19.8s_lc_fit_full.pdf}{0.24\linewidth}{J19h35m45.2s+04d14m19.8s}
	\fig{lcs/J19h44m44.6s+07d43m02.5s_lc_fit_full.pdf}{0.24\linewidth}{J19h44m44.6s+07d43m02.5s}
	\fig{lcs/J19h50m55.8s+02d00m43.2s_lc_fit_full.pdf}{0.24\linewidth}{J19h50m55.8s+02d00m43.2s}
	\fig{lcs/J19h56m06.7s+07d36m33.3s_lc_fit_full.pdf}{0.24\linewidth}{J19h56m06.7s+07d36m33.3s}}
\gridline{\fig{lcs/J19h59m09.1s-08d16m23.2s_lc_fit_full.pdf}{0.24\linewidth}{J19h59m09.1s$-$08d16m23.2s}
	\fig{lcs/J20h01m50.2s-06d19m43.4s_lc_fit_full.pdf}{0.24\linewidth}{J20h01m50.2s$-$06d19m43.4s}
	\fig{lcs/J20h03m41.5s-31d29m52.2s_lc_fit_full.pdf}{0.24\linewidth}{J20h03m41.5s$-$31d29m52.2s}
	\fig{lcs/J20h10m56.9s-00d34m26.6s_lc_fit_full.pdf}{0.24\linewidth}{J20h10m56.9s$-$00d34m26.6s}}
\gridline{\fig{lcs/J20h21m08.8s-35d55m27.3s_lc_fit_full.pdf}{0.24\linewidth}{J20h21m08.8s$-$35d55m27.3s}
	\fig{lcs/J20h26m49.5s+04d59m56.8s_lc_fit_full.pdf}{0.24\linewidth}{J20h26m49.5s+04d59m56.8s}
	\fig{lcs/J20h33m13.7s-44d23m23.8s_lc_fit_full.pdf}{0.24\linewidth}{J20h33m13.7s$-$44d23m23.8s}
	\fig{lcs/J20h35m05.4s-07d11m30.8s_lc_fit_full.pdf}{0.24\linewidth}{J20h35m05.4s$-$07d11m30.8s}}
\gridline{\fig{lcs/J20h36m29.2s-05d13m03.6s_lc_fit_full.pdf}{0.24\linewidth}{J20h36m29.2s$-$05d13m03.6s}
	\fig{lcs/J20h51m55.8s-36d55m22.5s_lc_fit_full.pdf}{0.24\linewidth}{J20h51m55.8s$-$36d55m22.5s}
	\fig{lcs/J21h16m03.2s-07d53m23.0s_lc_fit_full.pdf}{0.24\linewidth}{J21h16m03.2s$-$07d53m23.0s}
	\fig{lcs/J21h25m06.8s-05d36m39.2s_lc_fit_full.pdf}{0.24\linewidth}{J21h25m06.8s$-$05d36m39.2s}}
\gridline{\fig{lcs/J22h07m17.4s-08d02m10.3s_lc_fit_full.pdf}{0.24\linewidth}{J22h07m17.4s$-$08d02m10.3s}
	\fig{lcs/J22h07m55.3s+09d33m05.0s_lc_fit_full.pdf}{0.24\linewidth}{J22h07m55.3s+09d33m05.0s}}
\caption{Light curves of the ESE candidates in the VAST qualitative sample. \label{fig:ese_qual_lcs_3}}
\end{figure*}


==> ese_prop_quant_lcs.tex <==

\begin{figure*}
\centering
\gridline{\fig{lcs/J02h11m49.1s+06d00m14.5s_lc_fit_full.pdf}{0.24\linewidth}{J02h11m49.1s+06d00m14.5s}
	\fig{lcs/J04h26m32.5s+02d22m59.1s_lc_fit_full.pdf}{0.24\linewidth}{J04h26m32.5s+02d22m59.1s}
	\fig{lcs/J04h31m24.7s+06d22m08.5s_lc_fit_full.pdf}{0.24\linewidth}{J04h31m24.7s+06d22m08.5s}
	\fig{lcs/J05h14m50.7s+02d48m29.1s_lc_fit_full.pdf}{0.24\linewidth}{J05h14m50.7s+02d48m29.1s}}
\gridline{\fig{lcs/J06h01m58.9s-05d27m50.8s_lc_fit_full.pdf}{0.24\linewidth}{J06h01m58.9s$-$05d27m50.8s}
	\fig{lcs/J07h13m28.3s+06d51m41.9s_lc_fit_full.pdf}{0.24\linewidth}{J07h13m28.3s+06d51m41.9s}
	\fig{lcs/J11h54m58.5s-51d44m03.6s_lc_fit_full.pdf}{0.24\linewidth}{J11h54m58.5s$-$51d44m03.6s}
	\fig{lcs/J12h08m37.3s-41d05m14.1s_lc_fit_full.pdf}{0.24\linewidth}{J12h08m37.3s$-$41d05m14.1s}}
\gridline{\fig{lcs/J13h00m13.3s-50d11m53.0s_lc_fit_full.pdf}{0.24\linewidth}{J13h00m13.3s$-$50d11m53.0s}
	\fig{lcs/J13h02m45.2s-43d08m55.9s_lc_fit_full.pdf}{0.24\linewidth}{J13h02m45.2s$-$43d08m55.9s}
	\fig{lcs/J13h11m26.9s-31d00m36.2s_lc_fit_full.pdf}{0.24\linewidth}{J13h11m26.9s$-$31d00m36.2s}
	\fig{lcs/J15h14m46.8s+01d51m27.8s_lc_fit_full.pdf}{0.24\linewidth}{J15h14m46.8s+01d51m27.8s}}
\gridline{\fig{lcs/J15h42m44.0s+01d14m57.6s_lc_fit_full.pdf}{0.24\linewidth}{J15h42m44.0s+01d14m57.6s}
	\fig{lcs/J15h49m08.8s-01d16m27.9s_lc_fit_full.pdf}{0.24\linewidth}{J15h49m08.8s$-$01d16m27.9s}
	\fig{lcs/J16h17m52.7s-06d05m11.5s_lc_fit_full.pdf}{0.24\linewidth}{J16h17m52.7s$-$06d05m11.5s}
	\fig{lcs/J16h44m05.3s+02d14m08.8s_lc_fit_full.pdf}{0.24\linewidth}{J16h44m05.3s+02d14m08.8s}}
\gridline{\fig{lcs/J16h49m58.4s-04d48m47.2s_lc_fit_full.pdf}{0.24\linewidth}{J16h49m58.4s$-$04d48m47.2s}
	\fig{lcs/J16h58m44.7s+08d19m05.6s_lc_fit_full.pdf}{0.24\linewidth}{J16h58m44.7s+08d19m05.6s}
	\fig{lcs/J17h04m33.6s-08d55m52.2s_lc_fit_full.pdf}{0.24\linewidth}{J17h04m33.6s$-$08d55m52.2s}
	\fig{lcs/J17h05m43.5s+08d27m27.5s_lc_fit_full.pdf}{0.24\linewidth}{J17h05m43.5s+08d27m27.5s}}
\caption{Light curves of the ESE candidates in the VAST quantitative sample. \label{fig:ese_quant_lcs_1}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J17h07m15.7s-01d35m02.6s_lc_fit_full.pdf}{0.24\linewidth}{J17h07m15.7s$-$01d35m02.6s}
	\fig{lcs/J17h35m00.8s-07d33m20.7s_lc_fit_full.pdf}{0.24\linewidth}{J17h35m00.8s$-$07d33m20.7s}
	\fig{lcs/J17h43m49.3s+06d10m31.1s_lc_fit_full.pdf}{0.24\linewidth}{J17h43m49.3s+06d10m31.1s}
	\fig{lcs/J18h00m44.3s+04d31m59.0s_lc_fit_full.pdf}{0.24\linewidth}{J18h00m44.3s+04d31m59.0s}}
\gridline{\fig{lcs/J18h04m30.7s+08d58m57.3s_lc_fit_full.pdf}{0.24\linewidth}{J18h04m30.7s+08d58m57.3s}
	\fig{lcs/J19h31m55.5s-00d45m37.0s_lc_fit_full.pdf}{0.24\linewidth}{J19h31m55.5s$-$00d45m37.0s}
	\fig{lcs/J19h50m06.8s-07d16m42.7s_lc_fit_full.pdf}{0.24\linewidth}{J19h50m06.8s$-$07d16m42.7s}
	\fig{lcs/J20h11m33.7s-33d58m57.3s_lc_fit_full.pdf}{0.24\linewidth}{J20h11m33.7s$-$33d58m57.3s}}
\gridline{\fig{lcs/J20h35m15.8s-29d03m40.0s_lc_fit_full.pdf}{0.24\linewidth}{J20h35m15.8s$-$29d03m40.0s}}
\caption{Light curves of the ESE candidates in the VAST quantitative sample. \label{fig:ese_quant_lcs_2}}
\end{figure*}


==> eses_good_lcs.tex <==
\begin{figure*}
\centering
\gridline{\fig{lcs/J00h23m42.9s-59d30m32.0s_lc_fit.pdf}{0.24\linewidth}{J00h23m42.9s$-$59d30m32.0s}
	\fig{lcs/J01h50m09.8s-45d22m55.2s_lc_fit.pdf}{0.24\linewidth}{J01h50m09.8s$-$45d22m55.2s}
	\fig{lcs/J02h11m49.1s+06d00m14.5s_lc_fit.pdf}{0.24\linewidth}{J02h11m49.1s+06d00m14.5s}
	\fig{lcs/J03h58m55.3s+06d34m40.1s_lc_fit.pdf}{0.24\linewidth}{J03h58m55.3s+06d34m40.1s}}
\gridline{\fig{lcs/J04h02m42.0s+08d25m24.1s_lc_fit.pdf}{0.24\linewidth}{J04h02m42.0s+08d25m24.1s}
	\fig{lcs/J04h03m58.8s+06d45m38.9s_lc_fit.pdf}{0.24\linewidth}{J04h03m58.8s+06d45m38.9s}
	\fig{lcs/J04h08m00.2s-32d50m02.5s_lc_fit.pdf}{0.24\linewidth}{J04h08m00.2s$-$32d50m02.5s}
	\fig{lcs/J04h26m32.5s+02d22m59.1s_lc_fit.pdf}{0.24\linewidth}{J04h26m32.5s+02d22m59.1s}}
\gridline{\fig{lcs/J04h27m22.4s-49d07m41.9s_lc_fit.pdf}{0.24\linewidth}{J04h27m22.4s$-$49d07m41.9s}
	\fig{lcs/J04h31m24.7s+06d22m08.5s_lc_fit.pdf}{0.24\linewidth}{J04h31m24.7s+06d22m08.5s}
	\fig{lcs/J04h49m37.4s+08d11m33.9s_lc_fit.pdf}{0.24\linewidth}{J04h49m37.4s+08d11m33.9s}
	\fig{lcs/J04h51m27.2s+08d12m53.7s_lc_fit.pdf}{0.24\linewidth}{J04h51m27.2s+08d12m53.7s}}
\gridline{\fig{lcs/J05h00m04.8s+00d14m20.8s_lc_fit.pdf}{0.24\linewidth}{J05h00m04.8s+00d14m20.8s}
	\fig{lcs/J05h08m31.9s+06d00m11.9s_lc_fit.pdf}{0.24\linewidth}{J05h08m31.9s+06d00m11.9s}
	\fig{lcs/J05h08m48.5s-45d09m20.6s_lc_fit.pdf}{0.24\linewidth}{J05h08m48.5s$-$45d09m20.6s}
	\fig{lcs/J05h09m12.5s-45d22m19.2s_lc_fit.pdf}{0.24\linewidth}{J05h09m12.5s$-$45d22m19.2s}}
\gridline{\fig{lcs/J05h12m32.0s-02d58m29.1s_lc_fit.pdf}{0.24\linewidth}{J05h12m32.0s$-$02d58m29.1s}
	\fig{lcs/J05h13m41.0s-09d22m14.6s_lc_fit.pdf}{0.24\linewidth}{J05h13m41.0s$-$09d22m14.6s}
	\fig{lcs/J05h14m50.7s+02d48m29.1s_lc_fit.pdf}{0.24\linewidth}{J05h14m50.7s+02d48m29.1s}
	\fig{lcs/J05h23m25.7s+01d58m37.2s_lc_fit.pdf}{0.24\linewidth}{J05h23m25.7s+01d58m37.2s}}
\caption{Light curves of the ESE candidates in the VAST sample. \label{fig:ese_good_lcs_1}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J05h28m03.1s-33d03m48.2s_lc_fit.pdf}{0.24\linewidth}{J05h28m03.1s$-$33d03m48.2s}
	\fig{lcs/J05h52m02.1s-30d09m36.1s_lc_fit.pdf}{0.24\linewidth}{J05h52m02.1s$-$30d09m36.1s}
	\fig{lcs/J06h01m58.9s-05d27m50.8s_lc_fit.pdf}{0.24\linewidth}{J06h01m58.9s$-$05d27m50.8s}
	\fig{lcs/J07h13m28.3s+06d51m41.9s_lc_fit.pdf}{0.24\linewidth}{J07h13m28.3s+06d51m41.9s}}
\gridline{\fig{lcs/J07h28m56.5s-06d11m40.1s_lc_fit.pdf}{0.24\linewidth}{J07h28m56.5s$-$06d11m40.1s}
	\fig{lcs/J07h40m04.9s+04d15m28.6s_lc_fit.pdf}{0.24\linewidth}{J07h40m04.9s+04d15m28.6s}
	\fig{lcs/J07h58m28.0s+08d27m08.3s_lc_fit.pdf}{0.24\linewidth}{J07h58m28.0s+08d27m08.3s}
	\fig{lcs/J08h54m39.5s+08d43m25.7s_lc_fit.pdf}{0.24\linewidth}{J08h54m39.5s+08d43m25.7s}}
\gridline{\fig{lcs/J08h56m34.8s-06d54m09.4s_lc_fit.pdf}{0.24\linewidth}{J08h56m34.8s$-$06d54m09.4s}
	\fig{lcs/J09h09m43.2s+03d09m22.3s_lc_fit.pdf}{0.24\linewidth}{J09h09m43.2s+03d09m22.3s}
	\fig{lcs/J09h17m08.1s-03d06m18.0s_lc_fit.pdf}{0.24\linewidth}{J09h17m08.1s$-$03d06m18.0s}
	\fig{lcs/J09h42m15.5s+04d36m22.1s_lc_fit.pdf}{0.24\linewidth}{J09h42m15.5s+04d36m22.1s}}
\gridline{\fig{lcs/J10h24m43.5s-37d33m47.2s_lc_fit.pdf}{0.24\linewidth}{J10h24m43.5s$-$37d33m47.2s}
	\fig{lcs/J10h26m45.9s-28d56m41.1s_lc_fit.pdf}{0.24\linewidth}{J10h26m45.9s$-$28d56m41.1s}
	\fig{lcs/J10h44m24.0s-30d40m58.0s_lc_fit.pdf}{0.24\linewidth}{J10h44m24.0s$-$30d40m58.0s}
	\fig{lcs/J10h58m34.4s-42d15m13.3s_lc_fit.pdf}{0.24\linewidth}{J10h58m34.4s$-$42d15m13.3s}}
\gridline{\fig{lcs/J11h02m20.7s+01d42m05.5s_lc_fit.pdf}{0.24\linewidth}{J11h02m20.7s+01d42m05.5s}
	\fig{lcs/J11h32m59.3s-48d42m35.1s_lc_fit.pdf}{0.24\linewidth}{J11h32m59.3s$-$48d42m35.1s}
	\fig{lcs/J11h37m00.5s-45d05m12.6s_lc_fit.pdf}{0.24\linewidth}{J11h37m00.5s$-$45d05m12.6s}
	\fig{lcs/J11h49m40.0s-37d54m34.2s_lc_fit.pdf}{0.24\linewidth}{J11h49m40.0s$-$37d54m34.2s}}
\caption{Light curves of the ESE candidates in the VAST sample. \label{fig:ese_good_lcs_2}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J11h50m29.4s-33d57m16.2s_lc_fit.pdf}{0.24\linewidth}{J11h50m29.4s$-$33d57m16.2s}
	\fig{lcs/J11h54m58.5s-51d44m03.6s_lc_fit.pdf}{0.24\linewidth}{J11h54m58.5s$-$51d44m03.6s}
	\fig{lcs/J12h08m37.3s-41d05m14.1s_lc_fit.pdf}{0.24\linewidth}{J12h08m37.3s$-$41d05m14.1s}
	\fig{lcs/J12h17m01.5s-51d01m01.6s_lc_fit.pdf}{0.24\linewidth}{J12h17m01.5s$-$51d01m01.6s}}
\gridline{\fig{lcs/J12h17m58.4s-36d34m17.6s_lc_fit.pdf}{0.24\linewidth}{J12h17m58.4s$-$36d34m17.6s}
	\fig{lcs/J12h50m02.7s-50d41m48.7s_lc_fit.pdf}{0.24\linewidth}{J12h50m02.7s$-$50d41m48.7s}
	\fig{lcs/J12h50m51.8s-49d47m32.9s_lc_fit.pdf}{0.24\linewidth}{J12h50m51.8s$-$49d47m32.9s}
	\fig{lcs/J13h00m13.3s-50d11m53.0s_lc_fit.pdf}{0.24\linewidth}{J13h00m13.3s$-$50d11m53.0s}}
\gridline{\fig{lcs/J13h00m23.0s-42d08m39.3s_lc_fit.pdf}{0.24\linewidth}{J13h00m23.0s$-$42d08m39.3s}
	\fig{lcs/J13h02m45.2s-43d08m55.9s_lc_fit.pdf}{0.24\linewidth}{J13h02m45.2s$-$43d08m55.9s}
	\fig{lcs/J13h11m26.9s-31d00m36.2s_lc_fit.pdf}{0.24\linewidth}{J13h11m26.9s$-$31d00m36.2s}
	\fig{lcs/J13h15m37.8s-47d34m57.5s_lc_fit.pdf}{0.24\linewidth}{J13h15m37.8s$-$47d34m57.5s}}
\gridline{\fig{lcs/J13h23m43.8s-51d42m22.7s_lc_fit.pdf}{0.24\linewidth}{J13h23m43.8s$-$51d42m22.7s}
	\fig{lcs/J13h24m42.8s-50d20m37.8s_lc_fit.pdf}{0.24\linewidth}{J13h24m42.8s$-$50d20m37.8s}
	\fig{lcs/J13h24m50.9s-06d39m40.8s_lc_fit.pdf}{0.24\linewidth}{J13h24m50.9s$-$06d39m40.8s}
	\fig{lcs/J13h31m00.3s-38d09m28.0s_lc_fit.pdf}{0.24\linewidth}{J13h31m00.3s$-$38d09m28.0s}}
\gridline{\fig{lcs/J13h32m32.8s-47d28m30.0s_lc_fit.pdf}{0.24\linewidth}{J13h32m32.8s$-$47d28m30.0s}
	\fig{lcs/J13h36m03.2s-51d36m00.0s_lc_fit.pdf}{0.24\linewidth}{J13h36m03.2s$-$51d36m00.0s}
	\fig{lcs/J13h41m17.8s-49d03m36.8s_lc_fit.pdf}{0.24\linewidth}{J13h41m17.8s$-$49d03m36.8s}
	\fig{lcs/J13h48m31.0s-30d35m36.2s_lc_fit.pdf}{0.24\linewidth}{J13h48m31.0s$-$30d35m36.2s}}
\caption{Light curves of the ESE candidates in the VAST sample. \label{fig:ese_good_lcs_3}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J13h49m22.2s+07d12m17.6s_lc_fit.pdf}{0.24\linewidth}{J13h49m22.2s+07d12m17.6s}
	\fig{lcs/J13h49m46.1s+09d08m16.3s_lc_fit.pdf}{0.24\linewidth}{J13h49m46.1s+09d08m16.3s}
	\fig{lcs/J14h19m45.9s-08d27m06.4s_lc_fit.pdf}{0.24\linewidth}{J14h19m45.9s$-$08d27m06.4s}
	\fig{lcs/J14h34m52.7s-00d28m28.4s_lc_fit.pdf}{0.24\linewidth}{J14h34m52.7s$-$00d28m28.4s}}
\gridline{\fig{lcs/J15h06m37.4s+00d25m40.4s_lc_fit.pdf}{0.24\linewidth}{J15h06m37.4s+00d25m40.4s}
	\fig{lcs/J15h13m31.7s-09d19m19.6s_lc_fit.pdf}{0.24\linewidth}{J15h13m31.7s$-$09d19m19.6s}
	\fig{lcs/J15h14m46.8s+01d51m27.8s_lc_fit.pdf}{0.24\linewidth}{J15h14m46.8s+01d51m27.8s}
	\fig{lcs/J15h17m38.6s+03d45m28.3s_lc_fit.pdf}{0.24\linewidth}{J15h17m38.6s+03d45m28.3s}}
\gridline{\fig{lcs/J15h19m51.3s-09d18m48.8s_lc_fit.pdf}{0.24\linewidth}{J15h19m51.3s$-$09d18m48.8s}
	\fig{lcs/J15h24m45.4s-01d37m40.3s_lc_fit.pdf}{0.24\linewidth}{J15h24m45.4s$-$01d37m40.3s}
	\fig{lcs/J15h29m14.4s-04d14m07.6s_lc_fit.pdf}{0.24\linewidth}{J15h29m14.4s$-$04d14m07.6s}
	\fig{lcs/J15h42m36.1s-05d47m55.4s_lc_fit.pdf}{0.24\linewidth}{J15h42m36.1s$-$05d47m55.4s}}
\gridline{\fig{lcs/J15h42m44.0s+01d14m57.6s_lc_fit.pdf}{0.24\linewidth}{J15h42m44.0s+01d14m57.6s}
	\fig{lcs/J15h49m08.8s-01d16m27.9s_lc_fit.pdf}{0.24\linewidth}{J15h49m08.8s$-$01d16m27.9s}
	\fig{lcs/J15h49m40.2s+01d06m01.6s_lc_fit.pdf}{0.24\linewidth}{J15h49m40.2s+01d06m01.6s}
	\fig{lcs/J16h02m20.5s-04d25m36.5s_lc_fit.pdf}{0.24\linewidth}{J16h02m20.5s$-$04d25m36.5s}}
\gridline{\fig{lcs/J16h05m56.9s-01d09m49.3s_lc_fit.pdf}{0.24\linewidth}{J16h05m56.9s$-$01d09m49.3s}
	\fig{lcs/J16h06m06.9s+06d19m48.8s_lc_fit.pdf}{0.24\linewidth}{J16h06m06.9s+06d19m48.8s}
	\fig{lcs/J16h08m56.1s+09d10m38.5s_lc_fit.pdf}{0.24\linewidth}{J16h08m56.1s+09d10m38.5s}
	\fig{lcs/J16h10m11.9s-03d49m17.1s_lc_fit.pdf}{0.24\linewidth}{J16h10m11.9s$-$03d49m17.1s}}
\caption{Light curves of the ESE candidates in the VAST sample. \label{fig:ese_good_lcs_4}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J16h11m31.8s-03d40m58.3s_lc_fit.pdf}{0.24\linewidth}{J16h11m31.8s$-$03d40m58.3s}
	\fig{lcs/J16h17m52.7s-06d05m11.5s_lc_fit.pdf}{0.24\linewidth}{J16h17m52.7s$-$06d05m11.5s}
	\fig{lcs/J16h22m23.7s+00d13m28.7s_lc_fit.pdf}{0.24\linewidth}{J16h22m23.7s+00d13m28.7s}
	\fig{lcs/J16h23m46.0s-08d35m38.4s_lc_fit.pdf}{0.24\linewidth}{J16h23m46.0s$-$08d35m38.4s}}
\gridline{\fig{lcs/J16h27m12.9s+04d18m34.6s_lc_fit.pdf}{0.24\linewidth}{J16h27m12.9s+04d18m34.6s}
	\fig{lcs/J16h27m47.9s-09d01m06.4s_lc_fit.pdf}{0.24\linewidth}{J16h27m47.9s$-$09d01m06.4s}
	\fig{lcs/J16h30m07.9s-04d51m35.9s_lc_fit.pdf}{0.24\linewidth}{J16h30m07.9s$-$04d51m35.9s}
	\fig{lcs/J16h30m51.5s-08d10m09.0s_lc_fit.pdf}{0.24\linewidth}{J16h30m51.5s$-$08d10m09.0s}}
\gridline{\fig{lcs/J16h31m55.3s-08d30m08.2s_lc_fit.pdf}{0.24\linewidth}{J16h31m55.3s$-$08d30m08.2s}
	\fig{lcs/J16h39m39.0s+09d07m36.5s_lc_fit.pdf}{0.24\linewidth}{J16h39m39.0s+09d07m36.5s}
	\fig{lcs/J16h39m51.1s+01d16m50.4s_lc_fit.pdf}{0.24\linewidth}{J16h39m51.1s+01d16m50.4s}
	\fig{lcs/J16h40m43.3s-01d33m41.5s_lc_fit.pdf}{0.24\linewidth}{J16h40m43.3s$-$01d33m41.5s}}
\gridline{\fig{lcs/J16h41m00.2s+05d58m10.6s_lc_fit.pdf}{0.24\linewidth}{J16h41m00.2s+05d58m10.6s}
	\fig{lcs/J16h43m51.8s+08d55m05.9s_lc_fit.pdf}{0.24\linewidth}{J16h43m51.8s+08d55m05.9s}
	\fig{lcs/J16h44m05.3s+02d14m08.8s_lc_fit.pdf}{0.24\linewidth}{J16h44m05.3s+02d14m08.8s}
	\fig{lcs/J16h46m13.0s+05d17m50.1s_lc_fit.pdf}{0.24\linewidth}{J16h46m13.0s+05d17m50.1s}}
\gridline{\fig{lcs/J16h49m18.4s+09d21m43.7s_lc_fit.pdf}{0.24\linewidth}{J16h49m18.4s+09d21m43.7s}
	\fig{lcs/J16h49m58.4s-04d48m47.2s_lc_fit.pdf}{0.24\linewidth}{J16h49m58.4s$-$04d48m47.2s}
	\fig{lcs/J16h51m07.1s+01d24m06.2s_lc_fit.pdf}{0.24\linewidth}{J16h51m07.1s+01d24m06.2s}
	\fig{lcs/J16h52m06.0s+05d22m24.1s_lc_fit.pdf}{0.24\linewidth}{J16h52m06.0s+05d22m24.1s}}
\caption{Light curves of the ESE candidates in the VAST sample. \label{fig:ese_good_lcs_5}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J16h52m37.3s+01d00m16.3s_lc_fit.pdf}{0.24\linewidth}{J16h52m37.3s+01d00m16.3s}
	\fig{lcs/J16h57m14.4s+02d30m55.7s_lc_fit.pdf}{0.24\linewidth}{J16h57m14.4s+02d30m55.7s}
	\fig{lcs/J16h58m44.7s+08d19m05.6s_lc_fit.pdf}{0.24\linewidth}{J16h58m44.7s+08d19m05.6s}
	\fig{lcs/J16h59m22.1s-00d39m58.5s_lc_fit.pdf}{0.24\linewidth}{J16h59m22.1s$-$00d39m58.5s}}
\gridline{\fig{lcs/J17h00m23.9s+05d22m43.9s_lc_fit.pdf}{0.24\linewidth}{J17h00m23.9s+05d22m43.9s}
	\fig{lcs/J17h01m24.9s-06d31m33.5s_lc_fit.pdf}{0.24\linewidth}{J17h01m24.9s$-$06d31m33.5s}
	\fig{lcs/J17h02m07.7s-07d46m45.8s_lc_fit.pdf}{0.24\linewidth}{J17h02m07.7s$-$07d46m45.8s}
	\fig{lcs/J17h04m29.0s+04d20m34.7s_lc_fit.pdf}{0.24\linewidth}{J17h04m29.0s+04d20m34.7s}}
\gridline{\fig{lcs/J17h04m33.6s-08d55m52.2s_lc_fit.pdf}{0.24\linewidth}{J17h04m33.6s$-$08d55m52.2s}
	\fig{lcs/J17h05m43.5s+08d27m27.5s_lc_fit.pdf}{0.24\linewidth}{J17h05m43.5s+08d27m27.5s}
	\fig{lcs/J17h07m15.7s-01d35m02.6s_lc_fit.pdf}{0.24\linewidth}{J17h07m15.7s$-$01d35m02.6s}
	\fig{lcs/J17h07m24.3s-02d17m51.5s_lc_fit.pdf}{0.24\linewidth}{J17h07m24.3s$-$02d17m51.5s}}
\gridline{\fig{lcs/J17h07m51.3s-05d12m37.9s_lc_fit.pdf}{0.24\linewidth}{J17h07m51.3s$-$05d12m37.9s}
	\fig{lcs/J17h11m30.9s+09d21m27.7s_lc_fit.pdf}{0.24\linewidth}{J17h11m30.9s+09d21m27.7s}
	\fig{lcs/J17h12m08.0s+05d39m32.2s_lc_fit.pdf}{0.24\linewidth}{J17h12m08.0s+05d39m32.2s}
	\fig{lcs/J17h12m58.3s+01d01m59.8s_lc_fit.pdf}{0.24\linewidth}{J17h12m58.3s+01d01m59.8s}}
\gridline{\fig{lcs/J17h14m09.6s+03d33m20.7s_lc_fit.pdf}{0.24\linewidth}{J17h14m09.6s+03d33m20.7s}
	\fig{lcs/J17h14m40.6s+05d12m38.1s_lc_fit.pdf}{0.24\linewidth}{J17h14m40.6s+05d12m38.1s}
	\fig{lcs/J17h16m06.7s+07d08m47.2s_lc_fit.pdf}{0.24\linewidth}{J17h16m06.7s+07d08m47.2s}
	\fig{lcs/J17h16m40.5s-07d11m21.7s_lc_fit.pdf}{0.24\linewidth}{J17h16m40.5s$-$07d11m21.7s}}
\caption{Light curves of the ESE candidates in the VAST sample. \label{fig:ese_good_lcs_6}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J17h19m14.2s+02d15m56.3s_lc_fit.pdf}{0.24\linewidth}{J17h19m14.2s+02d15m56.3s}
	\fig{lcs/J17h21m35.0s+05d49m09.3s_lc_fit.pdf}{0.24\linewidth}{J17h21m35.0s+05d49m09.3s}
	\fig{lcs/J17h25m56.5s+00d30m47.0s_lc_fit.pdf}{0.24\linewidth}{J17h25m56.5s+00d30m47.0s}
	\fig{lcs/J17h31m49.6s+02d21m35.3s_lc_fit.pdf}{0.24\linewidth}{J17h31m49.6s+02d21m35.3s}}
\gridline{\fig{lcs/J17h34m45.7s+02d01m46.0s_lc_fit.pdf}{0.24\linewidth}{J17h34m45.7s+02d01m46.0s}
	\fig{lcs/J17h35m00.8s-07d33m20.7s_lc_fit.pdf}{0.24\linewidth}{J17h35m00.8s$-$07d33m20.7s}
	\fig{lcs/J17h37m09.8s+09d28m03.9s_lc_fit.pdf}{0.24\linewidth}{J17h37m09.8s+09d28m03.9s}
	\fig{lcs/J17h38m16.0s+01d25m39.1s_lc_fit.pdf}{0.24\linewidth}{J17h38m16.0s+01d25m39.1s}}
\gridline{\fig{lcs/J17h39m33.1s-03d47m55.5s_lc_fit.pdf}{0.24\linewidth}{J17h39m33.1s$-$03d47m55.5s}
	\fig{lcs/J17h39m42.2s+00d10m18.2s_lc_fit.pdf}{0.24\linewidth}{J17h39m42.2s+00d10m18.2s}
	\fig{lcs/J17h39m50.6s+03d18m09.8s_lc_fit.pdf}{0.24\linewidth}{J17h39m50.6s+03d18m09.8s}
	\fig{lcs/J17h40m54.7s+07d51m01.9s_lc_fit.pdf}{0.24\linewidth}{J17h40m54.7s+07d51m01.9s}}
\gridline{\fig{lcs/J17h41m47.8s+01d33m00.1s_lc_fit_full.pdf}{0.24\linewidth}{J17h41m47.8s+01d33m00.1s}
	\fig{lcs/J17h43m49.3s+06d10m31.1s_lc_fit.pdf}{0.24\linewidth}{J17h43m49.3s+06d10m31.1s}
	\fig{lcs/J17h44m30.9s+01d43m21.0s_lc_fit.pdf}{0.24\linewidth}{J17h44m30.9s+01d43m21.0s}
	\fig{lcs/J17h51m48.9s+08d05m25.3s_lc_fit.pdf}{0.24\linewidth}{J17h51m48.9s+08d05m25.3s}}
\gridline{\fig{lcs/J17h55m56.8s+00d34m41.1s_lc_fit.pdf}{0.24\linewidth}{J17h55m56.8s+00d34m41.1s}
	\fig{lcs/J17h57m13.1s+01d02m42.2s_lc_fit.pdf}{0.24\linewidth}{J17h57m13.1s+01d02m42.2s}
	\fig{lcs/J17h57m36.1s+03d19m38.8s_lc_fit.pdf}{0.24\linewidth}{J17h57m36.1s+03d19m38.8s}
	\fig{lcs/J17h57m42.7s-01d35m51.9s_lc_fit.pdf}{0.24\linewidth}{J17h57m42.7s$-$01d35m51.9s}}
\caption{Light curves of the ESE candidates in the VAST sample. \label{fig:ese_good_lcs_7}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J18h00m06.4s+01d49m41.2s_lc_fit.pdf}{0.24\linewidth}{J18h00m06.4s+01d49m41.2s}
	\fig{lcs/J18h00m44.3s+04d31m59.0s_lc_fit.pdf}{0.24\linewidth}{J18h00m44.3s+04d31m59.0s}
	\fig{lcs/J18h03m47.2s-01d16m26.4s_lc_fit.pdf}{0.24\linewidth}{J18h03m47.2s$-$01d16m26.4s}
	\fig{lcs/J18h04m02.3s-00d35m51.0s_lc_fit.pdf}{0.24\linewidth}{J18h04m02.3s$-$00d35m51.0s}}
\gridline{\fig{lcs/J18h04m30.7s+08d58m57.3s_lc_fit.pdf}{0.24\linewidth}{J18h04m30.7s+08d58m57.3s}
	\fig{lcs/J18h09m28.5s+01d14m04.5s_lc_fit.pdf}{0.24\linewidth}{J18h09m28.5s+01d14m04.5s}
	\fig{lcs/J18h15m23.7s+04d49m21.1s_lc_fit.pdf}{0.24\linewidth}{J18h15m23.7s+04d49m21.1s}
	\fig{lcs/J18h26m44.5s+09d04m06.0s_lc_fit.pdf}{0.24\linewidth}{J18h26m44.5s+09d04m06.0s}}
\gridline{\fig{lcs/J18h29m41.0s+03d55m32.7s_lc_fit.pdf}{0.24\linewidth}{J18h29m41.0s+03d55m32.7s}
	\fig{lcs/J19h07m10.6s-03d46m43.0s_lc_fit.pdf}{0.24\linewidth}{J19h07m10.6s$-$03d46m43.0s}
	\fig{lcs/J19h08m55.9s-05d05m27.6s_lc_fit.pdf}{0.24\linewidth}{J19h08m55.9s$-$05d05m27.6s}
	\fig{lcs/J19h15m33.4s-05d11m09.1s_lc_fit.pdf}{0.24\linewidth}{J19h15m33.4s$-$05d11m09.1s}}
\gridline{\fig{lcs/J19h19m34.4s-07d40m43.2s_lc_fit.pdf}{0.24\linewidth}{J19h19m34.4s$-$07d40m43.2s}
	\fig{lcs/J19h19m59.0s-07d57m25.7s_lc_fit.pdf}{0.24\linewidth}{J19h19m59.0s$-$07d57m25.7s}
	\fig{lcs/J19h20m25.0s-05d19m43.2s_lc_fit.pdf}{0.24\linewidth}{J19h20m25.0s$-$05d19m43.2s}
	\fig{lcs/J19h27m55.8s+06d42m49.0s_lc_fit.pdf}{0.24\linewidth}{J19h27m55.8s+06d42m49.0s}}
\gridline{\fig{lcs/J19h28m34.3s+06d49m06.8s_lc_fit.pdf}{0.24\linewidth}{J19h28m34.3s+06d49m06.8s}
	\fig{lcs/J19h31m55.5s-00d45m37.0s_lc_fit.pdf}{0.24\linewidth}{J19h31m55.5s$-$00d45m37.0s}
	\fig{lcs/J19h33m16.7s-08d22m39.7s_lc_fit.pdf}{0.24\linewidth}{J19h33m16.7s$-$08d22m39.7s}
	\fig{lcs/J19h34m46.2s-05d29m02.8s_lc_fit.pdf}{0.24\linewidth}{J19h34m46.2s$-$05d29m02.8s}}
\caption{Light curves of the ESE candidates in the VAST sample. \label{fig:ese_good_lcs_8}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J19h35m45.2s+04d14m19.8s_lc_fit.pdf}{0.24\linewidth}{J19h35m45.2s+04d14m19.8s}
	\fig{lcs/J19h39m07.0s-04d11m46.1s_lc_fit.pdf}{0.24\linewidth}{J19h39m07.0s$-$04d11m46.1s}
	\fig{lcs/J19h41m32.9s-08d16m54.5s_lc_fit.pdf}{0.24\linewidth}{J19h41m32.9s$-$08d16m54.5s}
	\fig{lcs/J19h44m44.6s+07d43m02.5s_lc_fit.pdf}{0.24\linewidth}{J19h44m44.6s+07d43m02.5s}}
\gridline{\fig{lcs/J19h46m52.3s-05d09m41.2s_lc_fit.pdf}{0.24\linewidth}{J19h46m52.3s$-$05d09m41.2s}
	\fig{lcs/J19h50m06.8s-07d16m42.7s_lc_fit.pdf}{0.24\linewidth}{J19h50m06.8s$-$07d16m42.7s}
	\fig{lcs/J19h50m55.8s+02d00m43.2s_lc_fit.pdf}{0.24\linewidth}{J19h50m55.8s+02d00m43.2s}
	\fig{lcs/J19h51m11.1s+06d03m18.5s_lc_fit.pdf}{0.24\linewidth}{J19h51m11.1s+06d03m18.5s}}
\gridline{\fig{lcs/J19h52m17.6s-45d28m19.3s_lc_fit.pdf}{0.24\linewidth}{J19h52m17.6s$-$45d28m19.3s}
	\fig{lcs/J19h53m44.9s-55d56m10.7s_lc_fit.pdf}{0.24\linewidth}{J19h53m44.9s$-$55d56m10.7s}
	\fig{lcs/J19h54m57.9s-08d40m28.6s_lc_fit.pdf}{0.24\linewidth}{J19h54m57.9s$-$08d40m28.6s}
	\fig{lcs/J19h56m06.7s+07d36m33.3s_lc_fit.pdf}{0.24\linewidth}{J19h56m06.7s+07d36m33.3s}}
\gridline{\fig{lcs/J19h59m09.1s-08d16m23.2s_lc_fit.pdf}{0.24\linewidth}{J19h59m09.1s$-$08d16m23.2s}
	\fig{lcs/J20h01m50.2s-06d19m43.4s_lc_fit.pdf}{0.24\linewidth}{J20h01m50.2s$-$06d19m43.4s}
	\fig{lcs/J20h03m41.5s-31d29m52.2s_lc_fit.pdf}{0.24\linewidth}{J20h03m41.5s$-$31d29m52.2s}
	\fig{lcs/J20h10m56.9s-00d34m26.6s_lc_fit.pdf}{0.24\linewidth}{J20h10m56.9s$-$00d34m26.6s}}
\gridline{\fig{lcs/J20h11m33.7s-33d58m57.3s_lc_fit.pdf}{0.24\linewidth}{J20h11m33.7s$-$33d58m57.3s}
	\fig{lcs/J20h13m26.5s-04d50m58.4s_lc_fit.pdf}{0.24\linewidth}{J20h13m26.5s$-$04d50m58.4s}
	\fig{lcs/J20h19m31.1s+05d41m40.9s_lc_fit.pdf}{0.24\linewidth}{J20h19m31.1s+05d41m40.9s}
	\fig{lcs/J20h21m08.8s-35d55m27.3s_lc_fit.pdf}{0.24\linewidth}{J20h21m08.8s$-$35d55m27.3s}}
\caption{Light curves of the ESE candidates in the VAST sample. \label{fig:ese_good_lcs_9}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{lcs/J20h26m49.5s+04d59m56.8s_lc_fit.pdf}{0.24\linewidth}{J20h26m49.5s+04d59m56.8s}
	\fig{lcs/J20h28m40.7s-30d56m10.4s_lc_fit.pdf}{0.24\linewidth}{J20h28m40.7s$-$30d56m10.4s}
	\fig{lcs/J20h33m13.7s-44d23m23.8s_lc_fit.pdf}{0.24\linewidth}{J20h33m13.7s$-$44d23m23.8s}
	\fig{lcs/J20h35m05.4s-07d11m30.8s_lc_fit.pdf}{0.24\linewidth}{J20h35m05.4s$-$07d11m30.8s}}
\gridline{\fig{lcs/J20h35m15.8s-29d03m40.0s_lc_fit.pdf}{0.24\linewidth}{J20h35m15.8s$-$29d03m40.0s}
	\fig{lcs/J20h36m29.2s-05d13m03.6s_lc_fit.pdf}{0.24\linewidth}{J20h36m29.2s$-$05d13m03.6s}
	\fig{lcs/J20h51m55.8s-36d55m22.5s_lc_fit.pdf}{0.24\linewidth}{J20h51m55.8s$-$36d55m22.5s}
	\fig{lcs/J21h16m03.2s-07d53m23.0s_lc_fit.pdf}{0.24\linewidth}{J21h16m03.2s$-$07d53m23.0s}}
\gridline{\fig{lcs/J21h17m25.0s-00d34m52.9s_lc_fit.pdf}{0.24\linewidth}{J21h17m25.0s$-$00d34m52.9s}
	\fig{lcs/J21h17m51.1s-09d19m08.8s_lc_fit.pdf}{0.24\linewidth}{J21h17m51.1s$-$09d19m08.8s}
	\fig{lcs/J21h25m06.8s-05d36m39.2s_lc_fit.pdf}{0.24\linewidth}{J21h25m06.8s$-$05d36m39.2s}
	\fig{lcs/J21h41m47.3s+06d11m16.0s_lc_fit.pdf}{0.24\linewidth}{J21h41m47.3s+06d11m16.0s}}
\gridline{\fig{lcs/J21h41m48.2s+04d38m19.7s_lc_fit.pdf}{0.24\linewidth}{J21h41m48.2s+04d38m19.7s}
	\fig{lcs/J22h06m51.7s+06d49m51.0s_lc_fit.pdf}{0.24\linewidth}{J22h06m51.7s+06d49m51.0s}
	\fig{lcs/J22h07m17.4s-08d02m10.3s_lc_fit.pdf}{0.24\linewidth}{J22h07m17.4s$-$08d02m10.3s}
	\fig{lcs/J22h07m55.3s+09d33m05.0s_lc_fit.pdf}{0.24\linewidth}{J22h07m55.3s+09d33m05.0s}}
\gridline{\fig{lcs/J23h19m19.0s-44d59m03.0s_lc_fit.pdf}{0.24\linewidth}{J23h19m19.0s$-$44d59m03.0s}}
\caption{Light curves of the ESE candidates in the VAST sample. \label{fig:ese_good_lcs_10}}
\end{figure*}

==> eses_maybe_lcs.tex <==
\begin{figure*}
\centering
\gridline{\fig{old_lcs/J01h15m12.5s-29d41m45.3s_lc_fit.pdf}{0.24\linewidth}{J01h15m12.5s$-$29d41m45.3s}
	\fig{old_lcs/J03h04m38.5s+00d12m41.7s_lc_fit.pdf}{0.24\linewidth}{J03h04m38.5s+00d12m41.7s}
	\fig{old_lcs/J03h11m05.9s-08d12m31.3s_lc_fit.pdf}{0.24\linewidth}{J03h11m05.9s$-$08d12m31.3s}
	\fig{old_lcs/J03h15m56.2s-06d25m01.6s_lc_fit.pdf}{0.24\linewidth}{J03h15m56.2s$-$06d25m01.6s}}
\gridline{\fig{old_lcs/J04h30m06.7s-39d06m22.2s_lc_fit.pdf}{0.24\linewidth}{J04h30m06.7s$-$39d06m22.2s}
	\fig{old_lcs/J04h31m36.0s-08d04m34.7s_lc_fit.pdf}{0.24\linewidth}{J04h31m36.0s$-$08d04m34.7s}
	\fig{old_lcs/J04h45m04.7s-39d37m12.7s_lc_fit.pdf}{0.24\linewidth}{J04h45m04.7s$-$39d37m12.7s}
	\fig{old_lcs/J05h07m03.7s-08d40m08.8s_lc_fit.pdf}{0.24\linewidth}{J05h07m03.7s$-$08d40m08.8s}}
\gridline{\fig{old_lcs/J05h09m17.4s-00d24m26.0s_lc_fit.pdf}{0.24\linewidth}{J05h09m17.4s$-$00d24m26.0s}
	\fig{old_lcs/J05h14m52.0s-00d54m15.6s_lc_fit.pdf}{0.24\linewidth}{J05h14m52.0s$-$00d54m15.6s}
	\fig{old_lcs/J05h16m45.1s+07d41m23.3s_lc_fit.pdf}{0.24\linewidth}{J05h16m45.1s+07d41m23.3s}
	\fig{old_lcs/J05h19m41.1s+00d34m30.3s_lc_fit.pdf}{0.24\linewidth}{J05h19m41.1s+00d34m30.3s}}
\gridline{\fig{old_lcs/J05h51m09.4s-04d06m55.1s_lc_fit.pdf}{0.24\linewidth}{J05h51m09.4s$-$04d06m55.1s}
	\fig{old_lcs/J06h11m39.7s-01d18m01.9s_lc_fit.pdf}{0.24\linewidth}{J06h11m39.7s$-$01d18m01.9s}
	\fig{old_lcs/J06h36m44.1s-05d30m01.9s_lc_fit.pdf}{0.24\linewidth}{J06h36m44.1s$-$05d30m01.9s}
	\fig{old_lcs/J07h46m13.8s-07d28m22.5s_lc_fit.pdf}{0.24\linewidth}{J07h46m13.8s$-$07d28m22.5s}}
\gridline{\fig{old_lcs/J09h01m08.6s-00d33m34.0s_lc_fit.pdf}{0.24\linewidth}{J09h01m08.6s$-$00d33m34.0s}
	\fig{old_lcs/J10h12m19.1s-30d22m37.2s_lc_fit.pdf}{0.24\linewidth}{J10h12m19.1s$-$30d22m37.2s}
	\fig{old_lcs/J10h20m59.6s-36d14m26.7s_lc_fit.pdf}{0.24\linewidth}{J10h20m59.6s$-$36d14m26.7s}
	\fig{old_lcs/J10h33m06.1s-30d54m39.9s_lc_fit.pdf}{0.24\linewidth}{J10h33m06.1s$-$30d54m39.9s}}
\caption{Light curves of the ESE candidates in the VAST bronze sample. \label{fig:ese_maybe_lcs_1}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{old_lcs/J10h55m29.0s-30d11m03.2s_lc_fit.pdf}{0.24\linewidth}{J10h55m29.0s$-$30d11m03.2s}
	\fig{old_lcs/J10h56m13.1s-35d27m35.5s_lc_fit.pdf}{0.24\linewidth}{J10h56m13.1s$-$35d27m35.5s}
	\fig{old_lcs/J11h32m48.9s-50d48m58.8s_lc_fit.pdf}{0.24\linewidth}{J11h32m48.9s$-$50d48m58.8s}
	\fig{old_lcs/J11h43m39.8s+07d00m12.6s_lc_fit.pdf}{0.24\linewidth}{J11h43m39.8s+07d00m12.6s}}
\gridline{\fig{old_lcs/J12h13m35.5s-50d31m42.7s_lc_fit.pdf}{0.24\linewidth}{J12h13m35.5s$-$50d31m42.7s}
	\fig{old_lcs/J12h50m22.8s-44d32m03.2s_lc_fit.pdf}{0.24\linewidth}{J12h50m22.8s$-$44d32m03.2s}
	\fig{old_lcs/J12h57m10.4s-46d37m40.8s_lc_fit.pdf}{0.24\linewidth}{J12h57m10.4s$-$46d37m40.8s}
	\fig{old_lcs/J13h08m26.8s-35d45m57.2s_lc_fit.pdf}{0.24\linewidth}{J13h08m26.8s$-$35d45m57.2s}}
\gridline{\fig{old_lcs/J13h31m07.7s-53d09m57.4s_lc_fit.pdf}{0.24\linewidth}{J13h31m07.7s$-$53d09m57.4s}
	\fig{old_lcs/J13h32m22.0s-52d16m39.0s_lc_fit.pdf}{0.24\linewidth}{J13h32m22.0s$-$52d16m39.0s}
	\fig{old_lcs/J13h37m56.4s-50d55m40.7s_lc_fit.pdf}{0.24\linewidth}{J13h37m56.4s$-$50d55m40.7s}
	\fig{old_lcs/J13h42m36.4s-50d39m12.9s_lc_fit.pdf}{0.24\linewidth}{J13h42m36.4s$-$50d39m12.9s}}
\gridline{\fig{old_lcs/J13h57m39.4s-45d20m29.1s_lc_fit.pdf}{0.24\linewidth}{J13h57m39.4s$-$45d20m29.1s}
	\fig{old_lcs/J14h06m02.1s-43d48m23.3s_lc_fit.pdf}{0.24\linewidth}{J14h06m02.1s$-$43d48m23.3s}
	\fig{old_lcs/J14h19m04.9s-09d00m45.5s_lc_fit.pdf}{0.24\linewidth}{J14h19m04.9s$-$09d00m45.5s}
	\fig{old_lcs/J14h22m25.1s+07d01m58.1s_lc_fit.pdf}{0.24\linewidth}{J14h22m25.1s+07d01m58.1s}}
\gridline{\fig{old_lcs/J15h43m39.8s+08d06m12.8s_lc_fit.pdf}{0.24\linewidth}{J15h43m39.8s+08d06m12.8s}
	\fig{old_lcs/J16h03m14.9s+08d10m20.3s_lc_fit.pdf}{0.24\linewidth}{J16h03m14.9s+08d10m20.3s}
	\fig{old_lcs/J16h10m12.4s-00d11m41.6s_lc_fit.pdf}{0.24\linewidth}{J16h10m12.4s$-$00d11m41.6s}
	\fig{old_lcs/J16h17m26.3s+06d32m32.5s_lc_fit.pdf}{0.24\linewidth}{J16h17m26.3s+06d32m32.5s}}
\caption{Light curves of the ESE candidates in the VAST bronze sample. \label{fig:ese_maybe_lcs_2}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{old_lcs/J16h18m46.7s+04d40m06.7s_lc_fit.pdf}{0.24\linewidth}{J16h18m46.7s+04d40m06.7s}
	\fig{old_lcs/J16h25m20.4s+05d56m40.9s_lc_fit.pdf}{0.24\linewidth}{J16h25m20.4s+05d56m40.9s}
	\fig{old_lcs/J16h36m41.6s+09d24m58.0s_lc_fit.pdf}{0.24\linewidth}{J16h36m41.6s+09d24m58.0s}
	\fig{old_lcs/J16h37m50.2s+02d11m44.0s_lc_fit.pdf}{0.24\linewidth}{J16h37m50.2s+02d11m44.0s}}
\gridline{\fig{old_lcs/J16h56m00.0s-00d30m29.2s_lc_fit.pdf}{0.24\linewidth}{J16h56m00.0s$-$00d30m29.2s}
	\fig{old_lcs/J16h59m10.9s-07d37m10.2s_lc_fit.pdf}{0.24\linewidth}{J16h59m10.9s$-$07d37m10.2s}
	\fig{old_lcs/J17h02m19.4s-03d38m58.1s_lc_fit.pdf}{0.24\linewidth}{J17h02m19.4s$-$03d38m58.1s}
	\fig{old_lcs/J17h06m45.8s+00d51m56.1s_lc_fit.pdf}{0.24\linewidth}{J17h06m45.8s+00d51m56.1s}}
\gridline{\fig{old_lcs/J17h09m31.9s-01d49m16.9s_lc_fit.pdf}{0.24\linewidth}{J17h09m31.9s$-$01d49m16.9s}
	\fig{old_lcs/J17h12m44.0s+05d23m59.7s_lc_fit.pdf}{0.24\linewidth}{J17h12m44.0s+05d23m59.7s}
	\fig{old_lcs/J17h24m17.6s+08d33m46.1s_lc_fit.pdf}{0.24\linewidth}{J17h24m17.6s+08d33m46.1s}
	\fig{old_lcs/J17h26m23.7s+04d23m57.5s_lc_fit.pdf}{0.24\linewidth}{J17h26m23.7s+04d23m57.5s}}
\gridline{\fig{old_lcs/J17h29m45.4s+04d16m12.5s_lc_fit.pdf}{0.24\linewidth}{J17h29m45.4s+04d16m12.5s}
	\fig{old_lcs/J17h32m53.0s+08d58m29.8s_lc_fit.pdf}{0.24\linewidth}{J17h32m53.0s+08d58m29.8s}
	\fig{old_lcs/J17h33m24.4s+09d21m41.7s_lc_fit.pdf}{0.24\linewidth}{J17h33m24.4s+09d21m41.7s}
	\fig{old_lcs/J17h36m54.7s-07d31m33.0s_lc_fit.pdf}{0.24\linewidth}{J17h36m54.7s$-$07d31m33.0s}}
\gridline{\fig{old_lcs/J17h54m43.5s+06d46m43.2s_lc_fit.pdf}{0.24\linewidth}{J17h54m43.5s+06d46m43.2s}
	\fig{old_lcs/J17h57m09.8s+08d56m28.5s_lc_fit.pdf}{0.24\linewidth}{J17h57m09.8s+08d56m28.5s}
	\fig{old_lcs/J18h00m51.8s+08d31m29.8s_lc_fit.pdf}{0.24\linewidth}{J18h00m51.8s+08d31m29.8s}
	\fig{old_lcs/J18h37m04.1s+09d09m24.1s_lc_fit.pdf}{0.24\linewidth}{J18h37m04.1s+09d09m24.1s}}
\caption{Light curves of the ESE candidates in the VAST bronze sample. \label{fig:ese_maybe_lcs_3}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{old_lcs/J19h17m57.7s-08d26m51.1s_lc_fit.pdf}{0.24\linewidth}{J19h17m57.7s$-$08d26m51.1s}
	\fig{old_lcs/J19h28m33.2s-01d10m46.7s_lc_fit.pdf}{0.24\linewidth}{J19h28m33.2s$-$01d10m46.7s}
	\fig{old_lcs/J19h35m03.6s-01d11m06.2s_lc_fit.pdf}{0.24\linewidth}{J19h35m03.6s$-$01d11m06.2s}
	\fig{old_lcs/J19h36m37.5s-06d17m34.0s_lc_fit.pdf}{0.24\linewidth}{J19h36m37.5s$-$06d17m34.0s}}
\gridline{\fig{old_lcs/J19h47m51.6s+04d22m15.8s_lc_fit.pdf}{0.24\linewidth}{J19h47m51.6s+04d22m15.8s}
	\fig{old_lcs/J19h49m34.5s+07d08m33.6s_lc_fit.pdf}{0.24\linewidth}{J19h49m34.5s+07d08m33.6s}
	\fig{old_lcs/J19h52m35.6s-06d57m06.7s_lc_fit.pdf}{0.24\linewidth}{J19h52m35.6s$-$06d57m06.7s}
	\fig{old_lcs/J19h53m41.4s+09d17m39.1s_lc_fit.pdf}{0.24\linewidth}{J19h53m41.4s+09d17m39.1s}}
\gridline{\fig{old_lcs/J19h58m18.1s+06d30m13.6s_lc_fit.pdf}{0.24\linewidth}{J19h58m18.1s+06d30m13.6s}
	\fig{old_lcs/J20h04m56.5s-31d09m50.8s_lc_fit.pdf}{0.24\linewidth}{J20h04m56.5s$-$31d09m50.8s}
	\fig{old_lcs/J20h05m44.9s-34d15m15.7s_lc_fit.pdf}{0.24\linewidth}{J20h05m44.9s$-$34d15m15.7s}
	\fig{old_lcs/J20h11m12.8s+07d13m32.4s_lc_fit.pdf}{0.24\linewidth}{J20h11m12.8s+07d13m32.4s}}
\gridline{\fig{old_lcs/J20h12m26.5s-30d39m46.4s_lc_fit.pdf}{0.24\linewidth}{J20h12m26.5s$-$30d39m46.4s}
	\fig{old_lcs/J20h20m49.5s-28d48m22.5s_lc_fit.pdf}{0.24\linewidth}{J20h20m49.5s$-$28d48m22.5s}
	\fig{old_lcs/J20h33m10.5s-44d44m52.8s_lc_fit.pdf}{0.24\linewidth}{J20h33m10.5s$-$44d44m52.8s}
	\fig{old_lcs/J20h39m09.1s-30d45m20.7s_lc_fit.pdf}{0.24\linewidth}{J20h39m09.1s$-$30d45m20.7s}}
\gridline{\fig{old_lcs/J20h48m47.1s-43d59m33.1s_lc_fit.pdf}{0.24\linewidth}{J20h48m47.1s$-$43d59m33.1s}
	\fig{old_lcs/J20h56m55.7s+00d20m31.9s_lc_fit.pdf}{0.24\linewidth}{J20h56m55.7s+00d20m31.9s}
	\fig{old_lcs/J21h02m49.3s-48d38m04.3s_lc_fit.pdf}{0.24\linewidth}{J21h02m49.3s$-$48d38m04.3s}
	\fig{old_lcs/J21h14m29.8s-00d52m17.6s_lc_fit.pdf}{0.24\linewidth}{J21h14m29.8s$-$00d52m17.6s}}
\caption{Light curves of the ESE candidates in the VAST bronze sample. \label{fig:ese_maybe_lcs_4}}
\end{figure*}
\begin{figure*}
\centering
\gridline{\fig{old_lcs/J21h19m14.3s-35d52m38.9s_lc_fit.pdf}{0.24\linewidth}{J21h19m14.3s$-$35d52m38.9s}
	\fig{old_lcs/J22h02m42.1s+04d36m37.8s_lc_fit.pdf}{0.24\linewidth}{J22h02m42.1s+04d36m37.8s}}
\caption{Light curves of the ESE candidates in the VAST bronze sample. \label{fig:ese_maybe_lcs_5}}
\end{figure*}

==> extended_sample_justification.tex <==
% \begin{deluxetable}{ll}
% \tablehead{\colhead{Source} & \colhead{Comment}}
% \startdata
% J01h15m12.5s$-$29d41m45.3s &  Second dip\\
% J03h04m38.5s+00d12m41.7s &  Asymmetric caustics\\
% J03h11m05.9s$-$08d12m31.3s & Single caustic spike \\
% J03h15m56.2s$-$06d25m01.6s &  Pre-variability\\
% J04h30m06.7s$-$39d06m22.2s &  Asymmetric dips\\
% J04h31m36.0s$-$08d04m34.7s &  Asymmetric caustics\\
% J04h45m04.7s$-$39d37m12.7s &  Asymmetric dips\\
% J05h07m03.7s$-$08d40m08.8s &  Asymmetric caustics\\
% J05h09m17.4s$-$00d24m26.0s &  Asymmetric caustics;\\
%  &  Additional variability\\
% J05h14m52.0s$-$00d54m15.6s &  Ongoing event (?);\\
%  &  Additional variability\\
% J05h16m45.1s+07d41m23.3s &  Additional variability\\
% J05h19m41.1s+00d34m30.3s &  Asymmetric caustics;\\
%  &  Additional variability\\
% J05h51m09.4s$-$04d06m55.1s &  Ongoing event (?);\\
% J06h11m39.7s$-$01d18m01.9s &  Ongoing event (?);\\
%  &  Additional variability\\
% J06h36m44.1s$-$05d30m01.9s &  Low SNR;\\
%  &  Additional variability\\
% J07h46m13.8s$-$07d28m22.5s &  Asymmetric dips;\\
%  &  Additional variability\\
% J09h01m08.6s$-$00d33m34.0s &  Pre-variability\\
% J10h12m19.1s$-$30d22m37.2s &  Additional variability\\
% J10h20m59.6s$-$36d14m26.7s &  Asymmetric caustics;\\
%  & Second dip \\
% J10h33m06.1s$-$30d54m39.9s &  Asymmetric dips;\\
%  & Ongoing event (?)\\
% J10h55m29.0s$-$30d11m03.2s &  Additional variability\\
% J10h56m13.1s$-$35d27m35.5s &  Second dip (?)\\
% J11h32m48.9s$-$50d48m58.8s &  Asymmetric caustics;\\
%  & Second dip (?) \\
% J11h43m39.8s+07d00m12.6s &  Asymmetric caustics;\\
%  &  Additional variability\\
% J12h13m35.5s$-$50d31m42.7s &  Asymmetric caustics;\\
% J12h50m22.8s$-$44d32m03.2s &  Additional variability\\
% J12h57m10.4s$-$46d37m40.8s &  Second dip (?)\\
%  &  Additional variability\\
% J13h08m26.8s$-$35d45m57.2s &  Additional variability\\
% J13h31m07.7s$-$53d09m57.4s &  Low SNR;\\
%  &  Additional variability\\
% J13h32m22.0s$-$52d16m39.0s &  Ongoing event (?)\\
% J13h37m56.4s$-$50d55m40.7s &  Ongoing event (?)\\
% J13h42m36.4s$-$50d39m12.9s &  Second dip (?)\\
% J13h57m39.4s$-$45d20m29.1s &  Ongoing event (?)\\
%  &  Additional variability\\
% J14h06m02.1s$-$43d48m23.3s &  Asymmetric dips;\\
%  &  Additional variability\\
% J14h19m04.9s$-$09d00m45.5s &  Additional variability\\
% J14h22m25.1s+07d01m58.1s &  Ongoing event (?)\\
%  &  Additional variability\\
% J15h43m39.8s+08d06m12.8s &  Additional variability\\
% J16h03m14.9s+08d10m20.3s &  Pre-variability\\
% J16h10m12.4s$-$00d11m41.6s &  Ongoing event (?)\\
% J16h17m26.3s+06d32m32.5s &  Low SNR\\
% J16h18m23.7s$-$06d03m26.3s &  Additional variability\\
% J16h18m46.7s+04d40m06.7s &  Additional variability;\\
% J16h25m20.4s+05d56m40.9s &  Additional variability\\
%  & Asymmetric dips \\
% J16h36m41.6s+09d24m58.0s &  Additional variability\\
% J16h37m50.2s+02d11m44.0s &  Additional variability\\
% J16h56m00.0s$-$00d30m29.2s &  Additional variability\\
% J16h59m10.9s$-$07d37m10.2s &  Additional variability\\
% J17h02m19.4s$-$03d38m58.1s &  Additional variability\\
% J17h06m45.8s+00d51m56.1s &  Additional variability\\
% J17h09m31.9s$-$01d49m16.9s &  Additional variability\\
% J17h12m44.0s+05d23m59.7s &  Additional variability\\
% J17h16m19.2s+01d33m06.6s &  Additional variability\\
% J17h24m17.6s+08d33m46.1s &  Additional variability\\
% J17h26m23.7s+04d23m57.5s &  Additional variability\\
% J17h29m45.4s+04d16m12.5s &  Second dip (?)\\
% J17h32m53.0s+08d58m29.8s &  Additional variability\\
% J17h33m24.4s+09d21m41.7s &  Asymmetric dips\\
%  & Additional variability \\
% J17h36m54.7s$-$07d31m33.0s &  Additional variability\\
% J17h54m43.5s+06d46m43.2s &  Second dip\\
% J17h57m09.8s+08d56m28.5s &  Additional variability\\
%  & Asymmetric caustics \\
% J18h00m51.8s+08d31m29.8s &  Additional variability\\
% J18h37m04.1s+09d09m24.1s &  Asymmetric caustics;\\
%  & Additional variability \\
% J19h17m57.7s$-$08d26m51.1s &  Additional variability\\
% J19h21m20.0s$-$05d34m32.1s &  Additional variability\\
% J19h28m33.2s$-$01d10m46.7s &  Additional variability \\
% J19h35m03.6s$-$01d11m06.2s &  Asymmetric caustics\\
%  & Additional variability \\
% J19h36m37.5s$-$06d17m34.0s &  Additional variability;\\
%  & Second dip (?) \\
% J19h47m51.6s+04d22m15.8s &  Asymmetric caustics\\
%  & Additional variability \\
% J19h49m34.5s+07d08m33.6s &  Additional variability\\
% J19h52m35.6s$-$06d57m06.7s &  Additional variability\\
% J19h53m41.4s+09d17m39.1s &  Additional variability\\
% J19h58m18.1s+06d30m13.6s &  Additional variability\\
%  & Pre-variability \\
% J20h04m56.5s$-$31d09m50.8s &  Additional variability\\
%  & Second dip (?) \\
% J20h05m44.9s$-$34d15m15.7s &  Additional variability\\
% J20h11m12.8s+07d13m32.4s &  Asymmetric caustics;\\
%  &  Additional variability\\
% J20h12m26.5s$-$30d39m46.4s &  Additional variability\\
% J20h20m49.5s$-$28d48m22.5s &  Additional variability;\\
%  & Pre-variability\\
% J20h33m10.5s$-$44d44m52.8s &  Additional variability\\
% J20h39m09.1s$-$30d45m20.7s &  Ongoing event (?)\\
%  & Additional variability \\
% J20h48m47.1s$-$43d59m33.1s &  Additional variability\\
% J20h56m55.7s+00d20m31.9s &  Additional variability\\
% J21h02m49.3s$-$48d38m04.3s &  Additional variability\\
% J21h14m29.8s$-$00d52m17.6s &  Additional variability \\
% J21h19m14.3s$-$35d52m38.9s &  Additional variability \\
% J22h02m42.1s+04d36m37.8s &  Additional variability\\
% \enddata
% \end{deluxetable}

\begin{table*}[t]
\centering
\caption{Details on the extended sample}
\label{tab:sources}
\begin{minipage}[t]{0.48\textwidth}
\begin{tabular}{ll}
\hline
\hline
Source & Comment \\
\hline
J01h15m12.5s$-$29d41m45.3s &  Second dip\\
J03h04m38.5s+00d12m41.7s &  Asymmetric caustics\\
J03h11m05.9s$-$08d12m31.3s & Single caustic spike \\
J03h15m56.2s$-$06d25m01.6s &  Pre-variability\\
J04h30m06.7s$-$39d06m22.2s &  Asymmetric dips\\
J04h31m36.0s$-$08d04m34.7s &  Asymmetric caustics\\
J04h45m04.7s$-$39d37m12.7s &  Asymmetric dips\\
J05h07m03.7s$-$08d40m08.8s &  Asymmetric caustics\\
J05h09m17.4s$-$00d24m26.0s &  Asymmetric caustics;\\
 &  Additional variability\\
J05h14m52.0s$-$00d54m15.6s &  Ongoing event (?);\\
 &  Additional variability\\
J05h16m45.1s+07d41m23.3s &  Additional variability\\
J05h19m41.1s+00d34m30.3s &  Asymmetric caustics;\\
 &  Additional variability\\
J05h51m09.4s$-$04d06m55.1s &  Ongoing event (?);\\
J06h11m39.7s$-$01d18m01.9s &  Ongoing event (?);\\
 &  Additional variability\\
J06h36m44.1s$-$05d30m01.9s &  Low SNR;\\
 &  Additional variability\\
J07h46m13.8s$-$07d28m22.5s &  Asymmetric dips;\\
 &  Additional variability\\
J09h01m08.6s$-$00d33m34.0s &  Pre-variability\\
J10h12m19.1s$-$30d22m37.2s &  Additional variability\\
J10h20m59.6s$-$36d14m26.7s &  Asymmetric caustics;\\
 & Second dip \\
J10h33m06.1s$-$30d54m39.9s &  Asymmetric dips;\\
 & Ongoing event (?)\\
J10h55m29.0s$-$30d11m03.2s &  Additional variability\\
J10h56m13.1s$-$35d27m35.5s &  Second dip (?)\\
J11h32m48.9s$-$50d48m58.8s &  Asymmetric caustics;\\
 & Second dip (?) \\
J11h43m39.8s+07d00m12.6s &  Asymmetric caustics;\\
 &  Additional variability\\
J12h13m35.5s$-$50d31m42.7s &  Asymmetric caustics;\\
J12h50m22.8s$-$44d32m03.2s &  Additional variability\\
J12h57m10.4s$-$46d37m40.8s &  Second dip (?)\\
 &  Additional variability\\
J13h08m26.8s$-$35d45m57.2s &  Additional variability\\
J13h31m07.7s$-$53d09m57.4s &  Low SNR;\\
 &  Additional variability\\
J13h32m22.0s$-$52d16m39.0s &  Ongoing event (?)\\
J13h37m56.4s$-$50d55m40.7s &  Ongoing event (?)\\
J13h42m36.4s$-$50d39m12.9s &  Second dip (?)\\
J13h57m39.4s$-$45d20m29.1s &  Ongoing event (?)\\
 &  Additional variability\\
J14h06m02.1s$-$43d48m23.3s &  Asymmetric dips;\\
 &  Additional variability\\
J14h19m04.9s$-$09d00m45.5s &  Additional variability\\
\hline
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\begin{tabular}{ll}
\hline
\hline
Source & Comment \\
\hline
J14h22m25.1s+07d01m58.1s &  Ongoing event (?)\\
 &  Additional variability\\
J15h43m39.8s+08d06m12.8s &  Additional variability\\
J16h03m14.9s+08d10m20.3s &  Pre-variability\\
J16h10m12.4s$-$00d11m41.6s &  Ongoing event (?)\\
J16h17m26.3s+06d32m32.5s &  Low SNR\\
J16h18m23.7s$-$06d03m26.3s &  Additional variability\\
J16h18m46.7s+04d40m06.7s &  Additional variability;\\
J16h25m20.4s+05d56m40.9s &  Additional variability\\
 & Asymmetric dips \\
J16h36m41.6s+09d24m58.0s &  Additional variability\\
J16h37m50.2s+02d11m44.0s &  Additional variability\\
J16h56m00.0s$-$00d30m29.2s &  Additional variability\\
J16h59m10.9s$-$07d37m10.2s &  Additional variability\\
J17h02m19.4s$-$03d38m58.1s &  Additional variability\\
J17h06m45.8s+00d51m56.1s &  Additional variability\\
J17h09m31.9s$-$01d49m16.9s &  Additional variability\\
J17h12m44.0s+05d23m59.7s &  Additional variability\\
J17h16m19.2s+01d33m06.6s &  Additional variability\\
J17h24m17.6s+08d33m46.1s &  Additional variability\\
J17h26m23.7s+04d23m57.5s &  Additional variability\\
J17h29m45.4s+04d16m12.5s &  Second dip (?)\\
J17h32m53.0s+08d58m29.8s &  Additional variability\\
J17h33m24.4s+09d21m41.7s &  Asymmetric dips\\
 & Additional variability \\
J17h36m54.7s$-$07d31m33.0s &  Additional variability\\
J17h54m43.5s+06d46m43.2s &  Second dip\\
J17h57m09.8s+08d56m28.5s &  Additional variability\\
 & Asymmetric caustics \\
J18h00m51.8s+08d31m29.8s &  Additional variability\\
J18h37m04.1s+09d09m24.1s &  Asymmetric caustics;\\
 & Additional variability \\
J19h17m57.7s$-$08d26m51.1s &  Additional variability\\
J19h21m20.0s$-$05d34m32.1s &  Additional variability\\
J19h28m33.2s$-$01d10m46.7s &  Additional variability \\
J19h35m03.6s$-$01d11m06.2s &  Asymmetric caustics\\
 & Additional variability \\
J19h36m37.5s$-$06d17m34.0s &  Additional variability;\\
 & Second dip (?) \\
 J19h47m51.6s+04d22m15.8s &  Asymmetric caustics\\
 & Additional variability \\
J19h49m34.5s+07d08m33.6s &  Additional variability\\
J19h52m35.6s$-$06d57m06.7s &  Additional variability\\
J19h53m41.4s+09d17m39.1s &  Additional variability\\
J19h58m18.1s+06d30m13.6s &  Additional variability\\
 & Pre-variability \\
J20h04m56.5s$-$31d09m50.8s &  Additional variability\\
 & Second dip (?) \\
J20h05m44.9s$-$34d15m15.7s &  Additional variability\\
\hline
\end{tabular}
\end{minipage}
\end{table*}

\clearpage
 
\begin{table}[t]
\centering
\begin{tabular}{ll}
\hline
Source & Comment \\
\hline
J20h11m12.8s+07d13m32.4s &  Asymmetric caustics;\\
 &  Additional variability\\
J20h12m26.5s$-$30d39m46.4s &  Additional variability\\
J20h20m49.5s$-$28d48m22.5s &  Additional variability;\\
 & Pre-variability\\
J20h33m10.5s$-$44d44m52.8s &  Additional variability\\
J20h39m09.1s$-$30d45m20.7s &  Ongoing event (?)\\
 & Additional variability \\
J20h48m47.1s$-$43d59m33.1s &  Additional variability\\
J20h56m55.7s+00d20m31.9s &  Additional variability\\
J21h02m49.3s$-$48d38m04.3s &  Additional variability\\
J21h14m29.8s$-$00d52m17.6s &  Additional variability \\
J21h19m14.3s$-$35d52m38.9s &  Additional variability \\
J22h02m42.1s+04d36m37.8s &  Additional variability\\
\hline
\end{tabular}
\end{table}
